Evolutionary Games on Infinite Strategy Sets: Convergence to Nash Equilibria via Dissipativity

We consider evolutionary dynamics for population games in which players have a continuum of strategies at their disposal. Models in this setting amount to infinite-dimensional differential equations evolving on the manifold of probability measures. We generalize dissipativity theory for evolutionary games from finite to infinite strategy sets that are compact metric spaces, and derive sufficient conditions for the stability of Nash equilibria under the infinite-dimensional dynamics. The resulting analysis is applicable to a broad class of evolutionary games, and is modular in the sense that the pertinent conditions on the dynamics and the game's payoff structure can be verified independently. By specializing our theory to the class of monotone games, we recover as special cases existing stability results for the Brown-von Neumann-Nash and impartial pairwise comparison dynamics. We also extend our theory to models with dynamic payoffs, further broadening the applicability of our framework. Throughout our analyses, we identify and elaborate on new technical conditions that are key in extending dissipativity theory from finite to infinite strategy sets, such as compactness of the set of Nash equilibria and evolution of dynamic payoffs within a compact positively invariant set. We illustrate our theory using a variety of case studies, including a novel, continuous variant of the war of attrition game.

==> root-long_version-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tex/abstract-old.tex <==
\begin{abstract}
In this work, we consider evolutionary dynamics for population games in which players may have a continuum of strategies at their disposal. Models in this setting amount to infinite-dimensional differential equations evolving on the manifold of probability measures. Due to the technical difficulties in analyzing such models, prior works in this setting are restricted to studying specific evolutionary dynamics models on a case-by-case basis. Taking a broader approach, recent work by \citet{arcak2021dissipativity} uses system-theoretic notions of dissipativity to derive sufficient conditions for general evolutionary games to converge to Nash equilibria, but such results are restricted to finite strategy sets. In this paper, we generalize dissipativity theory for evolutionary games to infinite strategy sets that are compact metric spaces. Our main result is a general sufficient condition for dynamic stability of Nash equilibria, and is modular in the sense that the pertinent conditions on the dynamics and the game's payoff structure can be verified independently. By specializing our theory to the class of monotone games, we recover as special cases the key stability results from \citet[Theorem~3]{hofbauer2009brown} and \citet[Theorem~4]{cheung2014pairwise} for the Brown-von Neumann-Nash and impartial pairwise comparison dynamics. We also extend our theory to models with dynamic payoffs, further broadening the applicability of our framework over past works. We illustrate the scope of our theory using examples, including the proposal of a ``continuous war of attrition'' game and its novel stability analysis, and the study of a monotone game subject to smoothing dynamics.
\end{abstract}


==> tex/approx.tex <==
	\section{Approximation via Finite Strategy Sets}
	\label{sec: approx}

	Following a similar spirit as the analysis in \citet{oechssler2002dynamic} for linear games $F$ endowed with the replicator dynamics, we consider in this section the case where an EDM over a finite strategy set approximates an EDM over a possibly infinite strategy set. Throughout this section, we assume that all strategy sets under consideration are compact. We consider rather general dynamics termed \emph{mean dynamics} \citep{sandholm2010population,cheung2014pairwise}, where the dynamics map $v$ takes the form
	\begin{equation}
		v(\mu,\rho)(B) = \int_S \int_B \varphi(s,s',\mu,\rho) d\lambda(s') d\mu(s) - \int_S \int_B \varphi(s',s,\mu,\rho) d\mu(s') d\lambda(s)
		\label{eq: mean_dynamics_map}
	\end{equation}
	for some (fixed-in-time) reference probability measure $\lambda\in\P(S)$ and some adequately integrable map $\varphi \colon S\times S \times \P(S) \times C_0(S) \to \Rpl$. Throughout this section, we do not necessarily assume that $\lambda$ is of full support. The map $\varphi$ is known as the \emph{revision protocol}. The first term in $v(\mu,\rho)(B)$ represents the ``inflow'' of mass into the strategies within $B\in\B(S)$, and the second term represents the corresponding ``outflow.'' The BNN dynamics of \autoref{ex: bnn} and the pairwise comparison dynamics of \autoref{ex: pcd} are both examples of mean dynamics, with $\varphi(s,s',\mu,\rho) = \max\{0,\left<\rho,\delta_{s'}\right> - \left<\rho,\mu\right>\}$ and $\varphi(s,s',\mu,\rho) = \gamma(s,s',\rho)$, respectively.

	Our main approximation result (\autoref{thm: approx} to come) shows that, under some regularity conditions, the solutions of finite approximations weakly converge to the infinite-dimensional dynamics on compact time intervals. We start by formally stating these regularity conditions in \autoref{ass: approx} below. We will soon see that \autoref{ass: approx} is satisfied by the BNN dynamics of \autoref{ex: bnn} and the impartial pairwise comparison dynamics of \autoref{ex: pcd} under suitable payoff structures.

	\begin{assumption}
		\label{ass: approx}
		Consider a game $F\colon \P(S) \to C_0(S)$ and a revision protocol $\varphi \colon S\times S \times \P(S) \times C_0(S) \to \Rpl$. The following all hold:
		\begin{enumerate}
			\item {\bf Boundedness.} There exists $M\in\Rpl$ such that
			\begin{equation*}
				|\varphi(s,s',\mu,F(\mu))| \le M
			\end{equation*}
			for all $s,s'\in S$ and all $\mu\in\P(S)$.
			\item {\bf Lipschitzness on $S$.} There exist $L_1,L_2\in\Rpl$ such that
			\begin{equation*}
				\varphi(\cdot,s',\mu,F(\mu)) \in \lip_{L_1}(S) ~ \text{for all $s'\in S$ and all $\mu\in\P(S)$},
			\end{equation*}
			and
			\begin{equation*}
				\varphi(s,\cdot,\mu,F(\mu)) \in \lip_{L_2}(S) ~ \text{for all $s\in S$ and all $\mu\in\P(S)$}.
			\end{equation*}
			\item {\bf Lipschitzness on $\P(S)$.} There exists $L_3\in\Rpl$ such that, for all $s,s'\in S$, it holds that
			\begin{equation*}
				|\varphi(s,s',\mu,F(\mu)) - \varphi(s,s',\mu',F(\mu'))| \le L_3 \|\mu - \mu'\|_\BL ~ \text{for all $\mu,\mu'\in\P(S)$}.
			\end{equation*}
		\end{enumerate}
	\end{assumption}

	We emphasize that all conditions in \autoref{ass: approx} are with respect to the closed-loop dynamics, i.e., they are required to hold for state-input pairs $(\mu,\rho)$ satisfying $\rho = F(\mu)$. In general, this is much less stringent than requiring them to hold for all states $\mu\in\P(S)$ and all inputs $\rho\in C_0(S)$. We now state the main approximation result.

	\begin{theoremE}[][end,restate,text link=]
		\label{thm: approx}
		Consider a game $F\colon \P(S)\to C_0(S)$ and a revision protocol $\varphi \colon S\times S \times \P(S) \times C_0(S) \to \Rpl$ that together satisfy \autoref{ass: approx}. Let $v\colon \P(S) \times C_0(S) \to T\P(S)$ take the form \eqref{eq: mean_dynamics_map} with some reference measure $\lambda\in\P(S)$, and for all $n\in\N$ let $v_n\colon \P(S) \times C_0(S) \to T\P(S)$ take the form \eqref{eq: mean_dynamics_map} with some reference measure $\lambda_n\in\P(S)$. Assume that \autoref{ass: exist_edm_solution} holds for $v$ and every $v_n$, so that there exist unique solutions $\mu \colon [0,\infty) \to \P(S)$ and $\mu_n \colon [0,\infty) \to \P(S)$ to the EDM \eqref{eq: edm} with dynamics maps $v$ and $v_n$ and arbitrary initial states $\mu(0)\in\P(S)$ and $\mu_n(0)\in\P(S)$, respectively. If $\lambda_n \to \lambda$ weakly as $n\to\infty$ and $\mu_n(0) \to \mu(0)$ weakly as $n\to\infty$, then
		\begin{equation*}
			\lim_{n\to \infty} \sup_{t\in[0,T]} \|\mu_n(t) - \mu(t)\|_\BL = 0
		\end{equation*}
		for all $T\in(0,\infty)$.
	\end{theoremE}

	\begin{proofE}
		Let $T\in(0,\infty)$. Furthermore, let $n\in\N$, let $t\in[0,T]$, and let $g\in\lip_1(S)$ be such that $\|g\|_\infty \le 1$. It holds that
		\begin{align*}
			\int_S g d\mu(t) &= \int_{[0,t]}\int_S g(s) d(\dot{\mu}(\tau))(s) d\tau + \int_S g(s) d(\mu(0))(s) \\
			&= \int_{[0,t]}\int_S g(s) \int_S \varphi(s',s,\mu(\tau),\rho(\tau)) d(\mu(\tau))(s') d\lambda(s) d\tau \\
			&\qquad - \int_{[0,t]}\int_S g(s) \int_S \varphi(s,s',\mu(\tau),\rho(\tau)) d\lambda(s') d(\mu(\tau))(s) d\tau \\
			& \qquad + \int_S g(s) d(\mu(0))(s),
		\end{align*}
		where $\rho(\tau) = F(\mu(\tau))$ for all $\tau\in[0,t]$. Similarly,
		\begin{align*}
			\int_S g d\mu_n(t) &= \int_{[0,t]}\int_S g(s) d(\dot{\mu}_n(\tau))(s) d\tau + \int_S g(s) d(\mu_n(0))(s) \\
			&= \int_{[0,t]}\int_S g(s) \int_S \varphi(s',s,\mu_n(\tau),\rho_n(\tau)) d(\mu_n(\tau))(s') d\lambda_n(s) d\tau \\
			&\qquad - \int_{[0,t]}\int_S g(s) \int_S \varphi(s,s',\mu_n(\tau),\rho_n(\tau)) d\lambda_n(s') d(\mu_n(\tau))(s) d\tau \\
			& \qquad + \int_S g(s) d(\mu_n(0))(s),
		\end{align*}
		where $\rho_n(\tau) = F(\mu_n(\tau))$ for all $\tau\in[0,t]$. Our goal is to estimate the difference $\int_S g d\mu(t) - \int_S g d\mu_n(t)$. We accomplish this by comparing the corresponding ``inflows,'' ``outflows,'' and initial states.

		\paragraph{Inflows.}
		We have that
		\begin{align*}
			\Delta_1(\tau) &\coloneqq \int_S g(s) \int_S \varphi(s',s,\mu(\tau),\rho(\tau)) d(\mu(\tau))(s') d\lambda(s) \\
			& \qquad - \int_S g(s) \int_S \varphi(s',s,\mu_n(\tau),\rho_n(\tau)) d(\mu_n(\tau))(s') d\lambda_n(s) \\
			&= \int_S g(s) \int_S \varphi(s',s,\mu(\tau),\rho(\tau)) d(\mu(\tau))(s') d\lambda(s) \\
			&\qquad - \int_S g(s) \int_S \varphi(s',s,\mu_n(\tau),\rho_n(\tau)) d(\mu(\tau))(s') d\lambda(s) \\
			&\qquad + \int_S g(s) \int_S \varphi(s',s,\mu_n(\tau),\rho_n(\tau)) d(\mu(\tau))(s') d\lambda(s) \\
			&\qquad - \int_S g(s) \int_S \varphi(s',s,\mu_n(\tau),\rho_n(\tau)) d(\mu_n(\tau))(s') d\lambda(s) \\
			&\qquad + \int_S g(s) \int_S \varphi(s',s,\mu_n(\tau),\rho_n(\tau)) d(\mu_n(\tau))(s') d\lambda(s) \\
			&\qquad - \int_S g(s) \int_S \varphi(s',s,\mu_n(\tau),\rho_n(\tau)) d(\mu_n(\tau))(s') d\lambda_n(s).
		\end{align*}
		Comparing neighboring terms, we have that
		\begin{align*}
			& \left|\int_S g(s) \int_S (\varphi(s',s,\mu(\tau),\rho(\tau)) - \varphi(s',s,\mu_n(\tau),\rho_n(\tau))) d(\mu(\tau))(s') d\lambda(s) \right| \\
			&\qquad = \left|\int_S g(s) \int_S (\varphi(s',s,\mu(\tau),F(\mu(\tau))) - \varphi(s',s,\mu_n(\tau),F(\mu_n(\tau)))) d(\mu(\tau))(s') d\lambda(s) \right| \\
			& \qquad \le \int_S |g(s)| \int_S L_3 \|\mu(\tau) - \mu_n(\tau)\|_\BL d(\mu(\tau))(s') d\lambda(s) \\
			&\qquad \le L_3\|\mu(\tau) - \mu_n(\tau)\|_\BL,
		\end{align*}
		which follows from the bound $\|g\|_\infty \le 1$ and the Lipschitzness of $\varphi$ on $\P(S)$. Next,
		\begin{align*}
			& \left|\int_S g(s) \int_S \varphi(s',s,\mu_n(\tau),\rho_n(\tau))d(\mu(\tau) - \mu_n(\tau))(s') d\lambda(s)\right| \\
			&\qquad = \left|\int_S g(s) \int_S \varphi(s',s,\mu_n(\tau),F(\mu_n(\tau)))d(\mu(\tau) - \mu_n(\tau))(s') d\lambda(s)\right| \\
			&\qquad \le \max\{L_1,M\} \|\mu(\tau) - \mu_n(\tau)\|_\BL,
		\end{align*}
		which follows from the boundedness and Lipschitzness of $\varphi$ in its first argument together with the bound $\|g\|_\infty \le 1$. Furthermore,
		\begin{align*}
			& \left|\int_S g(s) \int_S \varphi(s',s,\mu_n(\tau),\rho_n(\tau)) d(\mu_n(\tau))(s') d(\lambda - \lambda_n)(s)\right| \\
			& \qquad =\left|\int_S\int_S g(s) \varphi(s',s,\mu_n(\tau),F(\mu_n(\tau))) d(\lambda - \lambda_n)(s) d(\mu_n(\tau))(s')\right| \\
			&\qquad \le (L_2+M) \|\lambda - \lambda_n\|_\BL,
		\end{align*}
		which follows from the fact that $s\mapsto g(s)\varphi(s',s,\mu_n(\tau),F(\mu_n(\tau)))$ is bounded with constant $M$ and Lipschitz with constant $L_2+M$ (which intimately relies on boundedness of both $g$ and $\varphi$; in general, the product of Lipschitz functions is not Lipschitz). Thus, we conclude that
		\begin{equation*}
			|\Delta_1(\tau)| \le (L_3 + \max\{L_1,M\})\|\mu(\tau) - \mu_n(\tau)\|_\BL + (L_2+M) \|\lambda-\lambda_n\|_\BL.
		\end{equation*}

		\paragraph{Outflows.}
		Performing a nearly identical analysis as above, we find that for
		\begin{align*}
			\Delta_2(\tau) &\coloneqq \int_S g(s) \int_S \varphi(s,s',\mu(\tau),\rho(\tau)) d\lambda(s') d(\mu(\tau))(s) \\
			&\qquad - \int_S g(s) \int_S \varphi(s,s',\mu_n(\tau),\rho_n(\tau)) d\lambda_n(s') d(\mu_n(\tau))(s),
		\end{align*}
		it holds that
		\begin{equation*}
			|\Delta_2(\tau)| \le (L_1+L_3+M)\|\mu(\tau) - \mu_n(\tau)\|_\BL + \max\{L_2,M\}\|\lambda - \lambda_n\|_\BL.
		\end{equation*}

		\paragraph{Initial states.}

		We clearly have that
		\begin{equation*}
			\left|\int_S g(s) d(\mu(0))(s) - \int_S g(s) d(\mu_n(0))(s)\right| \le \|\mu(0)-\mu_n(0)\|_\BL,
		\end{equation*}
		since $\|g\|_\infty\le 1$ and $g\in\lip_1(S)$.

		\paragraph{Completing the proof.}

		Given our above estimates, we complete the proof as follows. First, we see that
		\begin{align*}
			& \left|\int_S gd\mu(t) - \int_S gd\mu_n(t)\right| \\
			& \qquad \le \int_{[0,t]}(|\Delta_1(\tau)| + |\Delta_2(\tau)|)d\tau + \|\mu(0) - \mu_n(0)\|_\BL \\
			& \qquad \le \int_{[0,t]}((2L_3 + L_1+M + \max\{L_1,M\})\|\mu(\tau)-\mu_n(\tau)\|_\BL + (L_2+M+\max\{L_2,M\})\|\lambda-\lambda_n\|_\BL)d\tau \\
			&\qquad \qquad + \|\mu(0) - \mu_n(0)\|_\BL \\
			&\qquad \le K \int_{[0,t]}(\|\mu(\tau)-\mu_n(\tau)\|_\BL + \|\lambda-\lambda_n\|_\BL)d\tau + \|\mu(0) - \mu_n(0)\|_\BL,
		\end{align*}
		where $K \coloneqq \max\{2L_3+3\max\{L_1,M\},3\max\{L_2,M\}\}$. Since $g$ is an arbitrary function in $\lip_1(S)$ satisfying $\|g\|_\infty \le 1$, we may take the supremum on the right-hand side of the above inequality to find that
		\begin{equation*}
			\|\mu(t) - \mu_n(t)\|_\BL \le K \int_{[0,t]}\left(\|\mu(\tau) - \mu_n(\tau)\|_\BL + \|\lambda - \lambda_n\|_\BL\right)d\tau + \|\mu(0) - \mu_n(0)\|_\BL.
		\end{equation*}
		Applying Gr\"onwall's inequality gives that
		\begin{align*}
			\|\mu(t) - \mu_n(t)\|_\BL &\le - \|\lambda - \lambda_n\|_\BL + (\|\lambda - \lambda_n\|_\BL + \|\mu(0) - \mu_n(0)\|_\BL) e^{Kt} \\
			& \le - \|\lambda - \lambda_n\|_\BL + (\|\lambda - \lambda_n\|_\BL + \|\mu(0) - \mu_n(0)\|_\BL) e^{KT},
		\end{align*}
		where the final inequality follows from the fact that $t\in[0,T]$ was chosen arbitrarily. Thus,
		\begin{equation*}
			\sup_{t\in[0,T]} \|\mu(t) - \mu_n(t)\|_\BL \le - \|\lambda - \lambda_n\|_\BL + (\|\lambda - \lambda_n\|_\BL + \|\mu(0) - \mu_n(0)\|_\BL) e^{KT}.
		\end{equation*}
		Since $n\in\N$ was chosen arbitrarily and $\lim_{n\to\infty} \|\lambda - \lambda_n\|_\BL = \lim_{n\to\infty}\| \mu(0) - \mu_n(0)\|_\BL = 0$ as both $\lambda_n \to \lambda$ weakly and $\mu_n(0) \to \mu(0)$ weakly as $n\to \infty$, we conclude that
		\begin{equation*}
			\lim_{n\to\infty} \sup_{t\in[0,T]} \|\mu(t) - \mu_n(t)\|_\BL = 0,
		\end{equation*}
		which is what was to be proven.
	\end{proofE}

	\begin{remark}
		\label{rem: approx}
		\autoref{thm: approx} yields quite a strong version of weak convergence of the approximation. In particular, the conclusion implies that, for all $T\in(0,\infty)$, it holds that
		\begin{equation*}
			\sup_{t\in[0,T]}\lim_{n\to\infty} \|\mu_n(t) - \mu(t)\|_\BL \le \lim_{n\to\infty}\sup_{t\in[0,T]}\|\mu_n(t) - \mu(t)\|_\BL = 0,
		\end{equation*}
		and hence for all $t\in[0,\infty)$, it holds that $\mu_n(t) \to \mu(t)$ weakly as $n\to\infty$.
	\end{remark}

	\begin{remark}
		\label{rem: empirical_distribution}
		Notice that, given a measure $\lambda\in\P(S)$, we may always construct an approximating measure $\lambda_n \coloneqq \frac{1}{n}\sum_{i=1}^n \delta_{s_i} \in\P(S)$ with $s_1,\dots,s_n \in S$ random variables drawn independently and identically distributed from $\lambda$, and in this case, the law of large numbers yields that $\lambda_n \to \lambda$ weakly as $n\to\infty$ $\lambda$-almost surely.
	\end{remark}

	Although \autoref{thm: approx} holds for general approximating measures $\lambda_n,\mu_n(0) \in\P(S)$, it is most useful to think of these as discrete measures with $\supp(\lambda_n) = \supp(\mu_n(0))$ and with $\card(\supp(\mu_n(0))) = n$. In this case, the evolutionary dynamics governed by the dynamics map $v_n$ are finite-dimensional (i.e., a system of $n$ ordinary differential equations), since all of the mass of $\mu_n$ remains on $\supp(\mu_n(0))$; the mass evolves on a finite set of strategies. Indeed, such approximations reduce to the more classical evolutionary dynamics models constructed directly on finite strategy sets, which we will formally show in \autoref{sec: approximation_reduction}. Before doing so, we will now show that, under ``suitably nice'' payoff structures, the BNN dynamics of \autoref{ex: bnn} and the impartial pairwise comparison dynamics of \autoref{ex: pcd} satisfy \autoref{ass: approx}.

	\begin{propositionE}[][end,restate,text link=]
		\label{prop: bnn_pcd_approx}
		Suppose that $S$ is compact. Consider a game $F\colon \P(S) \to C_0(S)$ and let $v \colon \P(S) \times C_0(S) \to T\P(S)$ be the dynamics map for either the BNN dynamics of \autoref{ex: bnn} or the impartial pairwise comparison dynamics of \autoref{ex: pcd} satisfying $\phi_{s'}\in\lip_{L'}(\R)$ for all $s'\in S$, for some $L'\in\Rpl$ (e.g., the Smith dynamics). If $F$ is Lipschitz continuous with respect to $\|\cdot\|_\BL$ and there exists $L\in\Rpl$ such that $F(\mu)\in\lip_L(S)$ for all $\mu\in\P(S)$, then \autoref{ass: approx} holds. In particular, this is the case for $F$ defined by
		\begin{equation*}
			F(\mu)(s) = \int_S f(s,s')d\mu(s')
		\end{equation*}
		with $f \colon S\times S \to \R$ bounded and Lipschitz with respect to the metric defined by $d_{S\times S}((s,s'),(\overline{s},\overline{s}')) = \|(d_S(s,\overline{s}),d_S(s',\overline{s}'))\|$ with $\|\cdot\|$ being any $p$-norm (including $p=\infty$) on $\R^2$ (which of course metrizes the product topology on $S\times S$).
	\end{propositionE}

	\begin{proofE}
		We first prove that the hypotheses on $F$ hold when $F$ is defined by
		\begin{equation}
			F(\mu)(s) = \int_S f(s,s')d\mu(s'),
			\label{eq: linear_payoff}
		\end{equation}
		with $f\colon S\times S \to \R$ bounded and Lipschitz with respect to $d_{S\times S}$. Let $M_f\in\Rpl$ and $L_f\in\Rpl$ be the associated boundedness and Lipschitzness constants of $f$, so that
		\begin{equation*}
			\sup_{(s,s')\in S\times S} |f(s,s')| \le M_f,
		\end{equation*}
		and
		\begin{equation*}
			|f(s,s') - f(\overline{s},\overline{s}')| \le L_f d_{S\times S}((s,s'),(\overline{s},\overline{s}'))
		\end{equation*}
		for all $(s,s'),(\overline{s},\overline{s}')\in S\times S$. It is easy to see that, since $d_{S\times S}((s,s'),(\overline{s},\overline{s}')) = \|(d_S(s,\overline{s}),d_S(s',\overline{s}'))\|$ for some $p$-norm on $\R^2$, it holds that $f(s,\cdot)$ and $f(\cdot,s')$ are $L_f$-Lipschitz on $S$ with respect to $d_S$, for all $s,s'\in S$.

		Let $\mu,\mu'\in\P(S)$. Then
		\begin{align*}
			\|F(\mu) - F(\mu')\|_\infty &= \sup_{s\in S}\left|\int_S f(s,s') d\mu(s') - \int_S f(s,s') d\mu'(s')\right| \\
			&= \sup_{s\in S} \left|\int_S f(s,s')d(\mu-\mu')(s')\right| \\
			&\le \max\{M_f,L_f\} \|\mu - \mu'\|_\BL,
		\end{align*}
		which proves that $F$ is Lipschitz continuous with respect to $\|\cdot\|_\BL$. Furthermore, we find that, for all $s,s'\in S$, it holds that
		\begin{equation*}
			|F(\mu)(s) - F(\mu)(s')| = \left|\int_S (f(s,\overline{s}) - f(s',\overline{s}))d\mu(\overline{s})\right| \le \int_S |f(s,\overline{s}) - f(s',\overline{s})|d|\mu|(\overline{s}) \le L_f d_S(s,s').
		\end{equation*}
		This proves that $F(\mu)\in \lip_{L_f}(S)$ for all $\mu\in\P(S)$, and hence that $F$ indeed satisfies the hypotheses of the lemma when given by \eqref{eq: linear_payoff}.

		Now suppose that $F$ is a general map (i.e., it does not necessarily take the form \eqref{eq: linear_payoff}) that is Lipschitz continuous with respect to $\|\cdot\|_\BL$, so that there exists $K\in\Rpl$ such that
		\begin{equation*}
			\|F(\mu) - F(\mu')\|_\infty \le K \|\mu - \mu'\|_\BL.
		\end{equation*}
		Furthermore, suppose that there exists $L\in\Rpl$ such that $F(\mu)\in\lip_L(S)$ for all $\mu\in\P(S)$. We will now prove the result for the two dynamics separately.
		
		\paragraph{BNN dynamics.}

		Consider the BNN dynamics of \autoref{ex: bnn}. The revision protocol is defined by
		\begin{equation*}
			\varphi(s,s',\mu,\rho) = \max\{0,\left<\rho,\delta_{s'}\right> - \left<\rho,\mu\right>\}.
		\end{equation*}
		
		Let $s,s'\in S$ and let $\mu\in\P(S)$. It holds that
		\begin{align*}
			|\varphi(s,s',\mu,F(\mu))| &\le |\left<F(\mu),\delta_{s'} - \mu\right>| \\
			&\le \|F(\mu)\|_\infty \|\delta_{s'} - \mu\|_\TV \\
			&\le 2\|F(\mu)\|_\infty \\
			&\le M
		\end{align*}
		with $M \coloneqq \frac{1}{2}\sup_{\mu' \in\P(S)}\|F(\mu')\|_\infty$ finite, since $F$ being Lipschitz continuous with respect to $\|\cdot\|_\BL$ implies that $F$ is weakly continuous, and hence $\mu' \mapsto \|F(\mu')\|_\infty$ is a weakly continuous map from the weakly compact set $\P(S)$ to $\Rpl$ (where weak compactness of $\P(S)$ comes from \autoref{lem: P(S)_compact}). This proves the first condition in \autoref{ass: approx}.

		Next, notice that, for all $s'\in S$ and all $\mu\in\P(S)$, the function $s\mapsto \varphi(s,s',\mu,F(\mu))$ is constant and hence Lipschitz with constant $0$. Let $s\in S$ and let $\mu\in\P(S)$. We see that
		\begin{align*}
			s' \mapsto \left<F(\mu),\delta_{s'}\right> - \left<F(\mu),\mu\right> = F(\mu)(s') - \left<F(\mu),\mu\right>
		\end{align*}
		is $L$-Lipschitz on $S$ since $F(\mu)\in \lip_L(S)$. Therefore, the composition
		\begin{equation*}
			s'\mapsto \varphi(s,s',\mu,F(\mu)) = \max\{0,\left<F(\mu),\delta_{s'}\right> - \left<F(\mu),\mu\right>\}
		\end{equation*}
		is also $L$-Lipschitz on $S$. Since $s$ and $\mu$ are arbitrary, this proves the second condition in \autoref{ass: approx}.

		Finally, let $s,s'\in S$ and let $\mu,\mu'\in\P(S)$. It holds that
		\begin{align*}
			& |\left<F(\mu),\delta_{s'}\right> - \left<F(\mu),\mu\right> - \left<F(\mu'),\delta_{s'}\right> + \left<F(\mu'),\mu'\right>| \\
			& \qquad \le |\left<F(\mu)-F(\mu'),\delta_{s'}\right>| + |\left<F(\mu),\mu\right> - \left<F(\mu),\mu'\right>| + |\left<F(\mu),\mu'\right> - \left<F(\mu'),\mu'\right>| \\
			&\qquad \le \|F(\mu)-F(\mu')\|_\infty + \left|\int_S F(\mu) d(\mu-\mu')\right| + \|F(\mu)-F(\mu')\|_\infty \\
			&\qquad \le 2K\|\mu-\mu'\|_\BL + \left|\int_S F(\mu) d(\mu-\mu')\right|.
		\end{align*}
		Since $F(\mu) \in \lip_L(S)$ and $\|F(\mu)\|_\infty \le 2M$, it holds that $F(\mu)$ is a bounded Lipschitz function, and we find that
		\begin{equation*}
			\left|\int_S F(\mu) d(\mu-\mu')\right| \le \max\{L,2M\} \|\mu-\mu'\|_\BL.
		\end{equation*}
		Thus,
		\begin{align*}
			& |\left<F(\mu),\delta_{s'}\right> - \left<F(\mu),\mu\right> - \left<F(\mu'),\delta_{s'}\right> + \left<F(\mu'),\mu'\right>| \\
			& \qquad \le (2K+\max\{L,2M\}) \|\mu-\mu'\|_\BL.
		\end{align*}
 		Since $s,s'\in S$ and $\mu,\mu'\in\P(S)$ were chosen arbitrarily, we conclude that
		\begin{equation*}
			\mu \mapsto \left<F(\mu),\delta_{s'}\right> - \left<F(\mu),\mu\right>
		\end{equation*}
		is Lipschitz continuous with respect to $\|\cdot\|_\BL$ with constant $2K+\max\{L,2M\}$ for all $s,s'\in S$. Since $x\mapsto \max\{0,x\}$ is a real-valued $1$-Lipschitz function on $\R$, this proves Lipschitzness of the composition, i.e., that
		\begin{equation*}
			|\varphi(s,s',\mu,F(\mu)) - \varphi(s,s',\mu',F(\mu'))| \le (2K+\max\{L,2M\})\|\mu-\mu'\|_\BL
		\end{equation*}
		for all $s,s'\in S$ and all $\mu,\mu'\in\P(S)$. This concludes the proof for the BNN dynamics.

		\paragraph{Impartial pairwise comparison dynamics.}

		Consider the impartial pairwise comparison dynamics of \autoref{ex: pcd}. The revision protocol is defined by
		\begin{equation*}
			\varphi(s,s',\mu,\rho) = \phi_{s'}(\rho(s') - \rho(s)),
		\end{equation*}
		where, under our assumptions, $\phi_{s'}$ is a nonnegative $L'$-Lipschitz function on $\R$ satisfying $\phi_{s'}(0) = 0$ by sign-preservation.
		
		Let $s,s'\in S$ and let $\mu\in\P(S)$. It holds that
		\begin{align*}
			|\varphi(s,s',\mu,F(\mu))| &= |\phi_{s'}(F(\mu)(s') - F(\mu)(s))| \\
			&= |\phi_{s'}(F(\mu)(s') - F(\mu)(s)) - \phi_{s'}(0)| \\
			&\le L' |F(\mu)(s') - F(\mu)(s) - 0| \\
			&\le \|F(\mu)\|_\infty \|\delta_{s'} - \delta_s\|_\TV \\
			&\le 2\|F(\mu)\|_\infty \\
			&\le M
		\end{align*}
		with $M \coloneqq \frac{1}{2}\sup_{\mu' \in\P(S)}\|F(\mu')\|_\infty$ finite, since $F$ being Lipschitz continuous with respect to $\|\cdot\|_\BL$ implies that $F$ is weakly continuous, and hence $\mu' \mapsto \|F(\mu')\|_\infty$ is a weakly continuous map from the weakly compact set $\P(S)$ to $\Rpl$ (where weak compactness of $\P(S)$ comes from \autoref{lem: P(S)_compact}). This proves the first condition in \autoref{ass: approx}.

		Next, let $s' \in S$ and let $\mu\in\P(S)$. We see that
		\begin{equation*}
			s\mapsto F(\mu)(s') - F(\mu)(s)
		\end{equation*}
		is $L$-Lipschitz on $S$ since $F(\mu)\in\lip_L(S)$. Therefore, the composition
		\begin{equation*}
			s\mapsto \varphi(s,s',\mu,F(\mu)) = \phi_{s'}(F(\mu)(s) - F(\mu)(s'))
		\end{equation*}
		is Lipschitz continuous on $S$ with constant $L'\cdot L$. Following the same line of analysis shows that, for all $s\in S$ and all $\mu\in\P(S)$, it holds that
		\begin{equation*}
			s' \mapsto \varphi(s,s',\mu,F(\mu))
		\end{equation*}
		is Lipschitz continuous on $S$ with constant $L'\cdot L$. Therefore, the second condition in \autoref{ass: approx} holds.

		Finally, let $s,s'\in S$ and let $\mu,\mu'\in\P(S)$. It holds that
		\begin{align*}
			|F(\mu)(s') - F(\mu)(s) - F(\mu')(s') + F(\mu')(s)| &\le |F(\mu)(s') - F(\mu')(s')| + |F(\mu)(s) - F(\mu')(s)| \\
			& \le 2\|F(\mu) - F(\mu')\|_\infty \\
			& \le 2K\|\mu-\mu'\|_\BL.
		\end{align*}
 		Since $s,s'\in S$ and $\mu,\mu'\in\P(S)$ were chosen arbitrarily, we conclude that
		\begin{equation*}
			\mu \mapsto F(\mu)(s') - F(\mu)(s)
		\end{equation*}
		is Lipschitz continuous with respect to $\|\cdot\|_\BL$ with constant $2K$ for all $s,s'\in S$. Since $\phi_{s'}$ is a real-valued $L'$-Lipschitz function on $\R$, this proves Lipschitzness of the composition, i.e., that
		\begin{equation*}
			|\varphi(s,s',\mu,F(\mu)) - \varphi(s,s',\mu',F(\mu'))| \le 2KL'\|\mu-\mu'\|_\BL
		\end{equation*}
		for all $s,s'\in S$ and all $\mu,\mu'\in\P(S)$. This concludes the proof for the impartial pairwise comparison dynamics.
	\end{proofE}

	\subsection{Reducing Approximations to Finite-Dimensional Dynamics}
	\label{sec: approximation_reduction}

	We will now make explicit the equivalence of the approximation dynamics with measures $\lambda_n,\mu_n(0)$ having finite support and the classical mean dynamics defined directly on finite strategy sets. Consider $n\in\N$, and suppose that $\supp(\lambda_n) = \supp(\mu_n(0)) = \{s_1,\dots,s_n\} \subseteq S$, with $\lambda_n = \sum_{i=1}^n \lambda_n(s_i) \delta_{s_i}$ and $\mu_n(0) = \sum_{i=1}^n (\mu_n(0))(s_i) \delta_{s_i}$ being discrete measures with respect to some reference measure $\nu\in\P(S)$ (e.g., Lebesgue measure when $S$ is a subset of Euclidean space). Here, we write $\lambda_n(s_i)$ to mean $\lambda_n(\{s_i\})$ and similarly for other measures evaluated on singleton sets. For notational convenience, define $S_n \coloneqq \{s_1,\dots,s_n\}$. Then, writing the closed-loop mean dynamics for the approximation yields
	\begin{align*}
		(\dot{\mu}_n(t))(B) &= v_n(\mu_n(t),F(\mu_n(t)))(B) \\
		&= \int_S\int_B \varphi(s,s',\mu_n(t),F(\mu_n(t))) d\lambda_n(s') d(\mu_n(t))(s) \\
		&\qquad - \int_S\int_B \varphi(s',s,\mu_n(t),F(\mu_n(t))) d(\mu_n(t))(s') d\lambda_n(s)
	\end{align*}
	for all $B\in\B(S)$. Since $\lambda_n(B) = (\mu_n(0))(B) = 0$ for $B = S\setminus S_n$, we immediately see that $(\dot{\mu}_n(0))(B) = 0$ and hence $(\mu_n(t))(B) = 0$ for all $t\in[0,\infty)$ for this set $B$. Thus, for all such $t$, the probability measure $\mu_n(t)$ is discrete with respect to the reference measure $\nu$ and has support $S_n$, implying that it takes the form
	\begin{equation*}
		\mu_n(t) = \sum_{i=1}^n (\mu_n(t))(s_i) \delta_{s_i}.
	\end{equation*}
	That is, $\mu_n$ is a curve evolving in the set
	\begin{equation*}
	\D(S_n) \coloneqq \conv\left(\bigcup_{s\in S_n}\{\delta_{s}\}\right) = \left\{\sum_{i=1}^n \theta_i \delta_{s_i} \in\P(S) : \theta \in \Delta^{n-1}\right\}.
	\end{equation*}
	Again utilizing the expression for the mean dynamics, we see that the mass on strategy $s_i$ evolves according to
	\begin{align*}
		(\dot{\mu}_n(t))(s_i) &= \lambda_n(s_i)\sum_{j=1}^n \varphi(s_j,s_i,\mu_n(t),F(\mu_n(t))) (\mu_n(t))(s_j) \\
		&\qquad - (\mu_n(t))(s_i) \sum_{j=1}^n \varphi(s_i,s_j,\mu_n(t),F(\mu_n(t))) \lambda_n(s_j).
	\end{align*}
	Now, we may uniquely identify $\mu_n$ with the curve $x\colon [0,\infty) \to \Rn$ defined by $x_i(t) = (\mu_n(t))(s_i)$. In doing so, it is easy to see that $\dot{x}_i(t) \coloneqq \frac{d x_i}{dt}(t) = (\dot{\mu}_n(t))(s_i)$. Continuing with our reduction, we may define an equivalent ``finite-dimensional game'' $\overline{F}\colon \Delta^{n-1} \to \Rn$ as the restriction of $F$ to the set of discrete measures in which the curve $\mu_n$ evolves:
	\begin{equation*}
		\overline{F}_i(\theta) = F\left(\sum_{j=1}^n \theta_j \delta_{s_j}\right)(s_i), ~ i\in\{1,\dots,n\}.
	\end{equation*}
	Notice that $\overline{F}$ is continuous (in the usual sense) whenever $F$ is weakly continuous. An equivalent (closed-loop) finite-dimensional revision protocol $\overline{\varphi} \colon \{1,\dots,n\}\times \{1,\dots,n\} \times \Delta^{n-1} \to \Rpl$ may be defined as
	\begin{equation*}
		\overline{\varphi}(i,j,\theta) = \varphi\left(s_i,s_j,\sum_{k=1}^n \theta_k \delta_{s_k}, F\left(\sum_{k=1}^n \theta_k \delta_{s_k}\right)\right).
	\end{equation*}
	These constructions allow us to equivalently rewrite the closed-loop mean dynamics of the approximation as
	\begin{equation}
		\dot{x}_i(t) = \lambda_n(s_i) \sum_{j=1}^n \overline{\varphi}(j,i,x(t)) x_j(t) - x_i(t) \sum_{j=1}^n \overline{\varphi}(i,j,x(t))\lambda_n(s_j), ~ i\in\{1,\dots,n\},
		\label{eq: n_ode}
	\end{equation}
	where of course $x(t) = (x_1(t),\dots,x_n(t))$. In setting $\lambda_n(s_i) = \frac{1}{n}$ for all $i\in\{1,\dots,n\}$, the system \eqref{eq: n_ode} of $n$ ordinary differential equations takes the form of the canonical mean dynamics over a finite strategy set (c.f., \citealt[Section~4.2]{sandholm2010population}). For the BNN dynamics of \autoref{ex: bnn}, our construction with $\lambda_n(s_i) = \frac{1}{n}$ for all $i$ amounts to
	\begin{equation*}
		\overline{\varphi}(i,j,\theta) = \max\left\{0,\overline{F}_j(\theta) - \theta^\top \overline{F}(\theta)\right\},
	\end{equation*}
	leading to
	\begin{equation*}
		\dot{x}_i(t) = \max\{0,\overline{F}_i(x(t)) - x(t)^\top \overline{F}(x(t))\} - x_i(t)\sum_{j=1}^n \max\{0,\overline{F}_j(x(t)) - x(t)^\top \overline{F}(x(t))\}, ~ i\in\{1,\dots,n\},
	\end{equation*}
	which coincides with the classical BNN dynamics on the finite strategy set $\{1,\dots,n\}$ (c.f., \citealt[Example~4.3.4]{sandholm2010population}). Similar recovery of the classical finite-dimensional pairwise comparison dynamics on $\{1,\dots,n\}$ are also achieved.

	Our reduction to finite-dimensional dynamics culminates in the following result as a corollary to \autoref{thm: approx}.

	\begin{corollaryE}[][end,restate,text link=]
		\label{cor: finite_approx}
		Consider a game $F\colon \P(S) \to C_0(S)$ and a revision protocol $\varphi \colon S \times S \times \P(S) \times C_0(S) \to \Rpl$ that together satisfy \autoref{ass: approx}. Let $v \colon \P(S) \times C_0(S) \to T\P(S)$ take the form \eqref{eq: mean_dynamics_map} with some reference measure $\lambda\in\P(S)$, and assume that \autoref{ass: exist_edm_solution} holds for $v$, so that there exists a unique solution $\mu \colon [0,\infty) \to \P(S)$ to the EDM \eqref{eq: edm} with dynamics map $v$ and arbitrary initial state $\mu(0)\in\P(S)$. Let $s_i \in S$ for all $i\in\N$, and let $\theta_n,x_n(0) \in \Delta^{n-1}$ for all $n\in\N$. Suppose that, for all $n\in\N$, there exists a unique solution $x_n \colon [0,\infty) \to \Delta^{n-1}$ to the system \eqref{eq: n_ode} of finite-dimensional ordinary differential equations with $\lambda_n \coloneqq \sum_{i=1}^n (\theta_n)_i \delta_{s_i}$ and initial state $x_n(0)$. If $\lambda_n \to \lambda$ weakly as $n\to\infty$ and $\sum_{i=1}^n (x_n(0))_i \delta_{s_i} \to \mu(0)$ weakly as $n\to\infty$, then
		\begin{equation}
			\lim_{n\to\infty} \sup_{t\in[0,T]}\left\| \sum_{i=1}^n (x_n(t))_i \delta_{s_i} - \mu(t) \right\|_\BL = 0
			\label{eq: finite_approx}
		\end{equation}
		for all $T\in (0,\infty)$. Furthermore, it holds that
		\begin{equation}
			\lim_{t\to\infty}\lim_{n\to\infty}\left\|\sum_{i=1}^n (\overline{x}_n)_i \delta_{s_i} - \mu(t)\right\|_\BL = 0
			\label{eq: finite_approx-2}
		\end{equation}
		whenever one also has that
		\begin{equation}
		\lim_{t\to\infty} \sup_{n\in\N}\|x_n(t) - \overline{x}_n\|_1 = 0
		\label{eq: not_paralyzed_by_choice}
		\end{equation}
		for some countable collection $\{\overline{x}_n \in \Delta^{n-1} : n\in\N\}$. In this case,
		\begin{enumerate}
			\item $\mu(t) \to \overline{\mu}$ weakly as $t\to\infty$ whenever $\sum_{i=1}^n (\overline{x}_n)_i \delta_{s_i} \to \overline{\mu}$ weakly as $n\to\infty$ for some $\overline{\mu}\in\P(S)$, and
			\item $\sum_{i=1}^n (\overline{x}_n)_i \delta_{s_i} \to \overline{\mu}$ weakly as $n\to\infty$ whenever $\mu(t) \to \overline{\mu}$ weakly as $t\to\infty$ for some $\overline{\mu}\in\P(S)$.
		\end{enumerate}
	\end{corollaryE}

	\begin{proofE}
		The result \eqref{eq: finite_approx} follows trivially from \autoref{thm: approx} together with the established equivalence between the finite-dimensional dynamics \eqref{eq: n_ode} with initial state $x_n(0)$ and the mean dynamics \eqref{eq: mean_dynamics_map} with reference measure $\lambda_n$ and initial state $\mu_n(0) \coloneqq \sum_{i=1}^n (x_n(0))_i \delta_{s_i}$.

		To prove that \eqref{eq: finite_approx-2} follows under the additional hypothesis \eqref{eq: not_paralyzed_by_choice}, suppose that
		\begin{equation*}
			\lim_{t\to\infty}\sup_{n\in\N}\|x_n(t) - \overline{x}_n\|_1 = 0
		\end{equation*}
		for some countable collection $\{\overline{x}_n\in\Delta^{n-1} : n\in\N\}$. Let $T\in(0,\infty)$. Then, we have for all $t\in[0,T]$ that
		\begin{align*}
			\limsup_{n \to \infty}\left\|\sum_{i=1}^n (\overline{x}_n)_i \delta_{s_i} - \mu(t)\right\|_\BL &\le \limsup_{n \to \infty} \left\|\sum_{i=1}^n ((\overline{x}_n)_i - (x_n(t))_i)\delta_{s_i}\right\|_\BL + \limsup_{n\to\infty} \left\|\sum_{i=1}^n (x_n(t))_i\delta_{s_i} - \mu(t)\right\|_\BL \\
			&\le \limsup_{n \to \infty} \left\|\sum_{i=1}^n ((\overline{x}_n)_i - (x_n(t))_i)\delta_{s_i}\right\|_\BL \\
			&\qquad + \limsup_{n\to\infty} \sup_{t\in[0,T]} \left\|\sum_{i=1}^n (x_n(t))_i\delta_{s_i} - \mu(t)\right\|_\BL \\
			&= \limsup_{n \to \infty} \left\|\sum_{i=1}^n ((\overline{x}_n)_i - (x_n(t))_i)\delta_{s_i}\right\|_\BL \\
			&\le \sup_{n \in \N} \left\|\sum_{i=1}^n ((\overline{x}_n)_i - (x_n(t))_i)\delta_{s_i}\right\|_\BL.
		\end{align*}
		In particular, at $t=T$, we find that
		\begin{equation*}
			\limsup_{n \to \infty}\left\|\sum_{i=1}^n (\overline{x}_n)_i \delta_{s_i} - \mu(T)\right\|_\BL \le \sup_{n \in \N} \left\|\sum_{i=1}^n ((\overline{x}_n)_i - (x_n(T))_i)\delta_{s_i}\right\|_\BL.
		\end{equation*}
		Since $T\in(0,\infty)$ is arbitrary, we conclude that
		\begin{align*}
			\limsup_{T\to\infty} \limsup_{n\to\infty} \left\|\sum_{i=1}^n (\overline{x}_n)_i \delta_{s_i} - \mu(T)\right\|_\BL &\le \limsup_{T\to\infty}\sup_{n \in \N} \left\|\sum_{i=1}^n ((\overline{x}_n)_i - (x_n(T))_i)\delta_{s_i}\right\|_\BL \\
			&\le \limsup_{T\to\infty} \sup_{n\in\N} \sum_{i=1}^n |(\overline{x}_n)_i - (x_n(T))_i| \|\delta_{s_i}\|_\BL \\
			&= \limsup_{T\to\infty} \sup_{n\in\N} \sum_{i=1}^n |(\overline{x}_n)_i - (x_n(T))_i| \\
			&= \limsup_{T\to\infty} \sup_{n\in\N} \|\overline{x}_n - x_n(T)\|_1 \\
			&= 0.
		\end{align*}
		Hence,
		\begin{equation*}
			\lim_{t\to\infty} \lim_{n\to\infty} \left\|\sum_{i=1}^n (\overline{x}_n)_i \delta_{s_i} - \mu(t)\right\|_\BL = 0,
		\end{equation*}
		which proves \eqref{eq: finite_approx-2}. The two final enumerated results follow trivially from the triangle inequality.
	\end{proofE}

	At this point, let us dissect \autoref{cor: finite_approx}. The result \eqref{eq: finite_approx} carries the same interpretation as the main approximation result of \autoref{thm: approx}, namely, that the approximate dynamics over finite strategy sets converge to the dynamics of the infinite-dimensional game uniformly on compact time intervals, as the number of strategies increase. The two final enumerated results ensure coincidence between an asymptotically stable equilibrium $\overline{\mu}$ of the infinite-dimensional game and the limit of the asymptotically stable equilibria $\overline{x}_n$ of the approximations. In particular, they assert that, when the discrete distribution generated by $\overline{x}_n$ converges towards some limiting distribution $\overline{\mu}$, then $\mu(t)$ must approach this same distribution, and, on the other hand, when $\mu(t)$ approaches some limiting distribution $\overline{\mu}$, the discrete distribution generated by $\overline{x}_n$ must converge towards the same distribution. These two results depend on \eqref{eq: finite_approx-2} holding, which relies intimately on the condition \eqref{eq: not_paralyzed_by_choice}. We now discuss this condition further.

	Mathematically, the condition \eqref{eq: not_paralyzed_by_choice} is a form of uniform convergence, namely, it may be equivalently stated as the following holding: for all $\epsilon > 0$, there exists $T > 0$ such that
	\begin{equation*}
		\| x_n (t) - \overline{x}_n\|_1 < \epsilon ~ \text{for all $t > T$ and all $n\in\N$}.
	\end{equation*}
	In other words, \eqref{eq: not_paralyzed_by_choice} holds if and only if $x_n(t) \to \overline{x}_n$ as $t\to\infty$, uniformly in $n$, and with respect to the topology induced by $\|\cdot\|_1$. Notice that we cannot hastily replace $\|\cdot\|_1$ with some other norm, even if they induce the same topology on $\Rn$ for fixed values of $n$, since the tightness of the bounds between equivalent norms on $\Rn$ may in general depend on $n$. Using $\|\cdot\|_1$ is natural in our setting, especially when considering a varying number of strategies $n\in\N$, as $\|x\|_1 = 1$ for all $x\in\Delta^{n-1}$ and $\sup_{x,x'\in\Delta^{n-1}}\|x-x'\|_1 \le 2$, irrespective of $n$.

	We now consider what the uniform convergence \eqref{eq: not_paralyzed_by_choice} represents in a game theoretic context. The uniformity in $n$ indicates that there is some common rate amongst all $n$ at which we can ensure $x_n(t) \to \overline{x}_n$ as $t\to\infty$. In other words, \eqref{eq: not_paralyzed_by_choice} characterizes the situation in which every finite-dimensional approximation converges to its associated equilibrium at some speed independent of the number of strategies available. This condition is in essence capturing the behavior of evolutionary games in which the players \emph{do not suffer from choice paralysis}, i.e., giving the players more strategies to choose from does not significantly slow down the overall dynamics of the game. From this perspective, the need for \eqref{eq: not_paralyzed_by_choice} should expected in order to guarantee the infinite-dimensional state $\mu(t)$ actually ``makes progress'' towards an equilibrium. On the contrary, if a population suffers from choice paralysis, it may be the case that, upon increasing the (finite) number of strategies available, the progression of the population state towards an equilibrium slows down; the more choices there are, the longer it takes players to figure out what they want to do. If the evolution rate of the population is slowed down enough (by the increase in choices) relative to the convergence rates toward equilibria at a fixed number of strategies, then convergence can no longer be guaranteed as the number of strategies grows towards infinity. Hence, stability guarantees for finite-dimensional approximations, e.g., via the dissipativity theory of \citet{arcak2021dissipativity}, may not suffice to guarantee stability for the infinite-dimensional game. This emphasizes the need for guarantees that directly consider infinite strategy sets, like ours developed in \autoref{sec: dissipativity_theory}.

	With the above interpretation of \eqref{eq: not_paralyzed_by_choice} in hand, we make the following definition.

	\begin{definition}
		\label{def: choice-mobile_trajectories}
		Consider a collection $\mathcal{X} = \{x_n: n\in\N\}$ of trajectories $x_n \colon [0,\infty) \to \Delta^{n-1}$ such that, for all $n\in\N$, there exists $\overline{x}_n \in\Delta^{n-1}$ such that $\lim_{t\to\infty} x_n(t) = \overline{x}_n$. The collection $\mathcal{X}$ is said to be \emph{choice-mobile} if
		\begin{equation*}
			\lim_{t\to\infty}\sup_{n\in\N}\|x_n(t) - \overline{x}_n\|_1 = 0.
		\end{equation*}
		The collection $\mathcal{X}$ is said to \emph{suffer from choice paralysis} if $\mathcal{X}$ is not choice-mobile.
	\end{definition}

	Certainly, the notions of choice-mobility and choice paralysis may be lifted to classes of finite-dimensional EDMs (with common payoff structure and common revision protocol) by considering the choice-mobility and choice paralysis of their generated trajectories. We then see that, under some technical conditions, \autoref{cor: finite_approx} asserts that stability is preserved when going from finite to infinite strategy sets whenever the trajectories generated by the finite-dimensional approximations are choice-mobile.

	In the following result, we show that one way that choice paralysis may occur is through decaying revision protocol values; paralysis occurs if the rate of strategy switching decreases towards zero as the number of strategies increases.

	\begin{propositionE}[][end,restate,text link=]
		\label{prop: choice_paralysis-decaying_switch_rate}
		Consider a game $F\colon \P(S) \to C_0(S)$, a revision protocol $\varphi \colon S \times S \times \P(S) \times C_0(S) \to \Rpl$. Let $s_i \in S$ for all $i\in\N$, and let $\theta_n,x_n(0)\in\Delta^{n-1}$ for all $n\in\N$. Suppose that, for all $n\in\N$, there exists a unique solution $x_n\colon [0,\infty) \to \Delta^{n-1}$ of the system \eqref{eq: n_ode} of finite-dimensional ordinary differential equations with $\lambda_n \coloneqq \sum_{i=1}^n (\theta_n)_i \delta_{s_i}$ and initial state $x_n(0)$. Also suppose that, for all $n\in\N$ it holds that $\lim_{t\to\infty}x_n(t) = \overline{x}_n$ for some $\overline{x}_n\in \Delta^{n-1}$. If there exists $\epsilon > 0$ and a sequence $\{M_n \in \Rpl : n\in\N\}$ such that $\lim_{n\to\infty}M_n = 0$ and, for all $n\in\N$, it holds that $\|x_n(0) - \overline{x}_n\|_1 > \epsilon$ and
		\begin{equation*}
			|\overline{\varphi}(i,j,\theta)| \le M_n
		\end{equation*}
		for all $i,j\in\{1,\dots,n\}$ and all $\theta\in\Delta^{n-1}$, then $\{x_n \colon n\in\N\}$ suffers from choice paralysis.
	\end{propositionE}

	\begin{proofE}
		Let $t\in[0,\infty)$ and let $n\in\N$. It holds that
		\begin{align*}
			\|x_n(t) - \overline{x}_n\|_1 &= \left\| \int_{[0,t]}\dot{x}_n(\tau) d\tau + x_n(0) - \overline{x}_n\right\|_1 \\
			&\ge \|x_n(0) - \overline{x}_n\|_1 - \left\| \int_{[0,t]} \dot{x}_n(\tau)d\tau\right\|_1 \\
			&\ge \|x_n(0) - \overline{x}_n\|_1 - \int_{[0,t]}\|\dot{x}_n(\tau)\|_1 d\tau.
		\end{align*}
		Therefore,
		\begin{align*}
			\limsup_{n\to\infty}\|x_n(0) - \overline{x}_n\|_1 &\le \limsup_{n\to\infty} \left(\|x_n(t) - \overline{x}_n\|_1 + \int_{[0,t]}\|\dot{x}_n(\tau)\|_1d\tau\right) \\
			&\le \limsup_{n\to\infty} \|x_n(t) - \overline{x}_n\|_1 + \limsup_{n\to\infty}\int_{[0,t]}\|\dot{x}_n(\tau)\|_1d\tau,
		\end{align*}
		implying that
		\begin{equation}
		\begin{aligned}
			\sup_{n\in\N}\|x_n(t) - \overline{x}_n\|_1 &\ge \limsup_{n\to\infty}\|x_n(t) - \overline{x}_n\|_1 \\
			&\ge \limsup_{n\to\infty}\|x_n(0) - \overline{x}_n\|_1 - \limsup_{n\to\infty} \int_{[0,t]}\|\dot{x}_n(\tau)\|_1 d\tau
		\end{aligned}
		\label{eq: choice_paralysis_proof}
		\end{equation}
		for all $t\in[0,\infty)$. Due to the assumed bound on $\overline{\varphi}$, \eqref{eq: n_ode} yields that
		\begin{equation*}
			|(\dot{x}_n(t))_i| \le M_n \lambda_n(s_i) \sum_{j=1}^n (x_n(t))_j + M_n (x_n(t))_i \sum_{j=1}^n \lambda_n(s_j) = M_n (\lambda_n(s_i) + (x_n(t))_i)
		\end{equation*}
		for all $n\in\N$, all $i\in\{1,\dots,n\}$, and all $t\in[0,\infty)$, and therefore
		\begin{equation*}
			\|\dot{x}_n(t)\|_1 = \sum_{i=1}^n|(\dot{x}_n(t))_i| \le M_n \sum_{i=1}^n\lambda_n(s_i) + M_n \sum_{i=1}^n (x_n(t))_i = 2M_n
		\end{equation*}
		for all $n\in\N$ and all $t\in[0,\infty)$. Therefore, \eqref{eq: choice_paralysis_proof} yields
		\begin{align*}
			\sup_{n\in\N} \|x_n(t) - \overline{x}_n\|_1 &\ge \limsup_{n\to\infty}\|x_n(0) - \overline{x}_n\|_1 - \limsup_{n\to\infty} \int_{[0,t]}2M_n d\tau \\
			&\ge \epsilon - \limsup_{n\to\infty} 2M_n t \\
			&= \epsilon
		\end{align*}
		for all $t\in[0,\infty)$. Thus, $\{x_n : n\in\N\}$ suffers from choice paralysis.
	\end{proofE}

	\hl{Note: Murat's circulant example for a deteriorating rate of convergence near replicator equilibria also works with the simpler payoff matrix $A=-I$. However, for both of these examples, we cannot necessarily say that the corresponding infinite game doesn't converge toward zero. The basin of attraction of the equilibria of the finite games may be decreasing, i.e., the deteriorating convergence rate of the linearization may only hold in a decreasingly small neighborhood, meaning the linearization doesn't actually say anything about the ``stopping'' of the infinite trajectories.}


==> tex/intro-old.tex <==
	\section{Introduction and Description of Main Results}
	\label{sec: description}

	In this section, we describe the problem and our results in a non-rigorous fashion. Consider an evolutionary game with strategies in some set $S$, and with payoffs defined by some function $F$, which encodes the payoff to each strategy when the game's population is at a certain state $\mu$. We are interested in an evolutionary dynamics model of the form
	\begin{equation}
		\dot{\mu}(t) = v(\mu(t),F(\mu(t))),
		\label{eq: edm-informal}
	\end{equation}
	which is a differential equation governing how the population state $\mu$ changes over time. The map $v$ may be viewed as the vector field describing the population's dynamics, which is dependent on the current state of the population as well as an ``input'' $F(\mu(t))$. In other words, the payoff function $F$ acts like a feedback controller, and steers the population dynamics according to how each strategy is currently paying off. \emph{The general problem at hand is to determine when this dynamics model converges to a Nash equilibrium of the game.}

	Inspired by \citet{arcak2021dissipativity}, we study the dynamic stability of this closed-loop system by independently studying properties of the system itself (i.e., the function $v$), and the control input (i.e., the payoff function $F$). The primary notion of interest is that of $\delta$-dissipative systems.

	\begin{definition}[Informal]
		\label{def: delta-dissipative-informal}
		The system $v$ is \emph{$\delta$-dissipative with supply rate $w$} if the rate of change of its internally stored energy is less than or equal to the energy supply rate $w$. If the rate of change in stored energy is strictly less than the energy supply rate $w$, then $v$ is \emph{strictly $\delta$-dissipative with supply rate $w$}.
	\end{definition}

	\autoref{def: delta-dissipative-informal} is made formal in \autoref{def: delta-dissipative}. Intuitively, if the energy supply rate is negative, then the energy supplied to the system is decreasing. Thus, if the supply rate remains negative, we expect the internal energy of a (strictly) $\delta$-dissipative system to decrease and for the state to converge to some ``lowest energy'' point, which is hopefully a Nash equilibrium. Our main result is that, under some technical stationarity, continuity, and differentiability conditions, this is indeed the case when the strategy set is compact and the payoff function $F$ induces negative supply rates along the system trajectories.

	\begin{theorem}[Main Result, Informal]
		\label{thm: delta-dissipative-informal}
		If the strategy set $S$ is compact, the system $v$ is $\delta$-dissipative with supply rate $w$, and the payoff function $F$ induces negative supply rates, then the set of Nash equilibria is dynamically stable under the evolutionary dynamics model \eqref{eq: edm-informal} under appropriate stationarity, continuity, and differentiability conditions. If, additionally, $v$ is strictly $\delta$-dissipative with supply rate $w$, then the set of Nash equilibria is asymptotically stable (also under under appropriate related technical conditions).
	\end{theorem}

	The payoff function $F$ inducing negative supply rates can be intuitively thought of as the energy imparted by the feedback controller never increasing along system trajectories.

	This write-up is organized as follows. In \autoref{sec: math_preliminaries}, we recall some mathematical definitions and results that are of use to us. Population games and evolutionary dynamics are formally introduced in \autoref{sec: population_games} and \autoref{sec: evolutionary_dynamics}, along with associated definitions and results for both static and dynamic stability. Our generalization of dissipativity theory to the infinite strategy set setting as well as our main result are presented in \autoref{sec: dissipativity_theory}. \iftoggle{proofs}{The proofs of all results that follow can be found in \autoref{sec: proofs}.}{Due to space constraints, we defer all proofs to our online technical report \citet{anderson2023dissipativity-long}.}


==> tex/to_do.tex <==
	\section{To Do}
	\label{sec: to_do}

	Here, we enumerate some ideas for future work.

	\begin{enumerate}
		\item BNN appears to converge to global optimizer of $s\mapsto \overline{f}(s)$ when using payoff defined by $f(s,s') = f(s) \pm f(s')$. Notice that this payoff is monotone, since integration against a measure in $T\P(S)$ twice will annihilate both terms. Can we perform guaranteed nonconvex optimization by running such BNN dynamics? Derive the theoretical guarantee for optimality by showing that global optima are equivalent to Nash, and that dynamics converge to Nash.
		\item In simulations, BNN converges to an interesting distribution for $f(s,s') = \sin(2\pi s s')$. Notice that this makes the game's average payoffs equal to the Fourier sign-transform under the measure $\mu$. What sort of game does this represent? It appears to not be monotone, despite its convergent behavior. Can we prove convergence another way? Study this specific game more deeply.
		\item The following approximation result may hold and be of interest: If $\{s_n : n\in\N\}$ is dense in $S$ and $\hat{F}_n$ is monotone for all $n$, then $F$ is monotone. This may be proved following the ideas in \href{https://math.stackexchange.com/questions/1310735/in-the-space-of-probability-distributions-is-the-set-of-discrete-distributions?noredirect=1&lq=1}{this link}. Similar results for preservation of Nash stationarity and passivity would be interesting.
		\item Replace ``overlines'' on $F$ and $\varphi$ in approximation theory section with ``hats'' (since we use ``overlines'' for extensions). Fix proofs.
		\item Add subscripts $n$ to $\overline{F}$ and $\overline{\varphi}$ (which should have ``hats'' after edits). Fix proofs.
		\item Do we use compactness of $S$ in our main approximation result? If not, re-word the statement at the beginning of the approximation section that says we assume compactness.
		\item Make explicit the dissipativity results in the context of approximation. Namely, show that asymptotic stability of Nash for finite games (e.g., by Murat's paper), yields weak asymptotic stability for infinite-dimensional games. Or, provide a counterexample.
	\end{enumerate}


==> tikzext/root-figure0-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable, and hence this is a sequential space. Therefore, $\P (S)$ is weakly closed if and only if it is weakly sequentially closed. It is clear that if $\{\mu _n \in \P (S) : n\in \N \}$ is a sequence in $\P (S)$ that weakly converges to $\mu \in \M (S)$, then $\mu \in \P (S)$ since it must be nonnegative and since the constant function $1$ is an element of $C(S)$. Hence, $\P (S)$ is weakly closed. By the Banach-Alaoglu theorem, the unit ball $\{\mu \in \M (S) : \|\mu \|_\TV \le 1\}$ is weak-$*$ compact and hence weakly compact as these two topologies coincide since $S$ is compact. Thus, the weakly closed subset $\P (S)$ of the weakly compact unit ball must also be weakly compact.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Let $\mu \in \P (S)$ be a NSS of the game $F\colon \P (S)\to C(S)$. Suppose that $h^F_{\nu :\mu }$ is right-continuous at $0$ for all $\nu \in \P (S)$. Let $\nu \in \P (S)$. Then, there exists $\epsilon (\nu )\in (0,1]$ such that \begin {equation*} h^F_{\nu :\mu }(\eta ) = E_F(\nu ,(1-\eta )\mu +\eta \nu ) - E_F(\mu ,(1-\eta )\mu +\eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,\epsilon (\nu )]$. Thus, by the right-continuity of $h^F_{\nu :\mu }$, it holds that \begin {equation*} E_F(\nu ,\mu )-E_F(\mu ,\mu ) = h^F_{\nu :\mu }(0) = \lim _{\eta \downarrow 0} h^F_{\nu :\mu }(\eta ) \le 0. \end {equation*} Since $\nu $ is arbitrary, this proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $\mu \in \P (S)$ is a GNSS of the game $F\colon \P (S)\to C(S)$. Let $\nu \in \P (S)$. Then, since $\mu $ is a GNSS of the game $F$, it holds that \begin {equation*} E_F((1-\eta )\mu +\eta \nu ,(1-\eta )\mu + \eta \nu ) - E_F(\mu ,(1-\eta )\mu +\eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,1]$. By linearity of $E_F$ in its first argument, we find that \begin {equation*} \eta E_F(\nu ,(1-\eta ) \mu + \eta \nu ) - \eta E_F(\mu ,(1-\eta ) \mu + \eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,1]$. Dividing by $\eta $ proves that $\mu $ is a NSS of the game $F$. The proof that $\mu $ being a GESS implies that $\mu $ is an ESS is identical as above with strict inqualities when considering $\nu \in \P (S)\setminus \{\mu \}$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Since $\mu $ is a GESS of the game $F$, it holds that $\mu $ is a NSS of the game $F$, and therefore $\mu \in \NE (F)$ by \autoref {prop: nss_implies_nash}, as $h^F_{\nu :\mu }$ is right-continuous at $0$. For all $\nu \in \P (S)\setminus \{\mu \}$, it holds that $E_F(\nu ,\nu ) < E(\mu ,\nu )$ since $\mu $ is a GESS of the game $F$, and therefore such $\nu $ are not Nash equilibria of the game $F$. This proves that indeed $\NE (F) = \{\mu \}$.\end{proof}

\prAtEndRestatevii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}It holds that $\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$. For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}Suppose that $\mu ([0,\infty ))\subseteq \P (S)$. Let $t\in (0,\infty )$. Since $\frac {\mu (t+\epsilon ) - \mu (t)}{\epsilon }$ converges strongly to $\dot {\mu }(t)$ as $\epsilon \to 0$, it also converges weakly to $\dot {\mu }(t)$ as $\epsilon \to 0$, so \begin {equation*} \lim _{\epsilon \to 0}\int _S f d \left (\frac {\mu (t+\epsilon ) - \mu (t)}{\epsilon }\right ) = \int _S f d\dot {\mu }(t) \end {equation*} for all $f\in C(S)$. In particular, taking $f$ to be the function that is identically $1$ on $S$ yields that \begin {equation*} \lim _{\epsilon \to 0} \frac {1}{\epsilon }\left (\mu (t+\epsilon )(S) - \mu (t)(S)\right ) = \dot {\mu }(t)(S). \end {equation*} Since $\mu (t)$ and $\mu (t+\epsilon )$ are probability measures for all $\epsilon \in [-t,\infty )$, it holds that $\mu (t+\epsilon )(S) = \mu (t)(S) = 1$ for all such $\epsilon $, and hence $\frac {1}{\epsilon }\left (\mu (t+\epsilon )(S) - \mu (t)(S)\right ) = 0$ for all $\epsilon \in [-t,\infty )\setminus \{0\}$. Therefore, it must be that \begin {equation*} \dot {\mu }(t)(S) = 0, \end {equation*} so indeed $\dot {\mu }(t) \in T\P (S)$. The case for $t=0$ follows similarly.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatexi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$. Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$ for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that $\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$, and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexii}\label{thm:prAtEndxii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}Since $v$ is $\delta $-dissipative with supply rate $w\colon \M (S) \times C(S) \to \R $, there exist $\sigma \colon \P (S) \times C(S) \to \Rpl $ and $\storage \colon \P (S) \times C(S) \to \Rpl $ with $\storage $ having an appropriate extension $\overline {\storage } \colon U\times C(S) \to \R $ as in \autoref {def: delta-dissipative}. Define $V \colon \P (S) \to \Rpl $ by $V(\mu ) = \storage (\mu ,F(\mu ))$. By \autoref {prop: ne_closed} and \autoref {prop: weakly_continuous_payoff}, $\NE (F)$ is weakly compact. Thus, by \autoref {lem: lyapunov}, it suffices to show that $V$ is a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ (according to \autoref {def: lyapunov_function}). Let $\overline {V}\colon U\cap U' \to \R $ be defined by $\overline {V}(\mu ) = \overline {\storage }(\mu ,\overline {F}(\mu ))$. Note that $U\cap U'$ is strongly open and contains $\P (S)$, and that $\overline {V}$ is weakly continuous and Fr\'echet differentiable since $\overline {\storage }$ is weak-$\infty $-continuous and $\overline {F}$ is weakly continuous, and both $\overline {\storage }$ and $\overline {F}$ are Fr\'echet differentiable. Also note that $\overline {V}(\mu ) = V(\mu )$ for all $\mu \in \P (S)$. Also, if $\mu \in \NE (F)$, then $v(\mu ,F(\mu )) = 0$ by \autoref {prop: ns_implies_rest_equals_nash}, and therefore $\overline {V}(\mu ) = V(\mu ) = \storage (\mu ,F(\mu )) = 0$ by \eqref {eq: delta-dissipative-2}. Furthermore, if $\mu \in \P (S)\setminus \NE (F)$, then again by \autoref {prop: ns_implies_rest_equals_nash} we have that $v(\mu ,F(\mu )) \ne 0$, so $\overline {V}(\mu ) = V(\mu ) = \storage (\mu ,F(\mu )) > 0$ by \eqref {eq: delta-dissipative-2}. Therefore, the first two conditions from \autoref {def: lyapunov_function} on $V$ to be a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ are satisfied. \par Next, since $\overline {\storage }$ and $\overline {F}$ are Fr\'echet differentiable, \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} for all $\mu \in U\cap U'$, and therefore, since $\overline {F}(\mu ) = F(\mu )$ for all $\mu \in \P (S)$, it holds for all $\mu \in \P (S)$ that \begin {equation} \begin {aligned} D\overline {V}(\mu )v(\mu ,F(\mu )) &= \partial _1 \overline {\storage }(\mu ,F(\mu )) v(\mu , F(\mu )) + \partial _2 \overline {\storage }(\mu ,F(\mu )) D\overline {F}(\mu ) v(\mu , F(\mu )) \\ &\le -\sigma (\mu ,F(\mu )) + w(v(\mu ,F(\mu )),D\overline {F}(\mu )v(\mu ,F(\mu ))) \\ &\le -\sigma (\mu ,F(\mu )) \\ &\le 0, \end {aligned} \label {eq: decreasing_derivative} \end {equation} where the first inequality follows from \eqref {eq: delta-dissipative-1}, and the second inequality follows from \eqref {eq: supply_inequality} together with the fact that $v(\mu ,F(\mu ))\in T\P (S)$. Hence, $V$ is indeed a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$, so $\NE (F)$ is weakly Lyapunov stable under the EDM \eqref {eq: edm}. \par Now suppose that the $\delta $-dissipativity of $v$ is strict and that the additional hypotheses of \autoref {ass: game_derivative} and \autoref {ass: dynamics_map} both hold. By \autoref {lem: strict_lyapunov}, it suffices to show that $V$ is a strict global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ (according to \autoref {def: lyapunov_function}). This amounts to proving that $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous and that $D\overline {V}(\mu )v(\mu ,F(\mu )) < 0$ for all $\mu \in \P (S)\setminus \NE (F)$. Indeed, the continuity condition holds by \autoref {lem: weakly_continuous_derivative}, which we proof after completing the current proof. \par Next, if $\mu \in \P (S)\setminus \NE (F)$, then \autoref {prop: ns_implies_rest_equals_nash} gives that $v(\mu ,F(\mu )) \ne 0$ so $\sigma (\mu ,F(\mu )) > 0$ by \eqref {eq: delta-dissipative-3}, implying that $D\overline {V}(\mu )v(\mu ,F(\mu )) < 0$ for all such $\mu $ by \eqref {eq: decreasing_derivative}. Hence, $V$ is indeed a strict global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$, so $\NE (F)$ is globally weakly attracting under the EDM \eqref {eq: edm}.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexiv}\label{thm:prAtEndxiv}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiv}]\phantomsection\label{proof:prAtEndxiv}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {align*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| &\le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {align*} }{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and also since $\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$ for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\quad + \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestatexv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxv}]\phantomsection\label{proof:prAtEndxv}Let $\mu \in \P (S)$ be a Nash equilibrium of the game $F$. Then $\int _S F_\mu d\nu \le \int _S F_\mu d\mu $ for all $\nu \in \P (S)$, so by monotonicity it holds that \begin {align*} E_F(\nu ,\nu ) - E_F(\mu ,\nu ) &= \int _S F_\nu d\nu - \int _S F_\nu d\mu \\ &= \int _S F_\mu (\nu -\mu ) + \int _S(F_\nu -F_\mu )d(\nu -\mu ) \\ &\le 0 \end {align*} for all $\nu \in \P (S)$. Hence, $\mu $ is a GNSS of the game $F$. It is clear that if $\mu $ is a strict Nash equilibrium or if $F$ is strictly monotone, then the above inequality becomes strict for $\nu \in \P (S)\setminus \{\mu \}$ and hence $\mu $ is a GESS of the game $F$ in these cases.\end{proof}

\prAtEndRestatexvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxvi}]\phantomsection\label{proof:prAtEndxvi}This follows directly from \autoref {prop: monotone_nash} together with \autoref {prop: unique_gess}.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexvii}\label{thm:prAtEndxvii}\label {lem: convex_stable_set} Consider a game $F\colon \P (S)\to C(S)$ and let $N\subseteq \P (S)$ be an arbitrary set of population states. Let $\stab _N^F \subseteq \P (S)$ denote the set of all population states $\mu \in \P (S)$ such that, for all $\nu \in N$, it holds that \begin {equation*} E_F(\nu ,\nu )\le E_F(\mu ,\nu ). \end {equation*} Then, it holds that $\stab _N^F$ is a convex set.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxvii}]\phantomsection\label{proof:prAtEndxvii}It holds that \begin {align*} \stab _N^F &= \{\mu \in \P (S) : \text {$E_F(\nu ,\nu ) \le E_F(\mu ,\nu )$ for all $\nu \in N$}\} \\ &= \bigcap _{\nu \in N} \{\mu \in \P (S) : E_F(\nu ,\nu ) \le E_F(\mu ,\nu )\}. \end {align*} Since $E_F$ is linear in its first argument, the set $\{\mu \in \P (S) : E_F(\nu ,\nu ) \le E_F(\mu ,\nu )\}$ is convex for all $\nu \in N$, and therefore the set $\stab _N^F$, being the intersection of convex sets, is also a convex set.\end{proof}

\prAtEndRestatexviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxviii}]\phantomsection\label{proof:prAtEndxviii}By \autoref {prop: monotone_nash}, every Nash equilibrium of the game $F$ is a GNSS of the game $F$, and by \autoref {prop: nss_implies_nash} every GNSS of the game $F$ is a Nash equilibrium of the game $F$. Hence, the set of Nash equilibria of the game $F$ equals the set of globally neutrally stable states of the game $F$, so $\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\nu ) \le E_F(\mu ,\nu )$ for all $\nu \in \P (S)$}\}$. Applying \autoref {lem: convex_stable_set} with $N = \P (S)$ proves the claim.\end{proof}

\prAtEndRestatexix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxix}]\phantomsection\label{proof:prAtEndxix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics.} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics.} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatexx*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxx}]\phantomsection\label{proof:prAtEndxx}Suppose that $v$ is Nash stationary, $v$ is $\delta $-passive, and $F$ is monotone. Let $w\colon \M (S) \times C(S) \to \R $ be defined by $w(\mu ,\eta ) = \left <\eta ,\mu \right >$. Then it holds that $v$ is $\delta $-dissipative with supply rate $w$. Furthermore, by \autoref {lem: monotone_sde}, $F$ satisfies self-defeating externalities, and therefore \begin {equation*} w(\nu ,D\overline {F}(\mu )\nu ) = \left <D\overline {F}(\mu )\nu ,\nu \right > \le 0 ~ \text {for all $\mu \in \P (S)$ and all $\nu \in T\P (S)$.} \end {equation*} Hence, by \autoref {thm: delta-dissipative}, it holds that $\NE (F)$ is weakly Lyapunov stable under the EDM \eqref {eq: edm}. The fact that $\NE (F)$ is globally weakly attracting under the EDM \eqref {eq: edm} given the additional hypotheses of \autoref {ass: game_derivative} and \autoref {ass: dynamics_map} is immediate from \autoref {thm: delta-dissipative}.\end{proof}

\prAtEndRestatexxi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxi}]\phantomsection\label{proof:prAtEndxxi}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\prAtEndRestatexxii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxii}]\phantomsection\label{proof:prAtEndxxii}Since $v$ is $\delta $-dissipative with supply rate $w\colon \M (S) \times C(S) \to \R $, there exist $\sigma \colon \P (S) \times C(S) \to \Rpl $ and $\storage \colon \P (S) \times C(S) \to \Rpl $ with $\storage $ having an appropriate extension $\overline {\storage } \colon U\times C(S) \to \R $ as in \autoref {def: delta-dissipative}. Furthermore, since $u$ is $\delta $-antidissipative with supply rate $\tilde {w}\colon \M (S) \times C(S) \to \R $, there exist $\gamma \colon \P (S) \times C(S) \to \Rpl $ and $\Gamma \colon \P (S) \times C(S) \to \Rpl $ with $\Gamma $ having an appropriate extension $\overline {\Gamma } \colon \tilde {U}\times C(S) \to \R $ as in \autoref {def: delta-antidissipative}. Define $V \colon \P (S)\times K \to \Rpl $ by $V(\mu ,\rho ) = \storage (\mu ,\rho ) + \Gamma (\mu ,\rho )$. Consider $P = \{(\mu ,\rho ) \in \P (S) \times C(S) : v(\mu ,\rho ) = 0, ~ u(\mu ,\rho ) = 0\}$. If $(\mu ,\rho ) \in P$, then $u(\mu ,\rho ) = 0$, implying that $\rho = F(\mu )$ by $F$-payoff stationarity, and hence $v(\mu ,F(\mu )) = 0$, so $\mu \in \NE (F)$ by Nash stationarity. Thus, $P \subseteq \NE (F) \times F(\NE (F)) \subseteq \P (S) \times K$. By \autoref {prop: ne_closed} and \autoref {prop: weakly_continuous_payoff}, $\NE (F)$ is weakly compact, and hence $F(\NE (F))$ is compact as $F$ is weakly continuous. Since $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain, and $u$ is weak-$\infty $-continuous, it holds that $P = v^{-1}(\{0\})\cap u^{-1}(\{0\})$ is weak-$\infty $-closed, and hence must be weak-$\infty $-compact as well as $\NE (F) \times F(\NE (F))$ is. Thus, by \autoref {lem: lyapunov}, it suffices to show that $V$ is a global Lyapunov function for $P$ under $(\mu ,\rho ) \mapsto (v(\mu ,\rho ),u(\mu ,\rho ))$ (according to \autoref {def: lyapunov_function}). Let $\overline {V}\colon U\cap \tilde {U} \times C(S) \to \R $ be defined by $\overline {V}(\mu ,\rho ) = \overline {\storage }(\mu ,\rho ) + \overline {\Gamma }(\mu ,\rho )$. Note that $U\cap \tilde {U}$ is strongly open and contains $\P (S)$, and that $\overline {V}$ is weak-$\infty $-continuous and Fr\'echet differentiable since $\overline {\storage }$ and $\overline {\Gamma }$ are. Also note that $\overline {V}(\mu ,\rho ) = V(\mu ,\rho )$ for all $(\mu ,\rho ) \in \P (S) \times K$. Also, if $(\mu ,\rho ) \in P$, then $v(\mu ,\rho ) = 0$ and $u(\mu ,\rho ) = 0$, so $\overline {V}(\mu ,\rho ) = 0$ by \eqref {eq: delta-dissipative-2} and \eqref {eq: delta-antidissipative-2}. Furthermore, if $(\mu ,\rho ) \in (\P (S) \times K) \setminus P$, then again by \eqref {eq: delta-dissipative-2} and \eqref {eq: delta-antidissipative-2} we have that $\overline {V}(\mu ,\rho ) > 0$. Therefore, the first two conditions from \autoref {def: lyapunov_function} on $V$ to be a global Lyapunov function for $P$ under $(v,u)$ are satisfied. \par Next, it holds for all $(\mu ,\rho ) \in \P (S) \times K$ that \begin {equation} \begin {aligned} D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) &= \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu , \rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) u(\mu , \rho ) + \partial _1 \overline {\Gamma }(\mu ,\rho ) v(\mu , \rho ) + \partial _2 \overline {\Gamma }(\mu ,\rho ) u(\mu , \rho ) \\ &\le -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),u(\mu ,\rho )) - \gamma (\mu ,\rho ) - \tilde {w}(v(\mu ,\rho ),u(\mu ,\rho )) \\ &\le -\sigma (\mu ,F(\mu )) - \gamma (\mu ,\rho ) \\ &\le 0, \end {aligned} \label {eq: decreasing_derivative-dpedm} \end {equation} where the first inequality follows from \eqref {eq: delta-dissipative-1} and \eqref {eq: delta-antidissipative-1}, and the second inequality follows from the fact that $\tilde {w} \ge w$. Hence, $V$ is indeed a global Lyapunov function for $P$ under $(v,u)$, so $P$ is weak-$\infty $-Lyapunov stable under the DPEDM \eqref {eq: dpedm}. \par Now suppose that the $\delta $-dissipativity of $v$ and the $\delta $-antidissipativity of $u$ are both strict, and that $v$ is $\|\cdot \|_\TV $-bounded on $\P (S)\times K$. By \autoref {lem: strict_lyapunov}, it suffices to show that $V$ is a strict global Lyapunov function for $P$ under $(\mu ,\rho )\mapsto (v(\mu ,\rho ),u(\mu ,\rho ))$ (according to \autoref {def: lyapunov_function}). This amounts to proving that $(\mu ,\rho ) \mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weak-$\infty $-continuous and that $D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) < 0$ for all $(\mu ,\rho )\in (\P (S) \times K)\setminus P$. Indeed, the continuity condition holds by \autoref {lem: weakly_continuous_derivative-dpedm}, which we proof after completing the current proof. \par Next, if $(\mu ,\rho )\in (\P (S)\times K)\setminus P$, then $v(\mu ,\rho ) \ne 0$ or $u(\mu ,\rho ) \ne 0$, so $\sigma (\mu ,\rho ) > 0$ or $\gamma (\mu ,\rho ) > 0$ by \eqref {eq: delta-dissipative-3} and \eqref {eq: delta-antidissipative-3}, implying that $D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) < 0$ for all such $(\mu ,\rho )$ by \eqref {eq: decreasing_derivative-dpedm}. Hence, $V$ is indeed a strict global Lyapunov function for $P$ under $(v,u)$, so $P$ is globally weak-$\infty $-attracting under the DPEDM \eqref {eq: dpedm} from $K$.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexxiii}\label{thm:prAtEndxxiii}\label {lem: weakly_continuous_derivative-dpedm} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxiii}]\phantomsection\label{proof:prAtEndxxiii}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexxiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxiv}]\phantomsection\label{proof:prAtEndxxiv}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexxv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxv}]\phantomsection\label{proof:prAtEndxxv}In this proof, we denote the indicator function on a set $A \subseteq \R $ by $\chi _A \colon \R \to \R $, where \begin {equation*} \chi _A(t) = \begin {aligned} \begin {cases} 1 & \text {if $t \in A$}, \\ 0 & \text {if $t \notin A$}. \end {cases} \end {aligned} \end {equation*} \par Let $\mu ,\nu \in \P (S)$. It holds that \begin {align*} & 2 \int _S \int _S \tilde {\Theta }(s-s') d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S \tilde {\Theta }(s-s') d(\mu -\nu )(s') d(\mu -\nu )(s) + \int _S \int _S \tilde {\Theta }(s'-s) d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S \left (\tilde {\Theta }(s-s') + \tilde {\Theta }(s'-s)\right ) d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S d(\mu -\nu )(s') d(\mu -\nu )(s) \\ & \qquad = ((\mu -\nu )(S))^2 \\ & \qquad =0, \end {align*} since $(\mu -\nu )(S) = \mu (S) - \nu (S) = 0$. Therefore, \begin {equation*} \int _S \int _S \tilde {\Theta }(s-s')d(\mu -\nu )(s')d(\mu -\nu )(s) = 0. \end {equation*} Next, we note that \begin {align*} \int _S \int _S \min \{s,s'\} d\mu (s') d\nu (s) &= \int _S \int _S \int _{[0,\min \{s,s'\}]} dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{t' \in \R : t' \le \min \{s,s'\}\}}(t) dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{t' \in \R : t'\le s\}}(t) \chi _{\{t'\in \R : t\le s'\}}(t) dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s) \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s') dt d\mu (s') d\nu (s) \\ &= \int _{[0,\infty )} \int _S \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s') d\mu (s')\int _S \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s) d\nu (s) dt \\ &= \int _{[0,\infty )} \mu (S \cap [t,\infty )) \nu (S\cap [t,\infty )) dt. \end {align*} Therefore, we find that \begin {align*} & \int _S \int _S \min \{s,s'\} d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _{[0,\infty )} \left (\mu (S\cap [t,\infty ))^2 - 2\mu (S\cap [t,\infty ))\nu (S\cap [t,\infty )) + \nu (S\cap [t,\infty ))^2\right ) dt \\ &\qquad = \int _{[0,\infty )} \left (\mu (S\cap [t,\infty )) - \nu (S\cap [t,\infty ))\right )^2 dt. \end {align*} Thus, overall, it holds that \begin {align*} \left <F(\mu ) - F(\nu ), \mu -\nu \right > &= \int _S(F_\mu (s) - F_\nu (s)) d(\mu -\nu )(s) \\ &= \int _S \int _S \tilde {f}(s,s') d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &= V\int _S \int _S \tilde {\Theta }(s-s')d(\mu -\nu )(s')d(\mu -\nu )(s) - \int _S \int _S \min \{s,s'\} d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &= -\int _{[0,\infty )} \left (\mu (S\cap [t,\infty )) - \nu (S\cap [t,\infty ))\right )^2 dt \\ &\le 0. \end {align*} Hence, $F$ is monotone.\end{proof}

\prAtEndRestatexxvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxvi}]\phantomsection\label{proof:prAtEndxxvi}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {prop: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-figure1-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable, and hence this is a sequential space. Therefore, $\P (S)$ is weakly closed if and only if it is weakly sequentially closed. It is clear that if $\{\mu _n \in \P (S) : n\in \N \}$ is a sequence in $\P (S)$ that weakly converges to $\mu \in \M (S)$, then $\mu \in \P (S)$ since it must be nonnegative and since the constant function $1$ is an element of $C(S)$. Hence, $\P (S)$ is weakly closed. By the Banach-Alaoglu theorem, the unit ball $\{\mu \in \M (S) : \|\mu \|_\TV \le 1\}$ is weak-$*$ compact and hence weakly compact as these two topologies coincide since $S$ is compact. Thus, the weakly closed subset $\P (S)$ of the weakly compact unit ball must also be weakly compact.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Let $\mu \in \P (S)$ be a NSS of the game $F\colon \P (S)\to C(S)$. Suppose that $h^F_{\nu :\mu }$ is right-continuous at $0$ for all $\nu \in \P (S)$. Let $\nu \in \P (S)$. Then, there exists $\epsilon (\nu )\in (0,1]$ such that \begin {equation*} h^F_{\nu :\mu }(\eta ) = E_F(\nu ,(1-\eta )\mu +\eta \nu ) - E_F(\mu ,(1-\eta )\mu +\eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,\epsilon (\nu )]$. Thus, by the right-continuity of $h^F_{\nu :\mu }$, it holds that \begin {equation*} E_F(\nu ,\mu )-E_F(\mu ,\mu ) = h^F_{\nu :\mu }(0) = \lim _{\eta \downarrow 0} h^F_{\nu :\mu }(\eta ) \le 0. \end {equation*} Since $\nu $ is arbitrary, this proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $\mu \in \P (S)$ is a GNSS of the game $F\colon \P (S)\to C(S)$. Let $\nu \in \P (S)$. Then, since $\mu $ is a GNSS of the game $F$, it holds that \begin {equation*} E_F((1-\eta )\mu +\eta \nu ,(1-\eta )\mu + \eta \nu ) - E_F(\mu ,(1-\eta )\mu +\eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,1]$. By linearity of $E_F$ in its first argument, we find that \begin {equation*} \eta E_F(\nu ,(1-\eta ) \mu + \eta \nu ) - \eta E_F(\mu ,(1-\eta ) \mu + \eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,1]$. Dividing by $\eta $ proves that $\mu $ is a NSS of the game $F$. The proof that $\mu $ being a GESS implies that $\mu $ is an ESS is identical as above with strict inqualities when considering $\nu \in \P (S)\setminus \{\mu \}$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Since $\mu $ is a GESS of the game $F$, it holds that $\mu $ is a NSS of the game $F$, and therefore $\mu \in \NE (F)$ by \autoref {prop: nss_implies_nash}, as $h^F_{\nu :\mu }$ is right-continuous at $0$. For all $\nu \in \P (S)\setminus \{\mu \}$, it holds that $E_F(\nu ,\nu ) < E(\mu ,\nu )$ since $\mu $ is a GESS of the game $F$, and therefore such $\nu $ are not Nash equilibria of the game $F$. This proves that indeed $\NE (F) = \{\mu \}$.\end{proof}

\prAtEndRestatevii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}It holds that $\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$. For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}Suppose that $\mu ([0,\infty ))\subseteq \P (S)$. Let $t\in (0,\infty )$. Since $\frac {\mu (t+\epsilon ) - \mu (t)}{\epsilon }$ converges strongly to $\dot {\mu }(t)$ as $\epsilon \to 0$, it also converges weakly to $\dot {\mu }(t)$ as $\epsilon \to 0$, so \begin {equation*} \lim _{\epsilon \to 0}\int _S f d \left (\frac {\mu (t+\epsilon ) - \mu (t)}{\epsilon }\right ) = \int _S f d\dot {\mu }(t) \end {equation*} for all $f\in C(S)$. In particular, taking $f$ to be the function that is identically $1$ on $S$ yields that \begin {equation*} \lim _{\epsilon \to 0} \frac {1}{\epsilon }\left (\mu (t+\epsilon )(S) - \mu (t)(S)\right ) = \dot {\mu }(t)(S). \end {equation*} Since $\mu (t)$ and $\mu (t+\epsilon )$ are probability measures for all $\epsilon \in [-t,\infty )$, it holds that $\mu (t+\epsilon )(S) = \mu (t)(S) = 1$ for all such $\epsilon $, and hence $\frac {1}{\epsilon }\left (\mu (t+\epsilon )(S) - \mu (t)(S)\right ) = 0$ for all $\epsilon \in [-t,\infty )\setminus \{0\}$. Therefore, it must be that \begin {equation*} \dot {\mu }(t)(S) = 0, \end {equation*} so indeed $\dot {\mu }(t) \in T\P (S)$. The case for $t=0$ follows similarly.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatexi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$. Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$ for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that $\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$, and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexii}\label{thm:prAtEndxii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}Since $v$ is $\delta $-dissipative with supply rate $w\colon \M (S) \times C(S) \to \R $, there exist $\sigma \colon \P (S) \times C(S) \to \Rpl $ and $\storage \colon \P (S) \times C(S) \to \Rpl $ with $\storage $ having an appropriate extension $\overline {\storage } \colon U\times C(S) \to \R $ as in \autoref {def: delta-dissipative}. Define $V \colon \P (S) \to \Rpl $ by $V(\mu ) = \storage (\mu ,F(\mu ))$. By \autoref {prop: ne_closed} and \autoref {prop: weakly_continuous_payoff}, $\NE (F)$ is weakly compact. Thus, by \autoref {lem: lyapunov}, it suffices to show that $V$ is a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ (according to \autoref {def: lyapunov_function}). Let $\overline {V}\colon U\cap U' \to \R $ be defined by $\overline {V}(\mu ) = \overline {\storage }(\mu ,\overline {F}(\mu ))$. Note that $U\cap U'$ is strongly open and contains $\P (S)$, and that $\overline {V}$ is weakly continuous and Fr\'echet differentiable since $\overline {\storage }$ is weak-$\infty $-continuous and $\overline {F}$ is weakly continuous, and both $\overline {\storage }$ and $\overline {F}$ are Fr\'echet differentiable. Also note that $\overline {V}(\mu ) = V(\mu )$ for all $\mu \in \P (S)$. Also, if $\mu \in \NE (F)$, then $v(\mu ,F(\mu )) = 0$ by \autoref {prop: ns_implies_rest_equals_nash}, and therefore $\overline {V}(\mu ) = V(\mu ) = \storage (\mu ,F(\mu )) = 0$ by \eqref {eq: delta-dissipative-2}. Furthermore, if $\mu \in \P (S)\setminus \NE (F)$, then again by \autoref {prop: ns_implies_rest_equals_nash} we have that $v(\mu ,F(\mu )) \ne 0$, so $\overline {V}(\mu ) = V(\mu ) = \storage (\mu ,F(\mu )) > 0$ by \eqref {eq: delta-dissipative-2}. Therefore, the first two conditions from \autoref {def: lyapunov_function} on $V$ to be a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ are satisfied. \par Next, since $\overline {\storage }$ and $\overline {F}$ are Fr\'echet differentiable, \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} for all $\mu \in U\cap U'$, and therefore, since $\overline {F}(\mu ) = F(\mu )$ for all $\mu \in \P (S)$, it holds for all $\mu \in \P (S)$ that \begin {equation} \begin {aligned} D\overline {V}(\mu )v(\mu ,F(\mu )) &= \partial _1 \overline {\storage }(\mu ,F(\mu )) v(\mu , F(\mu )) + \partial _2 \overline {\storage }(\mu ,F(\mu )) D\overline {F}(\mu ) v(\mu , F(\mu )) \\ &\le -\sigma (\mu ,F(\mu )) + w(v(\mu ,F(\mu )),D\overline {F}(\mu )v(\mu ,F(\mu ))) \\ &\le -\sigma (\mu ,F(\mu )) \\ &\le 0, \end {aligned} \label {eq: decreasing_derivative} \end {equation} where the first inequality follows from \eqref {eq: delta-dissipative-1}, and the second inequality follows from \eqref {eq: supply_inequality} together with the fact that $v(\mu ,F(\mu ))\in T\P (S)$. Hence, $V$ is indeed a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$, so $\NE (F)$ is weakly Lyapunov stable under the EDM \eqref {eq: edm}. \par Now suppose that the $\delta $-dissipativity of $v$ is strict and that the additional hypotheses of \autoref {ass: game_derivative} and \autoref {ass: dynamics_map} both hold. By \autoref {lem: strict_lyapunov}, it suffices to show that $V$ is a strict global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ (according to \autoref {def: lyapunov_function}). This amounts to proving that $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous and that $D\overline {V}(\mu )v(\mu ,F(\mu )) < 0$ for all $\mu \in \P (S)\setminus \NE (F)$. Indeed, the continuity condition holds by \autoref {lem: weakly_continuous_derivative}, which we proof after completing the current proof. \par Next, if $\mu \in \P (S)\setminus \NE (F)$, then \autoref {prop: ns_implies_rest_equals_nash} gives that $v(\mu ,F(\mu )) \ne 0$ so $\sigma (\mu ,F(\mu )) > 0$ by \eqref {eq: delta-dissipative-3}, implying that $D\overline {V}(\mu )v(\mu ,F(\mu )) < 0$ for all such $\mu $ by \eqref {eq: decreasing_derivative}. Hence, $V$ is indeed a strict global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$, so $\NE (F)$ is globally weakly attracting under the EDM \eqref {eq: edm}.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexiv}\label{thm:prAtEndxiv}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiv}]\phantomsection\label{proof:prAtEndxiv}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {align*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| &\le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {align*} }{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and also since $\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$ for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\quad + \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestatexv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxv}]\phantomsection\label{proof:prAtEndxv}Let $\mu \in \P (S)$ be a Nash equilibrium of the game $F$. Then $\int _S F_\mu d\nu \le \int _S F_\mu d\mu $ for all $\nu \in \P (S)$, so by monotonicity it holds that \begin {align*} E_F(\nu ,\nu ) - E_F(\mu ,\nu ) &= \int _S F_\nu d\nu - \int _S F_\nu d\mu \\ &= \int _S F_\mu (\nu -\mu ) + \int _S(F_\nu -F_\mu )d(\nu -\mu ) \\ &\le 0 \end {align*} for all $\nu \in \P (S)$. Hence, $\mu $ is a GNSS of the game $F$. It is clear that if $\mu $ is a strict Nash equilibrium or if $F$ is strictly monotone, then the above inequality becomes strict for $\nu \in \P (S)\setminus \{\mu \}$ and hence $\mu $ is a GESS of the game $F$ in these cases.\end{proof}

\prAtEndRestatexvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxvi}]\phantomsection\label{proof:prAtEndxvi}This follows directly from \autoref {prop: monotone_nash} together with \autoref {prop: unique_gess}.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexvii}\label{thm:prAtEndxvii}\label {lem: convex_stable_set} Consider a game $F\colon \P (S)\to C(S)$ and let $N\subseteq \P (S)$ be an arbitrary set of population states. Let $\stab _N^F \subseteq \P (S)$ denote the set of all population states $\mu \in \P (S)$ such that, for all $\nu \in N$, it holds that \begin {equation*} E_F(\nu ,\nu )\le E_F(\mu ,\nu ). \end {equation*} Then, it holds that $\stab _N^F$ is a convex set.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxvii}]\phantomsection\label{proof:prAtEndxvii}It holds that \begin {align*} \stab _N^F &= \{\mu \in \P (S) : \text {$E_F(\nu ,\nu ) \le E_F(\mu ,\nu )$ for all $\nu \in N$}\} \\ &= \bigcap _{\nu \in N} \{\mu \in \P (S) : E_F(\nu ,\nu ) \le E_F(\mu ,\nu )\}. \end {align*} Since $E_F$ is linear in its first argument, the set $\{\mu \in \P (S) : E_F(\nu ,\nu ) \le E_F(\mu ,\nu )\}$ is convex for all $\nu \in N$, and therefore the set $\stab _N^F$, being the intersection of convex sets, is also a convex set.\end{proof}

\prAtEndRestatexviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxviii}]\phantomsection\label{proof:prAtEndxviii}By \autoref {prop: monotone_nash}, every Nash equilibrium of the game $F$ is a GNSS of the game $F$, and by \autoref {prop: nss_implies_nash} every GNSS of the game $F$ is a Nash equilibrium of the game $F$. Hence, the set of Nash equilibria of the game $F$ equals the set of globally neutrally stable states of the game $F$, so $\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\nu ) \le E_F(\mu ,\nu )$ for all $\nu \in \P (S)$}\}$. Applying \autoref {lem: convex_stable_set} with $N = \P (S)$ proves the claim.\end{proof}

\prAtEndRestatexix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxix}]\phantomsection\label{proof:prAtEndxix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics.} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics.} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatexx*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxx}]\phantomsection\label{proof:prAtEndxx}Suppose that $v$ is Nash stationary, $v$ is $\delta $-passive, and $F$ is monotone. Let $w\colon \M (S) \times C(S) \to \R $ be defined by $w(\mu ,\eta ) = \left <\eta ,\mu \right >$. Then it holds that $v$ is $\delta $-dissipative with supply rate $w$. Furthermore, by \autoref {lem: monotone_sde}, $F$ satisfies self-defeating externalities, and therefore \begin {equation*} w(\nu ,D\overline {F}(\mu )\nu ) = \left <D\overline {F}(\mu )\nu ,\nu \right > \le 0 ~ \text {for all $\mu \in \P (S)$ and all $\nu \in T\P (S)$.} \end {equation*} Hence, by \autoref {thm: delta-dissipative}, it holds that $\NE (F)$ is weakly Lyapunov stable under the EDM \eqref {eq: edm}. The fact that $\NE (F)$ is globally weakly attracting under the EDM \eqref {eq: edm} given the additional hypotheses of \autoref {ass: game_derivative} and \autoref {ass: dynamics_map} is immediate from \autoref {thm: delta-dissipative}.\end{proof}

\prAtEndRestatexxi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxi}]\phantomsection\label{proof:prAtEndxxi}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\prAtEndRestatexxii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxii}]\phantomsection\label{proof:prAtEndxxii}Since $v$ is $\delta $-dissipative with supply rate $w\colon \M (S) \times C(S) \to \R $, there exist $\sigma \colon \P (S) \times C(S) \to \Rpl $ and $\storage \colon \P (S) \times C(S) \to \Rpl $ with $\storage $ having an appropriate extension $\overline {\storage } \colon U\times C(S) \to \R $ as in \autoref {def: delta-dissipative}. Furthermore, since $u$ is $\delta $-antidissipative with supply rate $\tilde {w}\colon \M (S) \times C(S) \to \R $, there exist $\gamma \colon \P (S) \times C(S) \to \Rpl $ and $\Gamma \colon \P (S) \times C(S) \to \Rpl $ with $\Gamma $ having an appropriate extension $\overline {\Gamma } \colon \tilde {U}\times C(S) \to \R $ as in \autoref {def: delta-antidissipative}. Define $V \colon \P (S)\times K \to \Rpl $ by $V(\mu ,\rho ) = \storage (\mu ,\rho ) + \Gamma (\mu ,\rho )$. Consider $P = \{(\mu ,\rho ) \in \P (S) \times C(S) : v(\mu ,\rho ) = 0, ~ u(\mu ,\rho ) = 0\}$. If $(\mu ,\rho ) \in P$, then $u(\mu ,\rho ) = 0$, implying that $\rho = F(\mu )$ by $F$-payoff stationarity, and hence $v(\mu ,F(\mu )) = 0$, so $\mu \in \NE (F)$ by Nash stationarity. Thus, $P \subseteq \NE (F) \times F(\NE (F)) \subseteq \P (S) \times K$. By \autoref {prop: ne_closed} and \autoref {prop: weakly_continuous_payoff}, $\NE (F)$ is weakly compact, and hence $F(\NE (F))$ is compact as $F$ is weakly continuous. Since $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain, and $u$ is weak-$\infty $-continuous, it holds that $P = v^{-1}(\{0\})\cap u^{-1}(\{0\})$ is weak-$\infty $-closed, and hence must be weak-$\infty $-compact as well as $\NE (F) \times F(\NE (F))$ is. Thus, by \autoref {lem: lyapunov}, it suffices to show that $V$ is a global Lyapunov function for $P$ under $(\mu ,\rho ) \mapsto (v(\mu ,\rho ),u(\mu ,\rho ))$ (according to \autoref {def: lyapunov_function}). Let $\overline {V}\colon U\cap \tilde {U} \times C(S) \to \R $ be defined by $\overline {V}(\mu ,\rho ) = \overline {\storage }(\mu ,\rho ) + \overline {\Gamma }(\mu ,\rho )$. Note that $U\cap \tilde {U}$ is strongly open and contains $\P (S)$, and that $\overline {V}$ is weak-$\infty $-continuous and Fr\'echet differentiable since $\overline {\storage }$ and $\overline {\Gamma }$ are. Also note that $\overline {V}(\mu ,\rho ) = V(\mu ,\rho )$ for all $(\mu ,\rho ) \in \P (S) \times K$. Also, if $(\mu ,\rho ) \in P$, then $v(\mu ,\rho ) = 0$ and $u(\mu ,\rho ) = 0$, so $\overline {V}(\mu ,\rho ) = 0$ by \eqref {eq: delta-dissipative-2} and \eqref {eq: delta-antidissipative-2}. Furthermore, if $(\mu ,\rho ) \in (\P (S) \times K) \setminus P$, then again by \eqref {eq: delta-dissipative-2} and \eqref {eq: delta-antidissipative-2} we have that $\overline {V}(\mu ,\rho ) > 0$. Therefore, the first two conditions from \autoref {def: lyapunov_function} on $V$ to be a global Lyapunov function for $P$ under $(v,u)$ are satisfied. \par Next, it holds for all $(\mu ,\rho ) \in \P (S) \times K$ that \begin {equation} \begin {aligned} D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) &= \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu , \rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) u(\mu , \rho ) + \partial _1 \overline {\Gamma }(\mu ,\rho ) v(\mu , \rho ) + \partial _2 \overline {\Gamma }(\mu ,\rho ) u(\mu , \rho ) \\ &\le -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),u(\mu ,\rho )) - \gamma (\mu ,\rho ) - \tilde {w}(v(\mu ,\rho ),u(\mu ,\rho )) \\ &\le -\sigma (\mu ,F(\mu )) - \gamma (\mu ,\rho ) \\ &\le 0, \end {aligned} \label {eq: decreasing_derivative-dpedm} \end {equation} where the first inequality follows from \eqref {eq: delta-dissipative-1} and \eqref {eq: delta-antidissipative-1}, and the second inequality follows from the fact that $\tilde {w} \ge w$. Hence, $V$ is indeed a global Lyapunov function for $P$ under $(v,u)$, so $P$ is weak-$\infty $-Lyapunov stable under the DPEDM \eqref {eq: dpedm}. \par Now suppose that the $\delta $-dissipativity of $v$ and the $\delta $-antidissipativity of $u$ are both strict, and that $v$ is $\|\cdot \|_\TV $-bounded on $\P (S)\times K$. By \autoref {lem: strict_lyapunov}, it suffices to show that $V$ is a strict global Lyapunov function for $P$ under $(\mu ,\rho )\mapsto (v(\mu ,\rho ),u(\mu ,\rho ))$ (according to \autoref {def: lyapunov_function}). This amounts to proving that $(\mu ,\rho ) \mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weak-$\infty $-continuous and that $D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) < 0$ for all $(\mu ,\rho )\in (\P (S) \times K)\setminus P$. Indeed, the continuity condition holds by \autoref {lem: weakly_continuous_derivative-dpedm}, which we proof after completing the current proof. \par Next, if $(\mu ,\rho )\in (\P (S)\times K)\setminus P$, then $v(\mu ,\rho ) \ne 0$ or $u(\mu ,\rho ) \ne 0$, so $\sigma (\mu ,\rho ) > 0$ or $\gamma (\mu ,\rho ) > 0$ by \eqref {eq: delta-dissipative-3} and \eqref {eq: delta-antidissipative-3}, implying that $D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) < 0$ for all such $(\mu ,\rho )$ by \eqref {eq: decreasing_derivative-dpedm}. Hence, $V$ is indeed a strict global Lyapunov function for $P$ under $(v,u)$, so $P$ is globally weak-$\infty $-attracting under the DPEDM \eqref {eq: dpedm} from $K$.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexxiii}\label{thm:prAtEndxxiii}\label {lem: weakly_continuous_derivative-dpedm} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxiii}]\phantomsection\label{proof:prAtEndxxiii}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexxiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxiv}]\phantomsection\label{proof:prAtEndxxiv}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexxv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxv}]\phantomsection\label{proof:prAtEndxxv}In this proof, we denote the indicator function on a set $A \subseteq \R $ by $\chi _A \colon \R \to \R $, where \begin {equation*} \chi _A(t) = \begin {aligned} \begin {cases} 1 & \text {if $t \in A$}, \\ 0 & \text {if $t \notin A$}. \end {cases} \end {aligned} \end {equation*} \par Let $\mu ,\nu \in \P (S)$. It holds that \begin {align*} & 2 \int _S \int _S \tilde {\Theta }(s-s') d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S \tilde {\Theta }(s-s') d(\mu -\nu )(s') d(\mu -\nu )(s) + \int _S \int _S \tilde {\Theta }(s'-s) d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S \left (\tilde {\Theta }(s-s') + \tilde {\Theta }(s'-s)\right ) d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S d(\mu -\nu )(s') d(\mu -\nu )(s) \\ & \qquad = ((\mu -\nu )(S))^2 \\ & \qquad =0, \end {align*} since $(\mu -\nu )(S) = \mu (S) - \nu (S) = 0$. Therefore, \begin {equation*} \int _S \int _S \tilde {\Theta }(s-s')d(\mu -\nu )(s')d(\mu -\nu )(s) = 0. \end {equation*} Next, we note that \begin {align*} \int _S \int _S \min \{s,s'\} d\mu (s') d\nu (s) &= \int _S \int _S \int _{[0,\min \{s,s'\}]} dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{t' \in \R : t' \le \min \{s,s'\}\}}(t) dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{t' \in \R : t'\le s\}}(t) \chi _{\{t'\in \R : t\le s'\}}(t) dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s) \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s') dt d\mu (s') d\nu (s) \\ &= \int _{[0,\infty )} \int _S \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s') d\mu (s')\int _S \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s) d\nu (s) dt \\ &= \int _{[0,\infty )} \mu (S \cap [t,\infty )) \nu (S\cap [t,\infty )) dt. \end {align*} Therefore, we find that \begin {align*} & \int _S \int _S \min \{s,s'\} d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _{[0,\infty )} \left (\mu (S\cap [t,\infty ))^2 - 2\mu (S\cap [t,\infty ))\nu (S\cap [t,\infty )) + \nu (S\cap [t,\infty ))^2\right ) dt \\ &\qquad = \int _{[0,\infty )} \left (\mu (S\cap [t,\infty )) - \nu (S\cap [t,\infty ))\right )^2 dt. \end {align*} Thus, overall, it holds that \begin {align*} \left <F(\mu ) - F(\nu ), \mu -\nu \right > &= \int _S(F_\mu (s) - F_\nu (s)) d(\mu -\nu )(s) \\ &= \int _S \int _S \tilde {f}(s,s') d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &= V\int _S \int _S \tilde {\Theta }(s-s')d(\mu -\nu )(s')d(\mu -\nu )(s) - \int _S \int _S \min \{s,s'\} d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &= -\int _{[0,\infty )} \left (\mu (S\cap [t,\infty )) - \nu (S\cap [t,\infty ))\right )^2 dt \\ &\le 0. \end {align*} Hence, $F$ is monotone.\end{proof}

\prAtEndRestatexxvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxvi}]\phantomsection\label{proof:prAtEndxxvi}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {prop: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-figure2-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable, and hence this is a sequential space. Therefore, $\P (S)$ is weakly closed if and only if it is weakly sequentially closed. It is clear that if $\{\mu _n \in \P (S) : n\in \N \}$ is a sequence in $\P (S)$ that weakly converges to $\mu \in \M (S)$, then $\mu \in \P (S)$ since it must be nonnegative and since the constant function $1$ is an element of $C(S)$. Hence, $\P (S)$ is weakly closed. By the Banach-Alaoglu theorem, the unit ball $\{\mu \in \M (S) : \|\mu \|_\TV \le 1\}$ is weak-$*$ compact and hence weakly compact as these two topologies coincide since $S$ is compact. Thus, the weakly closed subset $\P (S)$ of the weakly compact unit ball must also be weakly compact.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Let $\mu \in \P (S)$ be a NSS of the game $F\colon \P (S)\to C(S)$. Suppose that $h^F_{\nu :\mu }$ is right-continuous at $0$ for all $\nu \in \P (S)$. Let $\nu \in \P (S)$. Then, there exists $\epsilon (\nu )\in (0,1]$ such that \begin {equation*} h^F_{\nu :\mu }(\eta ) = E_F(\nu ,(1-\eta )\mu +\eta \nu ) - E_F(\mu ,(1-\eta )\mu +\eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,\epsilon (\nu )]$. Thus, by the right-continuity of $h^F_{\nu :\mu }$, it holds that \begin {equation*} E_F(\nu ,\mu )-E_F(\mu ,\mu ) = h^F_{\nu :\mu }(0) = \lim _{\eta \downarrow 0} h^F_{\nu :\mu }(\eta ) \le 0. \end {equation*} Since $\nu $ is arbitrary, this proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $\mu \in \P (S)$ is a GNSS of the game $F\colon \P (S)\to C(S)$. Let $\nu \in \P (S)$. Then, since $\mu $ is a GNSS of the game $F$, it holds that \begin {equation*} E_F((1-\eta )\mu +\eta \nu ,(1-\eta )\mu + \eta \nu ) - E_F(\mu ,(1-\eta )\mu +\eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,1]$. By linearity of $E_F$ in its first argument, we find that \begin {equation*} \eta E_F(\nu ,(1-\eta ) \mu + \eta \nu ) - \eta E_F(\mu ,(1-\eta ) \mu + \eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,1]$. Dividing by $\eta $ proves that $\mu $ is a NSS of the game $F$. The proof that $\mu $ being a GESS implies that $\mu $ is an ESS is identical as above with strict inqualities when considering $\nu \in \P (S)\setminus \{\mu \}$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Since $\mu $ is a GESS of the game $F$, it holds that $\mu $ is a NSS of the game $F$, and therefore $\mu \in \NE (F)$ by \autoref {prop: nss_implies_nash}, as $h^F_{\nu :\mu }$ is right-continuous at $0$. For all $\nu \in \P (S)\setminus \{\mu \}$, it holds that $E_F(\nu ,\nu ) < E(\mu ,\nu )$ since $\mu $ is a GESS of the game $F$, and therefore such $\nu $ are not Nash equilibria of the game $F$. This proves that indeed $\NE (F) = \{\mu \}$.\end{proof}

\prAtEndRestatevii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}It holds that $\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$. For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}Suppose that $\mu ([0,\infty ))\subseteq \P (S)$. Let $t\in (0,\infty )$. Since $\frac {\mu (t+\epsilon ) - \mu (t)}{\epsilon }$ converges strongly to $\dot {\mu }(t)$ as $\epsilon \to 0$, it also converges weakly to $\dot {\mu }(t)$ as $\epsilon \to 0$, so \begin {equation*} \lim _{\epsilon \to 0}\int _S f d \left (\frac {\mu (t+\epsilon ) - \mu (t)}{\epsilon }\right ) = \int _S f d\dot {\mu }(t) \end {equation*} for all $f\in C(S)$. In particular, taking $f$ to be the function that is identically $1$ on $S$ yields that \begin {equation*} \lim _{\epsilon \to 0} \frac {1}{\epsilon }\left (\mu (t+\epsilon )(S) - \mu (t)(S)\right ) = \dot {\mu }(t)(S). \end {equation*} Since $\mu (t)$ and $\mu (t+\epsilon )$ are probability measures for all $\epsilon \in [-t,\infty )$, it holds that $\mu (t+\epsilon )(S) = \mu (t)(S) = 1$ for all such $\epsilon $, and hence $\frac {1}{\epsilon }\left (\mu (t+\epsilon )(S) - \mu (t)(S)\right ) = 0$ for all $\epsilon \in [-t,\infty )\setminus \{0\}$. Therefore, it must be that \begin {equation*} \dot {\mu }(t)(S) = 0, \end {equation*} so indeed $\dot {\mu }(t) \in T\P (S)$. The case for $t=0$ follows similarly.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatexi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$. Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$ for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that $\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$, and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexii}\label{thm:prAtEndxii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}Since $v$ is $\delta $-dissipative with supply rate $w\colon \M (S) \times C(S) \to \R $, there exist $\sigma \colon \P (S) \times C(S) \to \Rpl $ and $\storage \colon \P (S) \times C(S) \to \Rpl $ with $\storage $ having an appropriate extension $\overline {\storage } \colon U\times C(S) \to \R $ as in \autoref {def: delta-dissipative}. Define $V \colon \P (S) \to \Rpl $ by $V(\mu ) = \storage (\mu ,F(\mu ))$. By \autoref {prop: ne_closed} and \autoref {prop: weakly_continuous_payoff}, $\NE (F)$ is weakly compact. Thus, by \autoref {lem: lyapunov}, it suffices to show that $V$ is a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ (according to \autoref {def: lyapunov_function}). Let $\overline {V}\colon U\cap U' \to \R $ be defined by $\overline {V}(\mu ) = \overline {\storage }(\mu ,\overline {F}(\mu ))$. Note that $U\cap U'$ is strongly open and contains $\P (S)$, and that $\overline {V}$ is weakly continuous and Fr\'echet differentiable since $\overline {\storage }$ is weak-$\infty $-continuous and $\overline {F}$ is weakly continuous, and both $\overline {\storage }$ and $\overline {F}$ are Fr\'echet differentiable. Also note that $\overline {V}(\mu ) = V(\mu )$ for all $\mu \in \P (S)$. Also, if $\mu \in \NE (F)$, then $v(\mu ,F(\mu )) = 0$ by \autoref {prop: ns_implies_rest_equals_nash}, and therefore $\overline {V}(\mu ) = V(\mu ) = \storage (\mu ,F(\mu )) = 0$ by \eqref {eq: delta-dissipative-2}. Furthermore, if $\mu \in \P (S)\setminus \NE (F)$, then again by \autoref {prop: ns_implies_rest_equals_nash} we have that $v(\mu ,F(\mu )) \ne 0$, so $\overline {V}(\mu ) = V(\mu ) = \storage (\mu ,F(\mu )) > 0$ by \eqref {eq: delta-dissipative-2}. Therefore, the first two conditions from \autoref {def: lyapunov_function} on $V$ to be a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ are satisfied. \par Next, since $\overline {\storage }$ and $\overline {F}$ are Fr\'echet differentiable, \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} for all $\mu \in U\cap U'$, and therefore, since $\overline {F}(\mu ) = F(\mu )$ for all $\mu \in \P (S)$, it holds for all $\mu \in \P (S)$ that \begin {equation} \begin {aligned} D\overline {V}(\mu )v(\mu ,F(\mu )) &= \partial _1 \overline {\storage }(\mu ,F(\mu )) v(\mu , F(\mu )) + \partial _2 \overline {\storage }(\mu ,F(\mu )) D\overline {F}(\mu ) v(\mu , F(\mu )) \\ &\le -\sigma (\mu ,F(\mu )) + w(v(\mu ,F(\mu )),D\overline {F}(\mu )v(\mu ,F(\mu ))) \\ &\le -\sigma (\mu ,F(\mu )) \\ &\le 0, \end {aligned} \label {eq: decreasing_derivative} \end {equation} where the first inequality follows from \eqref {eq: delta-dissipative-1}, and the second inequality follows from \eqref {eq: supply_inequality} together with the fact that $v(\mu ,F(\mu ))\in T\P (S)$. Hence, $V$ is indeed a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$, so $\NE (F)$ is weakly Lyapunov stable under the EDM \eqref {eq: edm}. \par Now suppose that the $\delta $-dissipativity of $v$ is strict and that the additional hypotheses of \autoref {ass: game_derivative} and \autoref {ass: dynamics_map} both hold. By \autoref {lem: strict_lyapunov}, it suffices to show that $V$ is a strict global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ (according to \autoref {def: lyapunov_function}). This amounts to proving that $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous and that $D\overline {V}(\mu )v(\mu ,F(\mu )) < 0$ for all $\mu \in \P (S)\setminus \NE (F)$. Indeed, the continuity condition holds by \autoref {lem: weakly_continuous_derivative}, which we proof after completing the current proof. \par Next, if $\mu \in \P (S)\setminus \NE (F)$, then \autoref {prop: ns_implies_rest_equals_nash} gives that $v(\mu ,F(\mu )) \ne 0$ so $\sigma (\mu ,F(\mu )) > 0$ by \eqref {eq: delta-dissipative-3}, implying that $D\overline {V}(\mu )v(\mu ,F(\mu )) < 0$ for all such $\mu $ by \eqref {eq: decreasing_derivative}. Hence, $V$ is indeed a strict global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$, so $\NE (F)$ is globally weakly attracting under the EDM \eqref {eq: edm}.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexiv}\label{thm:prAtEndxiv}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiv}]\phantomsection\label{proof:prAtEndxiv}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {align*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| &\le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {align*} }{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and also since $\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$ for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\quad + \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestatexv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxv}]\phantomsection\label{proof:prAtEndxv}Let $\mu \in \P (S)$ be a Nash equilibrium of the game $F$. Then $\int _S F_\mu d\nu \le \int _S F_\mu d\mu $ for all $\nu \in \P (S)$, so by monotonicity it holds that \begin {align*} E_F(\nu ,\nu ) - E_F(\mu ,\nu ) &= \int _S F_\nu d\nu - \int _S F_\nu d\mu \\ &= \int _S F_\mu (\nu -\mu ) + \int _S(F_\nu -F_\mu )d(\nu -\mu ) \\ &\le 0 \end {align*} for all $\nu \in \P (S)$. Hence, $\mu $ is a GNSS of the game $F$. It is clear that if $\mu $ is a strict Nash equilibrium or if $F$ is strictly monotone, then the above inequality becomes strict for $\nu \in \P (S)\setminus \{\mu \}$ and hence $\mu $ is a GESS of the game $F$ in these cases.\end{proof}

\prAtEndRestatexvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxvi}]\phantomsection\label{proof:prAtEndxvi}This follows directly from \autoref {prop: monotone_nash} together with \autoref {prop: unique_gess}.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexvii}\label{thm:prAtEndxvii}\label {lem: convex_stable_set} Consider a game $F\colon \P (S)\to C(S)$ and let $N\subseteq \P (S)$ be an arbitrary set of population states. Let $\stab _N^F \subseteq \P (S)$ denote the set of all population states $\mu \in \P (S)$ such that, for all $\nu \in N$, it holds that \begin {equation*} E_F(\nu ,\nu )\le E_F(\mu ,\nu ). \end {equation*} Then, it holds that $\stab _N^F$ is a convex set.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxvii}]\phantomsection\label{proof:prAtEndxvii}It holds that \begin {align*} \stab _N^F &= \{\mu \in \P (S) : \text {$E_F(\nu ,\nu ) \le E_F(\mu ,\nu )$ for all $\nu \in N$}\} \\ &= \bigcap _{\nu \in N} \{\mu \in \P (S) : E_F(\nu ,\nu ) \le E_F(\mu ,\nu )\}. \end {align*} Since $E_F$ is linear in its first argument, the set $\{\mu \in \P (S) : E_F(\nu ,\nu ) \le E_F(\mu ,\nu )\}$ is convex for all $\nu \in N$, and therefore the set $\stab _N^F$, being the intersection of convex sets, is also a convex set.\end{proof}

\prAtEndRestatexviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxviii}]\phantomsection\label{proof:prAtEndxviii}By \autoref {prop: monotone_nash}, every Nash equilibrium of the game $F$ is a GNSS of the game $F$, and by \autoref {prop: nss_implies_nash} every GNSS of the game $F$ is a Nash equilibrium of the game $F$. Hence, the set of Nash equilibria of the game $F$ equals the set of globally neutrally stable states of the game $F$, so $\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\nu ) \le E_F(\mu ,\nu )$ for all $\nu \in \P (S)$}\}$. Applying \autoref {lem: convex_stable_set} with $N = \P (S)$ proves the claim.\end{proof}

\prAtEndRestatexix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxix}]\phantomsection\label{proof:prAtEndxix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics.} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics.} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatexx*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxx}]\phantomsection\label{proof:prAtEndxx}Suppose that $v$ is Nash stationary, $v$ is $\delta $-passive, and $F$ is monotone. Let $w\colon \M (S) \times C(S) \to \R $ be defined by $w(\mu ,\eta ) = \left <\eta ,\mu \right >$. Then it holds that $v$ is $\delta $-dissipative with supply rate $w$. Furthermore, by \autoref {lem: monotone_sde}, $F$ satisfies self-defeating externalities, and therefore \begin {equation*} w(\nu ,D\overline {F}(\mu )\nu ) = \left <D\overline {F}(\mu )\nu ,\nu \right > \le 0 ~ \text {for all $\mu \in \P (S)$ and all $\nu \in T\P (S)$.} \end {equation*} Hence, by \autoref {thm: delta-dissipative}, it holds that $\NE (F)$ is weakly Lyapunov stable under the EDM \eqref {eq: edm}. The fact that $\NE (F)$ is globally weakly attracting under the EDM \eqref {eq: edm} given the additional hypotheses of \autoref {ass: game_derivative} and \autoref {ass: dynamics_map} is immediate from \autoref {thm: delta-dissipative}.\end{proof}

\prAtEndRestatexxi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxi}]\phantomsection\label{proof:prAtEndxxi}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\prAtEndRestatexxii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxii}]\phantomsection\label{proof:prAtEndxxii}Since $v$ is $\delta $-dissipative with supply rate $w\colon \M (S) \times C(S) \to \R $, there exist $\sigma \colon \P (S) \times C(S) \to \Rpl $ and $\storage \colon \P (S) \times C(S) \to \Rpl $ with $\storage $ having an appropriate extension $\overline {\storage } \colon U\times C(S) \to \R $ as in \autoref {def: delta-dissipative}. Furthermore, since $u$ is $\delta $-antidissipative with supply rate $\tilde {w}\colon \M (S) \times C(S) \to \R $, there exist $\gamma \colon \P (S) \times C(S) \to \Rpl $ and $\Gamma \colon \P (S) \times C(S) \to \Rpl $ with $\Gamma $ having an appropriate extension $\overline {\Gamma } \colon \tilde {U}\times C(S) \to \R $ as in \autoref {def: delta-antidissipative}. Define $V \colon \P (S)\times K \to \Rpl $ by $V(\mu ,\rho ) = \storage (\mu ,\rho ) + \Gamma (\mu ,\rho )$. Consider $P = \{(\mu ,\rho ) \in \P (S) \times C(S) : v(\mu ,\rho ) = 0, ~ u(\mu ,\rho ) = 0\}$. If $(\mu ,\rho ) \in P$, then $u(\mu ,\rho ) = 0$, implying that $\rho = F(\mu )$ by $F$-payoff stationarity, and hence $v(\mu ,F(\mu )) = 0$, so $\mu \in \NE (F)$ by Nash stationarity. Thus, $P \subseteq \NE (F) \times F(\NE (F)) \subseteq \P (S) \times K$. By \autoref {prop: ne_closed} and \autoref {prop: weakly_continuous_payoff}, $\NE (F)$ is weakly compact, and hence $F(\NE (F))$ is compact as $F$ is weakly continuous. Since $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain, and $u$ is weak-$\infty $-continuous, it holds that $P = v^{-1}(\{0\})\cap u^{-1}(\{0\})$ is weak-$\infty $-closed, and hence must be weak-$\infty $-compact as well as $\NE (F) \times F(\NE (F))$ is. Thus, by \autoref {lem: lyapunov}, it suffices to show that $V$ is a global Lyapunov function for $P$ under $(\mu ,\rho ) \mapsto (v(\mu ,\rho ),u(\mu ,\rho ))$ (according to \autoref {def: lyapunov_function}). Let $\overline {V}\colon U\cap \tilde {U} \times C(S) \to \R $ be defined by $\overline {V}(\mu ,\rho ) = \overline {\storage }(\mu ,\rho ) + \overline {\Gamma }(\mu ,\rho )$. Note that $U\cap \tilde {U}$ is strongly open and contains $\P (S)$, and that $\overline {V}$ is weak-$\infty $-continuous and Fr\'echet differentiable since $\overline {\storage }$ and $\overline {\Gamma }$ are. Also note that $\overline {V}(\mu ,\rho ) = V(\mu ,\rho )$ for all $(\mu ,\rho ) \in \P (S) \times K$. Also, if $(\mu ,\rho ) \in P$, then $v(\mu ,\rho ) = 0$ and $u(\mu ,\rho ) = 0$, so $\overline {V}(\mu ,\rho ) = 0$ by \eqref {eq: delta-dissipative-2} and \eqref {eq: delta-antidissipative-2}. Furthermore, if $(\mu ,\rho ) \in (\P (S) \times K) \setminus P$, then again by \eqref {eq: delta-dissipative-2} and \eqref {eq: delta-antidissipative-2} we have that $\overline {V}(\mu ,\rho ) > 0$. Therefore, the first two conditions from \autoref {def: lyapunov_function} on $V$ to be a global Lyapunov function for $P$ under $(v,u)$ are satisfied. \par Next, it holds for all $(\mu ,\rho ) \in \P (S) \times K$ that \begin {equation} \begin {aligned} D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) &= \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu , \rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) u(\mu , \rho ) + \partial _1 \overline {\Gamma }(\mu ,\rho ) v(\mu , \rho ) + \partial _2 \overline {\Gamma }(\mu ,\rho ) u(\mu , \rho ) \\ &\le -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),u(\mu ,\rho )) - \gamma (\mu ,\rho ) - \tilde {w}(v(\mu ,\rho ),u(\mu ,\rho )) \\ &\le -\sigma (\mu ,F(\mu )) - \gamma (\mu ,\rho ) \\ &\le 0, \end {aligned} \label {eq: decreasing_derivative-dpedm} \end {equation} where the first inequality follows from \eqref {eq: delta-dissipative-1} and \eqref {eq: delta-antidissipative-1}, and the second inequality follows from the fact that $\tilde {w} \ge w$. Hence, $V$ is indeed a global Lyapunov function for $P$ under $(v,u)$, so $P$ is weak-$\infty $-Lyapunov stable under the DPEDM \eqref {eq: dpedm}. \par Now suppose that the $\delta $-dissipativity of $v$ and the $\delta $-antidissipativity of $u$ are both strict, and that $v$ is $\|\cdot \|_\TV $-bounded on $\P (S)\times K$. By \autoref {lem: strict_lyapunov}, it suffices to show that $V$ is a strict global Lyapunov function for $P$ under $(\mu ,\rho )\mapsto (v(\mu ,\rho ),u(\mu ,\rho ))$ (according to \autoref {def: lyapunov_function}). This amounts to proving that $(\mu ,\rho ) \mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weak-$\infty $-continuous and that $D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) < 0$ for all $(\mu ,\rho )\in (\P (S) \times K)\setminus P$. Indeed, the continuity condition holds by \autoref {lem: weakly_continuous_derivative-dpedm}, which we proof after completing the current proof. \par Next, if $(\mu ,\rho )\in (\P (S)\times K)\setminus P$, then $v(\mu ,\rho ) \ne 0$ or $u(\mu ,\rho ) \ne 0$, so $\sigma (\mu ,\rho ) > 0$ or $\gamma (\mu ,\rho ) > 0$ by \eqref {eq: delta-dissipative-3} and \eqref {eq: delta-antidissipative-3}, implying that $D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) < 0$ for all such $(\mu ,\rho )$ by \eqref {eq: decreasing_derivative-dpedm}. Hence, $V$ is indeed a strict global Lyapunov function for $P$ under $(v,u)$, so $P$ is globally weak-$\infty $-attracting under the DPEDM \eqref {eq: dpedm} from $K$.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexxiii}\label{thm:prAtEndxxiii}\label {lem: weakly_continuous_derivative-dpedm} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxiii}]\phantomsection\label{proof:prAtEndxxiii}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexxiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxiv}]\phantomsection\label{proof:prAtEndxxiv}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexxv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxv}]\phantomsection\label{proof:prAtEndxxv}In this proof, we denote the indicator function on a set $A \subseteq \R $ by $\chi _A \colon \R \to \R $, where \begin {equation*} \chi _A(t) = \begin {aligned} \begin {cases} 1 & \text {if $t \in A$}, \\ 0 & \text {if $t \notin A$}. \end {cases} \end {aligned} \end {equation*} \par Let $\mu ,\nu \in \P (S)$. It holds that \begin {align*} & 2 \int _S \int _S \tilde {\Theta }(s-s') d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S \tilde {\Theta }(s-s') d(\mu -\nu )(s') d(\mu -\nu )(s) + \int _S \int _S \tilde {\Theta }(s'-s) d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S \left (\tilde {\Theta }(s-s') + \tilde {\Theta }(s'-s)\right ) d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S d(\mu -\nu )(s') d(\mu -\nu )(s) \\ & \qquad = ((\mu -\nu )(S))^2 \\ & \qquad =0, \end {align*} since $(\mu -\nu )(S) = \mu (S) - \nu (S) = 0$. Therefore, \begin {equation*} \int _S \int _S \tilde {\Theta }(s-s')d(\mu -\nu )(s')d(\mu -\nu )(s) = 0. \end {equation*} Next, we note that \begin {align*} \int _S \int _S \min \{s,s'\} d\mu (s') d\nu (s) &= \int _S \int _S \int _{[0,\min \{s,s'\}]} dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{t' \in \R : t' \le \min \{s,s'\}\}}(t) dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{t' \in \R : t'\le s\}}(t) \chi _{\{t'\in \R : t\le s'\}}(t) dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s) \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s') dt d\mu (s') d\nu (s) \\ &= \int _{[0,\infty )} \int _S \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s') d\mu (s')\int _S \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s) d\nu (s) dt \\ &= \int _{[0,\infty )} \mu (S \cap [t,\infty )) \nu (S\cap [t,\infty )) dt. \end {align*} Therefore, we find that \begin {align*} & \int _S \int _S \min \{s,s'\} d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _{[0,\infty )} \left (\mu (S\cap [t,\infty ))^2 - 2\mu (S\cap [t,\infty ))\nu (S\cap [t,\infty )) + \nu (S\cap [t,\infty ))^2\right ) dt \\ &\qquad = \int _{[0,\infty )} \left (\mu (S\cap [t,\infty )) - \nu (S\cap [t,\infty ))\right )^2 dt. \end {align*} Thus, overall, it holds that \begin {align*} \left <F(\mu ) - F(\nu ), \mu -\nu \right > &= \int _S(F_\mu (s) - F_\nu (s)) d(\mu -\nu )(s) \\ &= \int _S \int _S \tilde {f}(s,s') d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &= V\int _S \int _S \tilde {\Theta }(s-s')d(\mu -\nu )(s')d(\mu -\nu )(s) - \int _S \int _S \min \{s,s'\} d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &= -\int _{[0,\infty )} \left (\mu (S\cap [t,\infty )) - \nu (S\cap [t,\infty ))\right )^2 dt \\ &\le 0. \end {align*} Hence, $F$ is monotone.\end{proof}

\prAtEndRestatexxvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxvi}]\phantomsection\label{proof:prAtEndxxvi}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {prop: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-figure3-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable, and hence this is a sequential space. Therefore, $\P (S)$ is weakly closed if and only if it is weakly sequentially closed. It is clear that if $\{\mu _n \in \P (S) : n\in \N \}$ is a sequence in $\P (S)$ that weakly converges to $\mu \in \M (S)$, then $\mu \in \P (S)$ since it must be nonnegative and since the constant function $1$ is an element of $C(S)$. Hence, $\P (S)$ is weakly closed. By the Banach-Alaoglu theorem, the unit ball $\{\mu \in \M (S) : \|\mu \|_\TV \le 1\}$ is weak-$*$ compact and hence weakly compact as these two topologies coincide since $S$ is compact. Thus, the weakly closed subset $\P (S)$ of the weakly compact unit ball must also be weakly compact.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Let $\mu \in \P (S)$ be a NSS of the game $F\colon \P (S)\to C(S)$. Suppose that $h^F_{\nu :\mu }$ is right-continuous at $0$ for all $\nu \in \P (S)$. Let $\nu \in \P (S)$. Then, there exists $\epsilon (\nu )\in (0,1]$ such that \begin {equation*} h^F_{\nu :\mu }(\eta ) = E_F(\nu ,(1-\eta )\mu +\eta \nu ) - E_F(\mu ,(1-\eta )\mu +\eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,\epsilon (\nu )]$. Thus, by the right-continuity of $h^F_{\nu :\mu }$, it holds that \begin {equation*} E_F(\nu ,\mu )-E_F(\mu ,\mu ) = h^F_{\nu :\mu }(0) = \lim _{\eta \downarrow 0} h^F_{\nu :\mu }(\eta ) \le 0. \end {equation*} Since $\nu $ is arbitrary, this proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $\mu \in \P (S)$ is a GNSS of the game $F\colon \P (S)\to C(S)$. Let $\nu \in \P (S)$. Then, since $\mu $ is a GNSS of the game $F$, it holds that \begin {equation*} E_F((1-\eta )\mu +\eta \nu ,(1-\eta )\mu + \eta \nu ) - E_F(\mu ,(1-\eta )\mu +\eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,1]$. By linearity of $E_F$ in its first argument, we find that \begin {equation*} \eta E_F(\nu ,(1-\eta ) \mu + \eta \nu ) - \eta E_F(\mu ,(1-\eta ) \mu + \eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,1]$. Dividing by $\eta $ proves that $\mu $ is a NSS of the game $F$. The proof that $\mu $ being a GESS implies that $\mu $ is an ESS is identical as above with strict inqualities when considering $\nu \in \P (S)\setminus \{\mu \}$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Since $\mu $ is a GESS of the game $F$, it holds that $\mu $ is a NSS of the game $F$, and therefore $\mu \in \NE (F)$ by \autoref {prop: nss_implies_nash}, as $h^F_{\nu :\mu }$ is right-continuous at $0$. For all $\nu \in \P (S)\setminus \{\mu \}$, it holds that $E_F(\nu ,\nu ) < E(\mu ,\nu )$ since $\mu $ is a GESS of the game $F$, and therefore such $\nu $ are not Nash equilibria of the game $F$. This proves that indeed $\NE (F) = \{\mu \}$.\end{proof}

\prAtEndRestatevii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}It holds that $\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$. For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}Suppose that $\mu ([0,\infty ))\subseteq \P (S)$. Let $t\in (0,\infty )$. Since $\frac {\mu (t+\epsilon ) - \mu (t)}{\epsilon }$ converges strongly to $\dot {\mu }(t)$ as $\epsilon \to 0$, it also converges weakly to $\dot {\mu }(t)$ as $\epsilon \to 0$, so \begin {equation*} \lim _{\epsilon \to 0}\int _S f d \left (\frac {\mu (t+\epsilon ) - \mu (t)}{\epsilon }\right ) = \int _S f d\dot {\mu }(t) \end {equation*} for all $f\in C(S)$. In particular, taking $f$ to be the function that is identically $1$ on $S$ yields that \begin {equation*} \lim _{\epsilon \to 0} \frac {1}{\epsilon }\left (\mu (t+\epsilon )(S) - \mu (t)(S)\right ) = \dot {\mu }(t)(S). \end {equation*} Since $\mu (t)$ and $\mu (t+\epsilon )$ are probability measures for all $\epsilon \in [-t,\infty )$, it holds that $\mu (t+\epsilon )(S) = \mu (t)(S) = 1$ for all such $\epsilon $, and hence $\frac {1}{\epsilon }\left (\mu (t+\epsilon )(S) - \mu (t)(S)\right ) = 0$ for all $\epsilon \in [-t,\infty )\setminus \{0\}$. Therefore, it must be that \begin {equation*} \dot {\mu }(t)(S) = 0, \end {equation*} so indeed $\dot {\mu }(t) \in T\P (S)$. The case for $t=0$ follows similarly.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatexi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$. Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$ for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that $\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$, and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexii}\label{thm:prAtEndxii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}Since $v$ is $\delta $-dissipative with supply rate $w\colon \M (S) \times C(S) \to \R $, there exist $\sigma \colon \P (S) \times C(S) \to \Rpl $ and $\storage \colon \P (S) \times C(S) \to \Rpl $ with $\storage $ having an appropriate extension $\overline {\storage } \colon U\times C(S) \to \R $ as in \autoref {def: delta-dissipative}. Define $V \colon \P (S) \to \Rpl $ by $V(\mu ) = \storage (\mu ,F(\mu ))$. By \autoref {prop: ne_closed} and \autoref {prop: weakly_continuous_payoff}, $\NE (F)$ is weakly compact. Thus, by \autoref {lem: lyapunov}, it suffices to show that $V$ is a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ (according to \autoref {def: lyapunov_function}). Let $\overline {V}\colon U\cap U' \to \R $ be defined by $\overline {V}(\mu ) = \overline {\storage }(\mu ,\overline {F}(\mu ))$. Note that $U\cap U'$ is strongly open and contains $\P (S)$, and that $\overline {V}$ is weakly continuous and Fr\'echet differentiable since $\overline {\storage }$ is weak-$\infty $-continuous and $\overline {F}$ is weakly continuous, and both $\overline {\storage }$ and $\overline {F}$ are Fr\'echet differentiable. Also note that $\overline {V}(\mu ) = V(\mu )$ for all $\mu \in \P (S)$. Also, if $\mu \in \NE (F)$, then $v(\mu ,F(\mu )) = 0$ by \autoref {prop: ns_implies_rest_equals_nash}, and therefore $\overline {V}(\mu ) = V(\mu ) = \storage (\mu ,F(\mu )) = 0$ by \eqref {eq: delta-dissipative-2}. Furthermore, if $\mu \in \P (S)\setminus \NE (F)$, then again by \autoref {prop: ns_implies_rest_equals_nash} we have that $v(\mu ,F(\mu )) \ne 0$, so $\overline {V}(\mu ) = V(\mu ) = \storage (\mu ,F(\mu )) > 0$ by \eqref {eq: delta-dissipative-2}. Therefore, the first two conditions from \autoref {def: lyapunov_function} on $V$ to be a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ are satisfied. \par Next, since $\overline {\storage }$ and $\overline {F}$ are Fr\'echet differentiable, \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} for all $\mu \in U\cap U'$, and therefore, since $\overline {F}(\mu ) = F(\mu )$ for all $\mu \in \P (S)$, it holds for all $\mu \in \P (S)$ that \begin {equation} \begin {aligned} D\overline {V}(\mu )v(\mu ,F(\mu )) &= \partial _1 \overline {\storage }(\mu ,F(\mu )) v(\mu , F(\mu )) + \partial _2 \overline {\storage }(\mu ,F(\mu )) D\overline {F}(\mu ) v(\mu , F(\mu )) \\ &\le -\sigma (\mu ,F(\mu )) + w(v(\mu ,F(\mu )),D\overline {F}(\mu )v(\mu ,F(\mu ))) \\ &\le -\sigma (\mu ,F(\mu )) \\ &\le 0, \end {aligned} \label {eq: decreasing_derivative} \end {equation} where the first inequality follows from \eqref {eq: delta-dissipative-1}, and the second inequality follows from \eqref {eq: supply_inequality} together with the fact that $v(\mu ,F(\mu ))\in T\P (S)$. Hence, $V$ is indeed a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$, so $\NE (F)$ is weakly Lyapunov stable under the EDM \eqref {eq: edm}. \par Now suppose that the $\delta $-dissipativity of $v$ is strict and that the additional hypotheses of \autoref {ass: game_derivative} and \autoref {ass: dynamics_map} both hold. By \autoref {lem: strict_lyapunov}, it suffices to show that $V$ is a strict global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ (according to \autoref {def: lyapunov_function}). This amounts to proving that $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous and that $D\overline {V}(\mu )v(\mu ,F(\mu )) < 0$ for all $\mu \in \P (S)\setminus \NE (F)$. Indeed, the continuity condition holds by \autoref {lem: weakly_continuous_derivative}, which we proof after completing the current proof. \par Next, if $\mu \in \P (S)\setminus \NE (F)$, then \autoref {prop: ns_implies_rest_equals_nash} gives that $v(\mu ,F(\mu )) \ne 0$ so $\sigma (\mu ,F(\mu )) > 0$ by \eqref {eq: delta-dissipative-3}, implying that $D\overline {V}(\mu )v(\mu ,F(\mu )) < 0$ for all such $\mu $ by \eqref {eq: decreasing_derivative}. Hence, $V$ is indeed a strict global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$, so $\NE (F)$ is globally weakly attracting under the EDM \eqref {eq: edm}.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexiv}\label{thm:prAtEndxiv}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiv}]\phantomsection\label{proof:prAtEndxiv}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {align*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| &\le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {align*} }{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and also since $\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$ for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\quad + \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestatexv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxv}]\phantomsection\label{proof:prAtEndxv}Let $\mu \in \P (S)$ be a Nash equilibrium of the game $F$. Then $\int _S F_\mu d\nu \le \int _S F_\mu d\mu $ for all $\nu \in \P (S)$, so by monotonicity it holds that \begin {align*} E_F(\nu ,\nu ) - E_F(\mu ,\nu ) &= \int _S F_\nu d\nu - \int _S F_\nu d\mu \\ &= \int _S F_\mu (\nu -\mu ) + \int _S(F_\nu -F_\mu )d(\nu -\mu ) \\ &\le 0 \end {align*} for all $\nu \in \P (S)$. Hence, $\mu $ is a GNSS of the game $F$. It is clear that if $\mu $ is a strict Nash equilibrium or if $F$ is strictly monotone, then the above inequality becomes strict for $\nu \in \P (S)\setminus \{\mu \}$ and hence $\mu $ is a GESS of the game $F$ in these cases.\end{proof}

\prAtEndRestatexvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxvi}]\phantomsection\label{proof:prAtEndxvi}This follows directly from \autoref {prop: monotone_nash} together with \autoref {prop: unique_gess}.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexvii}\label{thm:prAtEndxvii}\label {lem: convex_stable_set} Consider a game $F\colon \P (S)\to C(S)$ and let $N\subseteq \P (S)$ be an arbitrary set of population states. Let $\stab _N^F \subseteq \P (S)$ denote the set of all population states $\mu \in \P (S)$ such that, for all $\nu \in N$, it holds that \begin {equation*} E_F(\nu ,\nu )\le E_F(\mu ,\nu ). \end {equation*} Then, it holds that $\stab _N^F$ is a convex set.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxvii}]\phantomsection\label{proof:prAtEndxvii}It holds that \begin {align*} \stab _N^F &= \{\mu \in \P (S) : \text {$E_F(\nu ,\nu ) \le E_F(\mu ,\nu )$ for all $\nu \in N$}\} \\ &= \bigcap _{\nu \in N} \{\mu \in \P (S) : E_F(\nu ,\nu ) \le E_F(\mu ,\nu )\}. \end {align*} Since $E_F$ is linear in its first argument, the set $\{\mu \in \P (S) : E_F(\nu ,\nu ) \le E_F(\mu ,\nu )\}$ is convex for all $\nu \in N$, and therefore the set $\stab _N^F$, being the intersection of convex sets, is also a convex set.\end{proof}

\prAtEndRestatexviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxviii}]\phantomsection\label{proof:prAtEndxviii}By \autoref {prop: monotone_nash}, every Nash equilibrium of the game $F$ is a GNSS of the game $F$, and by \autoref {prop: nss_implies_nash} every GNSS of the game $F$ is a Nash equilibrium of the game $F$. Hence, the set of Nash equilibria of the game $F$ equals the set of globally neutrally stable states of the game $F$, so $\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\nu ) \le E_F(\mu ,\nu )$ for all $\nu \in \P (S)$}\}$. Applying \autoref {lem: convex_stable_set} with $N = \P (S)$ proves the claim.\end{proof}

\prAtEndRestatexix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxix}]\phantomsection\label{proof:prAtEndxix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics.} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics.} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatexx*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxx}]\phantomsection\label{proof:prAtEndxx}Suppose that $v$ is Nash stationary, $v$ is $\delta $-passive, and $F$ is monotone. Let $w\colon \M (S) \times C(S) \to \R $ be defined by $w(\mu ,\eta ) = \left <\eta ,\mu \right >$. Then it holds that $v$ is $\delta $-dissipative with supply rate $w$. Furthermore, by \autoref {lem: monotone_sde}, $F$ satisfies self-defeating externalities, and therefore \begin {equation*} w(\nu ,D\overline {F}(\mu )\nu ) = \left <D\overline {F}(\mu )\nu ,\nu \right > \le 0 ~ \text {for all $\mu \in \P (S)$ and all $\nu \in T\P (S)$.} \end {equation*} Hence, by \autoref {thm: delta-dissipative}, it holds that $\NE (F)$ is weakly Lyapunov stable under the EDM \eqref {eq: edm}. The fact that $\NE (F)$ is globally weakly attracting under the EDM \eqref {eq: edm} given the additional hypotheses of \autoref {ass: game_derivative} and \autoref {ass: dynamics_map} is immediate from \autoref {thm: delta-dissipative}.\end{proof}

\prAtEndRestatexxi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxi}]\phantomsection\label{proof:prAtEndxxi}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\prAtEndRestatexxii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxii}]\phantomsection\label{proof:prAtEndxxii}Since $v$ is $\delta $-dissipative with supply rate $w\colon \M (S) \times C(S) \to \R $, there exist $\sigma \colon \P (S) \times C(S) \to \Rpl $ and $\storage \colon \P (S) \times C(S) \to \Rpl $ with $\storage $ having an appropriate extension $\overline {\storage } \colon U\times C(S) \to \R $ as in \autoref {def: delta-dissipative}. Furthermore, since $u$ is $\delta $-antidissipative with supply rate $\tilde {w}\colon \M (S) \times C(S) \to \R $, there exist $\gamma \colon \P (S) \times C(S) \to \Rpl $ and $\Gamma \colon \P (S) \times C(S) \to \Rpl $ with $\Gamma $ having an appropriate extension $\overline {\Gamma } \colon \tilde {U}\times C(S) \to \R $ as in \autoref {def: delta-antidissipative}. Define $V \colon \P (S)\times K \to \Rpl $ by $V(\mu ,\rho ) = \storage (\mu ,\rho ) + \Gamma (\mu ,\rho )$. Consider $P = \{(\mu ,\rho ) \in \P (S) \times C(S) : v(\mu ,\rho ) = 0, ~ u(\mu ,\rho ) = 0\}$. If $(\mu ,\rho ) \in P$, then $u(\mu ,\rho ) = 0$, implying that $\rho = F(\mu )$ by $F$-payoff stationarity, and hence $v(\mu ,F(\mu )) = 0$, so $\mu \in \NE (F)$ by Nash stationarity. Thus, $P \subseteq \NE (F) \times F(\NE (F)) \subseteq \P (S) \times K$. By \autoref {prop: ne_closed} and \autoref {prop: weakly_continuous_payoff}, $\NE (F)$ is weakly compact, and hence $F(\NE (F))$ is compact as $F$ is weakly continuous. Since $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain, and $u$ is weak-$\infty $-continuous, it holds that $P = v^{-1}(\{0\})\cap u^{-1}(\{0\})$ is weak-$\infty $-closed, and hence must be weak-$\infty $-compact as well as $\NE (F) \times F(\NE (F))$ is. Thus, by \autoref {lem: lyapunov}, it suffices to show that $V$ is a global Lyapunov function for $P$ under $(\mu ,\rho ) \mapsto (v(\mu ,\rho ),u(\mu ,\rho ))$ (according to \autoref {def: lyapunov_function}). Let $\overline {V}\colon U\cap \tilde {U} \times C(S) \to \R $ be defined by $\overline {V}(\mu ,\rho ) = \overline {\storage }(\mu ,\rho ) + \overline {\Gamma }(\mu ,\rho )$. Note that $U\cap \tilde {U}$ is strongly open and contains $\P (S)$, and that $\overline {V}$ is weak-$\infty $-continuous and Fr\'echet differentiable since $\overline {\storage }$ and $\overline {\Gamma }$ are. Also note that $\overline {V}(\mu ,\rho ) = V(\mu ,\rho )$ for all $(\mu ,\rho ) \in \P (S) \times K$. Also, if $(\mu ,\rho ) \in P$, then $v(\mu ,\rho ) = 0$ and $u(\mu ,\rho ) = 0$, so $\overline {V}(\mu ,\rho ) = 0$ by \eqref {eq: delta-dissipative-2} and \eqref {eq: delta-antidissipative-2}. Furthermore, if $(\mu ,\rho ) \in (\P (S) \times K) \setminus P$, then again by \eqref {eq: delta-dissipative-2} and \eqref {eq: delta-antidissipative-2} we have that $\overline {V}(\mu ,\rho ) > 0$. Therefore, the first two conditions from \autoref {def: lyapunov_function} on $V$ to be a global Lyapunov function for $P$ under $(v,u)$ are satisfied. \par Next, it holds for all $(\mu ,\rho ) \in \P (S) \times K$ that \begin {equation} \begin {aligned} D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) &= \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu , \rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) u(\mu , \rho ) + \partial _1 \overline {\Gamma }(\mu ,\rho ) v(\mu , \rho ) + \partial _2 \overline {\Gamma }(\mu ,\rho ) u(\mu , \rho ) \\ &\le -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),u(\mu ,\rho )) - \gamma (\mu ,\rho ) - \tilde {w}(v(\mu ,\rho ),u(\mu ,\rho )) \\ &\le -\sigma (\mu ,F(\mu )) - \gamma (\mu ,\rho ) \\ &\le 0, \end {aligned} \label {eq: decreasing_derivative-dpedm} \end {equation} where the first inequality follows from \eqref {eq: delta-dissipative-1} and \eqref {eq: delta-antidissipative-1}, and the second inequality follows from the fact that $\tilde {w} \ge w$. Hence, $V$ is indeed a global Lyapunov function for $P$ under $(v,u)$, so $P$ is weak-$\infty $-Lyapunov stable under the DPEDM \eqref {eq: dpedm}. \par Now suppose that the $\delta $-dissipativity of $v$ and the $\delta $-antidissipativity of $u$ are both strict, and that $v$ is $\|\cdot \|_\TV $-bounded on $\P (S)\times K$. By \autoref {lem: strict_lyapunov}, it suffices to show that $V$ is a strict global Lyapunov function for $P$ under $(\mu ,\rho )\mapsto (v(\mu ,\rho ),u(\mu ,\rho ))$ (according to \autoref {def: lyapunov_function}). This amounts to proving that $(\mu ,\rho ) \mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weak-$\infty $-continuous and that $D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) < 0$ for all $(\mu ,\rho )\in (\P (S) \times K)\setminus P$. Indeed, the continuity condition holds by \autoref {lem: weakly_continuous_derivative-dpedm}, which we proof after completing the current proof. \par Next, if $(\mu ,\rho )\in (\P (S)\times K)\setminus P$, then $v(\mu ,\rho ) \ne 0$ or $u(\mu ,\rho ) \ne 0$, so $\sigma (\mu ,\rho ) > 0$ or $\gamma (\mu ,\rho ) > 0$ by \eqref {eq: delta-dissipative-3} and \eqref {eq: delta-antidissipative-3}, implying that $D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) < 0$ for all such $(\mu ,\rho )$ by \eqref {eq: decreasing_derivative-dpedm}. Hence, $V$ is indeed a strict global Lyapunov function for $P$ under $(v,u)$, so $P$ is globally weak-$\infty $-attracting under the DPEDM \eqref {eq: dpedm} from $K$.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexxiii}\label{thm:prAtEndxxiii}\label {lem: weakly_continuous_derivative-dpedm} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxiii}]\phantomsection\label{proof:prAtEndxxiii}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexxiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxiv}]\phantomsection\label{proof:prAtEndxxiv}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexxv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxv}]\phantomsection\label{proof:prAtEndxxv}In this proof, we denote the indicator function on a set $A \subseteq \R $ by $\chi _A \colon \R \to \R $, where \begin {equation*} \chi _A(t) = \begin {aligned} \begin {cases} 1 & \text {if $t \in A$}, \\ 0 & \text {if $t \notin A$}. \end {cases} \end {aligned} \end {equation*} \par Let $\mu ,\nu \in \P (S)$. It holds that \begin {align*} & 2 \int _S \int _S \tilde {\Theta }(s-s') d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S \tilde {\Theta }(s-s') d(\mu -\nu )(s') d(\mu -\nu )(s) + \int _S \int _S \tilde {\Theta }(s'-s) d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S \left (\tilde {\Theta }(s-s') + \tilde {\Theta }(s'-s)\right ) d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S d(\mu -\nu )(s') d(\mu -\nu )(s) \\ & \qquad = ((\mu -\nu )(S))^2 \\ & \qquad =0, \end {align*} since $(\mu -\nu )(S) = \mu (S) - \nu (S) = 0$. Therefore, \begin {equation*} \int _S \int _S \tilde {\Theta }(s-s')d(\mu -\nu )(s')d(\mu -\nu )(s) = 0. \end {equation*} Next, we note that \begin {align*} \int _S \int _S \min \{s,s'\} d\mu (s') d\nu (s) &= \int _S \int _S \int _{[0,\min \{s,s'\}]} dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{t' \in \R : t' \le \min \{s,s'\}\}}(t) dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{t' \in \R : t'\le s\}}(t) \chi _{\{t'\in \R : t\le s'\}}(t) dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s) \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s') dt d\mu (s') d\nu (s) \\ &= \int _{[0,\infty )} \int _S \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s') d\mu (s')\int _S \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s) d\nu (s) dt \\ &= \int _{[0,\infty )} \mu (S \cap [t,\infty )) \nu (S\cap [t,\infty )) dt. \end {align*} Therefore, we find that \begin {align*} & \int _S \int _S \min \{s,s'\} d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _{[0,\infty )} \left (\mu (S\cap [t,\infty ))^2 - 2\mu (S\cap [t,\infty ))\nu (S\cap [t,\infty )) + \nu (S\cap [t,\infty ))^2\right ) dt \\ &\qquad = \int _{[0,\infty )} \left (\mu (S\cap [t,\infty )) - \nu (S\cap [t,\infty ))\right )^2 dt. \end {align*} Thus, overall, it holds that \begin {align*} \left <F(\mu ) - F(\nu ), \mu -\nu \right > &= \int _S(F_\mu (s) - F_\nu (s)) d(\mu -\nu )(s) \\ &= \int _S \int _S \tilde {f}(s,s') d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &= V\int _S \int _S \tilde {\Theta }(s-s')d(\mu -\nu )(s')d(\mu -\nu )(s) - \int _S \int _S \min \{s,s'\} d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &= -\int _{[0,\infty )} \left (\mu (S\cap [t,\infty )) - \nu (S\cap [t,\infty ))\right )^2 dt \\ &\le 0. \end {align*} Hence, $F$ is monotone.\end{proof}

\prAtEndRestatexxvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxvi}]\phantomsection\label{proof:prAtEndxxvi}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {prop: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-figure4-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable, and hence this is a sequential space. Therefore, $\P (S)$ is weakly closed if and only if it is weakly sequentially closed. It is clear that if $\{\mu _n \in \P (S) : n\in \N \}$ is a sequence in $\P (S)$ that weakly converges to $\mu \in \M (S)$, then $\mu \in \P (S)$ since it must be nonnegative and since the constant function $1$ is an element of $C(S)$. Hence, $\P (S)$ is weakly closed. By the Banach-Alaoglu theorem, the unit ball $\{\mu \in \M (S) : \|\mu \|_\TV \le 1\}$ is weak-$*$ compact and hence weakly compact as these two topologies coincide since $S$ is compact. Thus, the weakly closed subset $\P (S)$ of the weakly compact unit ball must also be weakly compact.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Let $\mu \in \P (S)$ be a NSS of the game $F\colon \P (S)\to C(S)$. Suppose that $h^F_{\nu :\mu }$ is right-continuous at $0$ for all $\nu \in \P (S)$. Let $\nu \in \P (S)$. Then, there exists $\epsilon (\nu )\in (0,1]$ such that \begin {equation*} h^F_{\nu :\mu }(\eta ) = E_F(\nu ,(1-\eta )\mu +\eta \nu ) - E_F(\mu ,(1-\eta )\mu +\eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,\epsilon (\nu )]$. Thus, by the right-continuity of $h^F_{\nu :\mu }$, it holds that \begin {equation*} E_F(\nu ,\mu )-E_F(\mu ,\mu ) = h^F_{\nu :\mu }(0) = \lim _{\eta \downarrow 0} h^F_{\nu :\mu }(\eta ) \le 0. \end {equation*} Since $\nu $ is arbitrary, this proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $\mu \in \P (S)$ is a GNSS of the game $F\colon \P (S)\to C(S)$. Let $\nu \in \P (S)$. Then, since $\mu $ is a GNSS of the game $F$, it holds that \begin {equation*} E_F((1-\eta )\mu +\eta \nu ,(1-\eta )\mu + \eta \nu ) - E_F(\mu ,(1-\eta )\mu +\eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,1]$. By linearity of $E_F$ in its first argument, we find that \begin {equation*} \eta E_F(\nu ,(1-\eta ) \mu + \eta \nu ) - \eta E_F(\mu ,(1-\eta ) \mu + \eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,1]$. Dividing by $\eta $ proves that $\mu $ is a NSS of the game $F$. The proof that $\mu $ being a GESS implies that $\mu $ is an ESS is identical as above with strict inqualities when considering $\nu \in \P (S)\setminus \{\mu \}$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Since $\mu $ is a GESS of the game $F$, it holds that $\mu $ is a NSS of the game $F$, and therefore $\mu \in \NE (F)$ by \autoref {prop: nss_implies_nash}, as $h^F_{\nu :\mu }$ is right-continuous at $0$. For all $\nu \in \P (S)\setminus \{\mu \}$, it holds that $E_F(\nu ,\nu ) < E(\mu ,\nu )$ since $\mu $ is a GESS of the game $F$, and therefore such $\nu $ are not Nash equilibria of the game $F$. This proves that indeed $\NE (F) = \{\mu \}$.\end{proof}

\prAtEndRestatevii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}It holds that $\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$. For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}Suppose that $\mu ([0,\infty ))\subseteq \P (S)$. Let $t\in (0,\infty )$. Since $\frac {\mu (t+\epsilon ) - \mu (t)}{\epsilon }$ converges strongly to $\dot {\mu }(t)$ as $\epsilon \to 0$, it also converges weakly to $\dot {\mu }(t)$ as $\epsilon \to 0$, so \begin {equation*} \lim _{\epsilon \to 0}\int _S f d \left (\frac {\mu (t+\epsilon ) - \mu (t)}{\epsilon }\right ) = \int _S f d\dot {\mu }(t) \end {equation*} for all $f\in C(S)$. In particular, taking $f$ to be the function that is identically $1$ on $S$ yields that \begin {equation*} \lim _{\epsilon \to 0} \frac {1}{\epsilon }\left (\mu (t+\epsilon )(S) - \mu (t)(S)\right ) = \dot {\mu }(t)(S). \end {equation*} Since $\mu (t)$ and $\mu (t+\epsilon )$ are probability measures for all $\epsilon \in [-t,\infty )$, it holds that $\mu (t+\epsilon )(S) = \mu (t)(S) = 1$ for all such $\epsilon $, and hence $\frac {1}{\epsilon }\left (\mu (t+\epsilon )(S) - \mu (t)(S)\right ) = 0$ for all $\epsilon \in [-t,\infty )\setminus \{0\}$. Therefore, it must be that \begin {equation*} \dot {\mu }(t)(S) = 0, \end {equation*} so indeed $\dot {\mu }(t) \in T\P (S)$. The case for $t=0$ follows similarly.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatexi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$. Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$ for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that $\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$, and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexii}\label{thm:prAtEndxii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}Since $v$ is $\delta $-dissipative with supply rate $w\colon \M (S) \times C(S) \to \R $, there exist $\sigma \colon \P (S) \times C(S) \to \Rpl $ and $\storage \colon \P (S) \times C(S) \to \Rpl $ with $\storage $ having an appropriate extension $\overline {\storage } \colon U\times C(S) \to \R $ as in \autoref {def: delta-dissipative}. Define $V \colon \P (S) \to \Rpl $ by $V(\mu ) = \storage (\mu ,F(\mu ))$. By \autoref {prop: ne_closed} and \autoref {prop: weakly_continuous_payoff}, $\NE (F)$ is weakly compact. Thus, by \autoref {lem: lyapunov}, it suffices to show that $V$ is a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ (according to \autoref {def: lyapunov_function}). Let $\overline {V}\colon U\cap U' \to \R $ be defined by $\overline {V}(\mu ) = \overline {\storage }(\mu ,\overline {F}(\mu ))$. Note that $U\cap U'$ is strongly open and contains $\P (S)$, and that $\overline {V}$ is weakly continuous and Fr\'echet differentiable since $\overline {\storage }$ is weak-$\infty $-continuous and $\overline {F}$ is weakly continuous, and both $\overline {\storage }$ and $\overline {F}$ are Fr\'echet differentiable. Also note that $\overline {V}(\mu ) = V(\mu )$ for all $\mu \in \P (S)$. Also, if $\mu \in \NE (F)$, then $v(\mu ,F(\mu )) = 0$ by \autoref {prop: ns_implies_rest_equals_nash}, and therefore $\overline {V}(\mu ) = V(\mu ) = \storage (\mu ,F(\mu )) = 0$ by \eqref {eq: delta-dissipative-2}. Furthermore, if $\mu \in \P (S)\setminus \NE (F)$, then again by \autoref {prop: ns_implies_rest_equals_nash} we have that $v(\mu ,F(\mu )) \ne 0$, so $\overline {V}(\mu ) = V(\mu ) = \storage (\mu ,F(\mu )) > 0$ by \eqref {eq: delta-dissipative-2}. Therefore, the first two conditions from \autoref {def: lyapunov_function} on $V$ to be a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ are satisfied. \par Next, since $\overline {\storage }$ and $\overline {F}$ are Fr\'echet differentiable, \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} for all $\mu \in U\cap U'$, and therefore, since $\overline {F}(\mu ) = F(\mu )$ for all $\mu \in \P (S)$, it holds for all $\mu \in \P (S)$ that \begin {equation} \begin {aligned} D\overline {V}(\mu )v(\mu ,F(\mu )) &= \partial _1 \overline {\storage }(\mu ,F(\mu )) v(\mu , F(\mu )) + \partial _2 \overline {\storage }(\mu ,F(\mu )) D\overline {F}(\mu ) v(\mu , F(\mu )) \\ &\le -\sigma (\mu ,F(\mu )) + w(v(\mu ,F(\mu )),D\overline {F}(\mu )v(\mu ,F(\mu ))) \\ &\le -\sigma (\mu ,F(\mu )) \\ &\le 0, \end {aligned} \label {eq: decreasing_derivative} \end {equation} where the first inequality follows from \eqref {eq: delta-dissipative-1}, and the second inequality follows from \eqref {eq: supply_inequality} together with the fact that $v(\mu ,F(\mu ))\in T\P (S)$. Hence, $V$ is indeed a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$, so $\NE (F)$ is weakly Lyapunov stable under the EDM \eqref {eq: edm}. \par Now suppose that the $\delta $-dissipativity of $v$ is strict and that the additional hypotheses of \autoref {ass: game_derivative} and \autoref {ass: dynamics_map} both hold. By \autoref {lem: strict_lyapunov}, it suffices to show that $V$ is a strict global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ (according to \autoref {def: lyapunov_function}). This amounts to proving that $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous and that $D\overline {V}(\mu )v(\mu ,F(\mu )) < 0$ for all $\mu \in \P (S)\setminus \NE (F)$. Indeed, the continuity condition holds by \autoref {lem: weakly_continuous_derivative}, which we proof after completing the current proof. \par Next, if $\mu \in \P (S)\setminus \NE (F)$, then \autoref {prop: ns_implies_rest_equals_nash} gives that $v(\mu ,F(\mu )) \ne 0$ so $\sigma (\mu ,F(\mu )) > 0$ by \eqref {eq: delta-dissipative-3}, implying that $D\overline {V}(\mu )v(\mu ,F(\mu )) < 0$ for all such $\mu $ by \eqref {eq: decreasing_derivative}. Hence, $V$ is indeed a strict global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$, so $\NE (F)$ is globally weakly attracting under the EDM \eqref {eq: edm}.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexiv}\label{thm:prAtEndxiv}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiv}]\phantomsection\label{proof:prAtEndxiv}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {align*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| &\le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {align*} }{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and also since $\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$ for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\quad + \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestatexv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxv}]\phantomsection\label{proof:prAtEndxv}Let $\mu \in \P (S)$ be a Nash equilibrium of the game $F$. Then $\int _S F_\mu d\nu \le \int _S F_\mu d\mu $ for all $\nu \in \P (S)$, so by monotonicity it holds that \begin {align*} E_F(\nu ,\nu ) - E_F(\mu ,\nu ) &= \int _S F_\nu d\nu - \int _S F_\nu d\mu \\ &= \int _S F_\mu (\nu -\mu ) + \int _S(F_\nu -F_\mu )d(\nu -\mu ) \\ &\le 0 \end {align*} for all $\nu \in \P (S)$. Hence, $\mu $ is a GNSS of the game $F$. It is clear that if $\mu $ is a strict Nash equilibrium or if $F$ is strictly monotone, then the above inequality becomes strict for $\nu \in \P (S)\setminus \{\mu \}$ and hence $\mu $ is a GESS of the game $F$ in these cases.\end{proof}

\prAtEndRestatexvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxvi}]\phantomsection\label{proof:prAtEndxvi}This follows directly from \autoref {prop: monotone_nash} together with \autoref {prop: unique_gess}.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexvii}\label{thm:prAtEndxvii}\label {lem: convex_stable_set} Consider a game $F\colon \P (S)\to C(S)$ and let $N\subseteq \P (S)$ be an arbitrary set of population states. Let $\stab _N^F \subseteq \P (S)$ denote the set of all population states $\mu \in \P (S)$ such that, for all $\nu \in N$, it holds that \begin {equation*} E_F(\nu ,\nu )\le E_F(\mu ,\nu ). \end {equation*} Then, it holds that $\stab _N^F$ is a convex set.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxvii}]\phantomsection\label{proof:prAtEndxvii}It holds that \begin {align*} \stab _N^F &= \{\mu \in \P (S) : \text {$E_F(\nu ,\nu ) \le E_F(\mu ,\nu )$ for all $\nu \in N$}\} \\ &= \bigcap _{\nu \in N} \{\mu \in \P (S) : E_F(\nu ,\nu ) \le E_F(\mu ,\nu )\}. \end {align*} Since $E_F$ is linear in its first argument, the set $\{\mu \in \P (S) : E_F(\nu ,\nu ) \le E_F(\mu ,\nu )\}$ is convex for all $\nu \in N$, and therefore the set $\stab _N^F$, being the intersection of convex sets, is also a convex set.\end{proof}

\prAtEndRestatexviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxviii}]\phantomsection\label{proof:prAtEndxviii}By \autoref {prop: monotone_nash}, every Nash equilibrium of the game $F$ is a GNSS of the game $F$, and by \autoref {prop: nss_implies_nash} every GNSS of the game $F$ is a Nash equilibrium of the game $F$. Hence, the set of Nash equilibria of the game $F$ equals the set of globally neutrally stable states of the game $F$, so $\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\nu ) \le E_F(\mu ,\nu )$ for all $\nu \in \P (S)$}\}$. Applying \autoref {lem: convex_stable_set} with $N = \P (S)$ proves the claim.\end{proof}

\prAtEndRestatexix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxix}]\phantomsection\label{proof:prAtEndxix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics.} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics.} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatexx*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxx}]\phantomsection\label{proof:prAtEndxx}Suppose that $v$ is Nash stationary, $v$ is $\delta $-passive, and $F$ is monotone. Let $w\colon \M (S) \times C(S) \to \R $ be defined by $w(\mu ,\eta ) = \left <\eta ,\mu \right >$. Then it holds that $v$ is $\delta $-dissipative with supply rate $w$. Furthermore, by \autoref {lem: monotone_sde}, $F$ satisfies self-defeating externalities, and therefore \begin {equation*} w(\nu ,D\overline {F}(\mu )\nu ) = \left <D\overline {F}(\mu )\nu ,\nu \right > \le 0 ~ \text {for all $\mu \in \P (S)$ and all $\nu \in T\P (S)$.} \end {equation*} Hence, by \autoref {thm: delta-dissipative}, it holds that $\NE (F)$ is weakly Lyapunov stable under the EDM \eqref {eq: edm}. The fact that $\NE (F)$ is globally weakly attracting under the EDM \eqref {eq: edm} given the additional hypotheses of \autoref {ass: game_derivative} and \autoref {ass: dynamics_map} is immediate from \autoref {thm: delta-dissipative}.\end{proof}

\prAtEndRestatexxi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxi}]\phantomsection\label{proof:prAtEndxxi}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\prAtEndRestatexxii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxii}]\phantomsection\label{proof:prAtEndxxii}Since $v$ is $\delta $-dissipative with supply rate $w\colon \M (S) \times C(S) \to \R $, there exist $\sigma \colon \P (S) \times C(S) \to \Rpl $ and $\storage \colon \P (S) \times C(S) \to \Rpl $ with $\storage $ having an appropriate extension $\overline {\storage } \colon U\times C(S) \to \R $ as in \autoref {def: delta-dissipative}. Furthermore, since $u$ is $\delta $-antidissipative with supply rate $\tilde {w}\colon \M (S) \times C(S) \to \R $, there exist $\gamma \colon \P (S) \times C(S) \to \Rpl $ and $\Gamma \colon \P (S) \times C(S) \to \Rpl $ with $\Gamma $ having an appropriate extension $\overline {\Gamma } \colon \tilde {U}\times C(S) \to \R $ as in \autoref {def: delta-antidissipative}. Define $V \colon \P (S)\times K \to \Rpl $ by $V(\mu ,\rho ) = \storage (\mu ,\rho ) + \Gamma (\mu ,\rho )$. Consider $P = \{(\mu ,\rho ) \in \P (S) \times C(S) : v(\mu ,\rho ) = 0, ~ u(\mu ,\rho ) = 0\}$. If $(\mu ,\rho ) \in P$, then $u(\mu ,\rho ) = 0$, implying that $\rho = F(\mu )$ by $F$-payoff stationarity, and hence $v(\mu ,F(\mu )) = 0$, so $\mu \in \NE (F)$ by Nash stationarity. Thus, $P \subseteq \NE (F) \times F(\NE (F)) \subseteq \P (S) \times K$. By \autoref {prop: ne_closed} and \autoref {prop: weakly_continuous_payoff}, $\NE (F)$ is weakly compact, and hence $F(\NE (F))$ is compact as $F$ is weakly continuous. Since $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain, and $u$ is weak-$\infty $-continuous, it holds that $P = v^{-1}(\{0\})\cap u^{-1}(\{0\})$ is weak-$\infty $-closed, and hence must be weak-$\infty $-compact as well as $\NE (F) \times F(\NE (F))$ is. Thus, by \autoref {lem: lyapunov}, it suffices to show that $V$ is a global Lyapunov function for $P$ under $(\mu ,\rho ) \mapsto (v(\mu ,\rho ),u(\mu ,\rho ))$ (according to \autoref {def: lyapunov_function}). Let $\overline {V}\colon U\cap \tilde {U} \times C(S) \to \R $ be defined by $\overline {V}(\mu ,\rho ) = \overline {\storage }(\mu ,\rho ) + \overline {\Gamma }(\mu ,\rho )$. Note that $U\cap \tilde {U}$ is strongly open and contains $\P (S)$, and that $\overline {V}$ is weak-$\infty $-continuous and Fr\'echet differentiable since $\overline {\storage }$ and $\overline {\Gamma }$ are. Also note that $\overline {V}(\mu ,\rho ) = V(\mu ,\rho )$ for all $(\mu ,\rho ) \in \P (S) \times K$. Also, if $(\mu ,\rho ) \in P$, then $v(\mu ,\rho ) = 0$ and $u(\mu ,\rho ) = 0$, so $\overline {V}(\mu ,\rho ) = 0$ by \eqref {eq: delta-dissipative-2} and \eqref {eq: delta-antidissipative-2}. Furthermore, if $(\mu ,\rho ) \in (\P (S) \times K) \setminus P$, then again by \eqref {eq: delta-dissipative-2} and \eqref {eq: delta-antidissipative-2} we have that $\overline {V}(\mu ,\rho ) > 0$. Therefore, the first two conditions from \autoref {def: lyapunov_function} on $V$ to be a global Lyapunov function for $P$ under $(v,u)$ are satisfied. \par Next, it holds for all $(\mu ,\rho ) \in \P (S) \times K$ that \begin {equation} \begin {aligned} D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) &= \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu , \rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) u(\mu , \rho ) + \partial _1 \overline {\Gamma }(\mu ,\rho ) v(\mu , \rho ) + \partial _2 \overline {\Gamma }(\mu ,\rho ) u(\mu , \rho ) \\ &\le -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),u(\mu ,\rho )) - \gamma (\mu ,\rho ) - \tilde {w}(v(\mu ,\rho ),u(\mu ,\rho )) \\ &\le -\sigma (\mu ,F(\mu )) - \gamma (\mu ,\rho ) \\ &\le 0, \end {aligned} \label {eq: decreasing_derivative-dpedm} \end {equation} where the first inequality follows from \eqref {eq: delta-dissipative-1} and \eqref {eq: delta-antidissipative-1}, and the second inequality follows from the fact that $\tilde {w} \ge w$. Hence, $V$ is indeed a global Lyapunov function for $P$ under $(v,u)$, so $P$ is weak-$\infty $-Lyapunov stable under the DPEDM \eqref {eq: dpedm}. \par Now suppose that the $\delta $-dissipativity of $v$ and the $\delta $-antidissipativity of $u$ are both strict, and that $v$ is $\|\cdot \|_\TV $-bounded on $\P (S)\times K$. By \autoref {lem: strict_lyapunov}, it suffices to show that $V$ is a strict global Lyapunov function for $P$ under $(\mu ,\rho )\mapsto (v(\mu ,\rho ),u(\mu ,\rho ))$ (according to \autoref {def: lyapunov_function}). This amounts to proving that $(\mu ,\rho ) \mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weak-$\infty $-continuous and that $D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) < 0$ for all $(\mu ,\rho )\in (\P (S) \times K)\setminus P$. Indeed, the continuity condition holds by \autoref {lem: weakly_continuous_derivative-dpedm}, which we proof after completing the current proof. \par Next, if $(\mu ,\rho )\in (\P (S)\times K)\setminus P$, then $v(\mu ,\rho ) \ne 0$ or $u(\mu ,\rho ) \ne 0$, so $\sigma (\mu ,\rho ) > 0$ or $\gamma (\mu ,\rho ) > 0$ by \eqref {eq: delta-dissipative-3} and \eqref {eq: delta-antidissipative-3}, implying that $D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) < 0$ for all such $(\mu ,\rho )$ by \eqref {eq: decreasing_derivative-dpedm}. Hence, $V$ is indeed a strict global Lyapunov function for $P$ under $(v,u)$, so $P$ is globally weak-$\infty $-attracting under the DPEDM \eqref {eq: dpedm} from $K$.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexxiii}\label{thm:prAtEndxxiii}\label {lem: weakly_continuous_derivative-dpedm} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxiii}]\phantomsection\label{proof:prAtEndxxiii}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexxiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxiv}]\phantomsection\label{proof:prAtEndxxiv}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexxv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxv}]\phantomsection\label{proof:prAtEndxxv}In this proof, we denote the indicator function on a set $A \subseteq \R $ by $\chi _A \colon \R \to \R $, where \begin {equation*} \chi _A(t) = \begin {aligned} \begin {cases} 1 & \text {if $t \in A$}, \\ 0 & \text {if $t \notin A$}. \end {cases} \end {aligned} \end {equation*} \par Let $\mu ,\nu \in \P (S)$. It holds that \begin {align*} & 2 \int _S \int _S \tilde {\Theta }(s-s') d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S \tilde {\Theta }(s-s') d(\mu -\nu )(s') d(\mu -\nu )(s) + \int _S \int _S \tilde {\Theta }(s'-s) d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S \left (\tilde {\Theta }(s-s') + \tilde {\Theta }(s'-s)\right ) d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S d(\mu -\nu )(s') d(\mu -\nu )(s) \\ & \qquad = ((\mu -\nu )(S))^2 \\ & \qquad =0, \end {align*} since $(\mu -\nu )(S) = \mu (S) - \nu (S) = 0$. Therefore, \begin {equation*} \int _S \int _S \tilde {\Theta }(s-s')d(\mu -\nu )(s')d(\mu -\nu )(s) = 0. \end {equation*} Next, we note that \begin {align*} \int _S \int _S \min \{s,s'\} d\mu (s') d\nu (s) &= \int _S \int _S \int _{[0,\min \{s,s'\}]} dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{t' \in \R : t' \le \min \{s,s'\}\}}(t) dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{t' \in \R : t'\le s\}}(t) \chi _{\{t'\in \R : t\le s'\}}(t) dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s) \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s') dt d\mu (s') d\nu (s) \\ &= \int _{[0,\infty )} \int _S \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s') d\mu (s')\int _S \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s) d\nu (s) dt \\ &= \int _{[0,\infty )} \mu (S \cap [t,\infty )) \nu (S\cap [t,\infty )) dt. \end {align*} Therefore, we find that \begin {align*} & \int _S \int _S \min \{s,s'\} d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _{[0,\infty )} \left (\mu (S\cap [t,\infty ))^2 - 2\mu (S\cap [t,\infty ))\nu (S\cap [t,\infty )) + \nu (S\cap [t,\infty ))^2\right ) dt \\ &\qquad = \int _{[0,\infty )} \left (\mu (S\cap [t,\infty )) - \nu (S\cap [t,\infty ))\right )^2 dt. \end {align*} Thus, overall, it holds that \begin {align*} \left <F(\mu ) - F(\nu ), \mu -\nu \right > &= \int _S(F_\mu (s) - F_\nu (s)) d(\mu -\nu )(s) \\ &= \int _S \int _S \tilde {f}(s,s') d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &= V\int _S \int _S \tilde {\Theta }(s-s')d(\mu -\nu )(s')d(\mu -\nu )(s) - \int _S \int _S \min \{s,s'\} d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &= -\int _{[0,\infty )} \left (\mu (S\cap [t,\infty )) - \nu (S\cap [t,\infty ))\right )^2 dt \\ &\le 0. \end {align*} Hence, $F$ is monotone.\end{proof}

\prAtEndRestatexxvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxvi}]\phantomsection\label{proof:prAtEndxxvi}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {prop: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-figure5-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable, and hence this is a sequential space. Therefore, $\P (S)$ is weakly closed if and only if it is weakly sequentially closed. It is clear that if $\{\mu _n \in \P (S) : n\in \N \}$ is a sequence in $\P (S)$ that weakly converges to $\mu \in \M (S)$, then $\mu \in \P (S)$ since it must be nonnegative and since the constant function $1$ is an element of $C(S)$. Hence, $\P (S)$ is weakly closed. By the Banach-Alaoglu theorem, the unit ball $\{\mu \in \M (S) : \|\mu \|_\TV \le 1\}$ is weak-$*$ compact and hence weakly compact as these two topologies coincide since $S$ is compact. Thus, the weakly closed subset $\P (S)$ of the weakly compact unit ball must also be weakly compact.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Let $\mu \in \P (S)$ be a NSS of the game $F\colon \P (S)\to C(S)$. Suppose that $h^F_{\nu :\mu }$ is right-continuous at $0$ for all $\nu \in \P (S)$. Let $\nu \in \P (S)$. Then, there exists $\epsilon (\nu )\in (0,1]$ such that \begin {equation*} h^F_{\nu :\mu }(\eta ) = E_F(\nu ,(1-\eta )\mu +\eta \nu ) - E_F(\mu ,(1-\eta )\mu +\eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,\epsilon (\nu )]$. Thus, by the right-continuity of $h^F_{\nu :\mu }$, it holds that \begin {equation*} E_F(\nu ,\mu )-E_F(\mu ,\mu ) = h^F_{\nu :\mu }(0) = \lim _{\eta \downarrow 0} h^F_{\nu :\mu }(\eta ) \le 0. \end {equation*} Since $\nu $ is arbitrary, this proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $\mu \in \P (S)$ is a GNSS of the game $F\colon \P (S)\to C(S)$. Let $\nu \in \P (S)$. Then, since $\mu $ is a GNSS of the game $F$, it holds that \begin {equation*} E_F((1-\eta )\mu +\eta \nu ,(1-\eta )\mu + \eta \nu ) - E_F(\mu ,(1-\eta )\mu +\eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,1]$. By linearity of $E_F$ in its first argument, we find that \begin {equation*} \eta E_F(\nu ,(1-\eta ) \mu + \eta \nu ) - \eta E_F(\mu ,(1-\eta ) \mu + \eta \nu ) \le 0 \end {equation*} for all $\eta \in (0,1]$. Dividing by $\eta $ proves that $\mu $ is a NSS of the game $F$. The proof that $\mu $ being a GESS implies that $\mu $ is an ESS is identical as above with strict inqualities when considering $\nu \in \P (S)\setminus \{\mu \}$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Since $\mu $ is a GESS of the game $F$, it holds that $\mu $ is a NSS of the game $F$, and therefore $\mu \in \NE (F)$ by \autoref {prop: nss_implies_nash}, as $h^F_{\nu :\mu }$ is right-continuous at $0$. For all $\nu \in \P (S)\setminus \{\mu \}$, it holds that $E_F(\nu ,\nu ) < E(\mu ,\nu )$ since $\mu $ is a GESS of the game $F$, and therefore such $\nu $ are not Nash equilibria of the game $F$. This proves that indeed $\NE (F) = \{\mu \}$.\end{proof}

\prAtEndRestatevii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}It holds that $\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$. For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}Suppose that $\mu ([0,\infty ))\subseteq \P (S)$. Let $t\in (0,\infty )$. Since $\frac {\mu (t+\epsilon ) - \mu (t)}{\epsilon }$ converges strongly to $\dot {\mu }(t)$ as $\epsilon \to 0$, it also converges weakly to $\dot {\mu }(t)$ as $\epsilon \to 0$, so \begin {equation*} \lim _{\epsilon \to 0}\int _S f d \left (\frac {\mu (t+\epsilon ) - \mu (t)}{\epsilon }\right ) = \int _S f d\dot {\mu }(t) \end {equation*} for all $f\in C(S)$. In particular, taking $f$ to be the function that is identically $1$ on $S$ yields that \begin {equation*} \lim _{\epsilon \to 0} \frac {1}{\epsilon }\left (\mu (t+\epsilon )(S) - \mu (t)(S)\right ) = \dot {\mu }(t)(S). \end {equation*} Since $\mu (t)$ and $\mu (t+\epsilon )$ are probability measures for all $\epsilon \in [-t,\infty )$, it holds that $\mu (t+\epsilon )(S) = \mu (t)(S) = 1$ for all such $\epsilon $, and hence $\frac {1}{\epsilon }\left (\mu (t+\epsilon )(S) - \mu (t)(S)\right ) = 0$ for all $\epsilon \in [-t,\infty )\setminus \{0\}$. Therefore, it must be that \begin {equation*} \dot {\mu }(t)(S) = 0, \end {equation*} so indeed $\dot {\mu }(t) \in T\P (S)$. The case for $t=0$ follows similarly.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatexi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$. Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$ for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that $\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$, and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexii}\label{thm:prAtEndxii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}Since $v$ is $\delta $-dissipative with supply rate $w\colon \M (S) \times C(S) \to \R $, there exist $\sigma \colon \P (S) \times C(S) \to \Rpl $ and $\storage \colon \P (S) \times C(S) \to \Rpl $ with $\storage $ having an appropriate extension $\overline {\storage } \colon U\times C(S) \to \R $ as in \autoref {def: delta-dissipative}. Define $V \colon \P (S) \to \Rpl $ by $V(\mu ) = \storage (\mu ,F(\mu ))$. By \autoref {prop: ne_closed} and \autoref {prop: weakly_continuous_payoff}, $\NE (F)$ is weakly compact. Thus, by \autoref {lem: lyapunov}, it suffices to show that $V$ is a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ (according to \autoref {def: lyapunov_function}). Let $\overline {V}\colon U\cap U' \to \R $ be defined by $\overline {V}(\mu ) = \overline {\storage }(\mu ,\overline {F}(\mu ))$. Note that $U\cap U'$ is strongly open and contains $\P (S)$, and that $\overline {V}$ is weakly continuous and Fr\'echet differentiable since $\overline {\storage }$ is weak-$\infty $-continuous and $\overline {F}$ is weakly continuous, and both $\overline {\storage }$ and $\overline {F}$ are Fr\'echet differentiable. Also note that $\overline {V}(\mu ) = V(\mu )$ for all $\mu \in \P (S)$. Also, if $\mu \in \NE (F)$, then $v(\mu ,F(\mu )) = 0$ by \autoref {prop: ns_implies_rest_equals_nash}, and therefore $\overline {V}(\mu ) = V(\mu ) = \storage (\mu ,F(\mu )) = 0$ by \eqref {eq: delta-dissipative-2}. Furthermore, if $\mu \in \P (S)\setminus \NE (F)$, then again by \autoref {prop: ns_implies_rest_equals_nash} we have that $v(\mu ,F(\mu )) \ne 0$, so $\overline {V}(\mu ) = V(\mu ) = \storage (\mu ,F(\mu )) > 0$ by \eqref {eq: delta-dissipative-2}. Therefore, the first two conditions from \autoref {def: lyapunov_function} on $V$ to be a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ are satisfied. \par Next, since $\overline {\storage }$ and $\overline {F}$ are Fr\'echet differentiable, \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} for all $\mu \in U\cap U'$, and therefore, since $\overline {F}(\mu ) = F(\mu )$ for all $\mu \in \P (S)$, it holds for all $\mu \in \P (S)$ that \begin {equation} \begin {aligned} D\overline {V}(\mu )v(\mu ,F(\mu )) &= \partial _1 \overline {\storage }(\mu ,F(\mu )) v(\mu , F(\mu )) + \partial _2 \overline {\storage }(\mu ,F(\mu )) D\overline {F}(\mu ) v(\mu , F(\mu )) \\ &\le -\sigma (\mu ,F(\mu )) + w(v(\mu ,F(\mu )),D\overline {F}(\mu )v(\mu ,F(\mu ))) \\ &\le -\sigma (\mu ,F(\mu )) \\ &\le 0, \end {aligned} \label {eq: decreasing_derivative} \end {equation} where the first inequality follows from \eqref {eq: delta-dissipative-1}, and the second inequality follows from \eqref {eq: supply_inequality} together with the fact that $v(\mu ,F(\mu ))\in T\P (S)$. Hence, $V$ is indeed a global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$, so $\NE (F)$ is weakly Lyapunov stable under the EDM \eqref {eq: edm}. \par Now suppose that the $\delta $-dissipativity of $v$ is strict and that the additional hypotheses of \autoref {ass: game_derivative} and \autoref {ass: dynamics_map} both hold. By \autoref {lem: strict_lyapunov}, it suffices to show that $V$ is a strict global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$ (according to \autoref {def: lyapunov_function}). This amounts to proving that $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous and that $D\overline {V}(\mu )v(\mu ,F(\mu )) < 0$ for all $\mu \in \P (S)\setminus \NE (F)$. Indeed, the continuity condition holds by \autoref {lem: weakly_continuous_derivative}, which we proof after completing the current proof. \par Next, if $\mu \in \P (S)\setminus \NE (F)$, then \autoref {prop: ns_implies_rest_equals_nash} gives that $v(\mu ,F(\mu )) \ne 0$ so $\sigma (\mu ,F(\mu )) > 0$ by \eqref {eq: delta-dissipative-3}, implying that $D\overline {V}(\mu )v(\mu ,F(\mu )) < 0$ for all such $\mu $ by \eqref {eq: decreasing_derivative}. Hence, $V$ is indeed a strict global Lyapunov function for $\NE (F)$ under $\mu \mapsto v(\mu ,F(\mu ))$, so $\NE (F)$ is globally weakly attracting under the EDM \eqref {eq: edm}.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexiv}\label{thm:prAtEndxiv}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiv}]\phantomsection\label{proof:prAtEndxiv}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {align*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| &\le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {align*} }{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and also since $\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$ for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\quad + \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestatexv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxv}]\phantomsection\label{proof:prAtEndxv}Let $\mu \in \P (S)$ be a Nash equilibrium of the game $F$. Then $\int _S F_\mu d\nu \le \int _S F_\mu d\mu $ for all $\nu \in \P (S)$, so by monotonicity it holds that \begin {align*} E_F(\nu ,\nu ) - E_F(\mu ,\nu ) &= \int _S F_\nu d\nu - \int _S F_\nu d\mu \\ &= \int _S F_\mu (\nu -\mu ) + \int _S(F_\nu -F_\mu )d(\nu -\mu ) \\ &\le 0 \end {align*} for all $\nu \in \P (S)$. Hence, $\mu $ is a GNSS of the game $F$. It is clear that if $\mu $ is a strict Nash equilibrium or if $F$ is strictly monotone, then the above inequality becomes strict for $\nu \in \P (S)\setminus \{\mu \}$ and hence $\mu $ is a GESS of the game $F$ in these cases.\end{proof}

\prAtEndRestatexvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxvi}]\phantomsection\label{proof:prAtEndxvi}This follows directly from \autoref {prop: monotone_nash} together with \autoref {prop: unique_gess}.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexvii}\label{thm:prAtEndxvii}\label {lem: convex_stable_set} Consider a game $F\colon \P (S)\to C(S)$ and let $N\subseteq \P (S)$ be an arbitrary set of population states. Let $\stab _N^F \subseteq \P (S)$ denote the set of all population states $\mu \in \P (S)$ such that, for all $\nu \in N$, it holds that \begin {equation*} E_F(\nu ,\nu )\le E_F(\mu ,\nu ). \end {equation*} Then, it holds that $\stab _N^F$ is a convex set.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxvii}]\phantomsection\label{proof:prAtEndxvii}It holds that \begin {align*} \stab _N^F &= \{\mu \in \P (S) : \text {$E_F(\nu ,\nu ) \le E_F(\mu ,\nu )$ for all $\nu \in N$}\} \\ &= \bigcap _{\nu \in N} \{\mu \in \P (S) : E_F(\nu ,\nu ) \le E_F(\mu ,\nu )\}. \end {align*} Since $E_F$ is linear in its first argument, the set $\{\mu \in \P (S) : E_F(\nu ,\nu ) \le E_F(\mu ,\nu )\}$ is convex for all $\nu \in N$, and therefore the set $\stab _N^F$, being the intersection of convex sets, is also a convex set.\end{proof}

\prAtEndRestatexviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxviii}]\phantomsection\label{proof:prAtEndxviii}By \autoref {prop: monotone_nash}, every Nash equilibrium of the game $F$ is a GNSS of the game $F$, and by \autoref {prop: nss_implies_nash} every GNSS of the game $F$ is a Nash equilibrium of the game $F$. Hence, the set of Nash equilibria of the game $F$ equals the set of globally neutrally stable states of the game $F$, so $\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\nu ) \le E_F(\mu ,\nu )$ for all $\nu \in \P (S)$}\}$. Applying \autoref {lem: convex_stable_set} with $N = \P (S)$ proves the claim.\end{proof}

\prAtEndRestatexix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxix}]\phantomsection\label{proof:prAtEndxix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics.} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics.} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatexx*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxx}]\phantomsection\label{proof:prAtEndxx}Suppose that $v$ is Nash stationary, $v$ is $\delta $-passive, and $F$ is monotone. Let $w\colon \M (S) \times C(S) \to \R $ be defined by $w(\mu ,\eta ) = \left <\eta ,\mu \right >$. Then it holds that $v$ is $\delta $-dissipative with supply rate $w$. Furthermore, by \autoref {lem: monotone_sde}, $F$ satisfies self-defeating externalities, and therefore \begin {equation*} w(\nu ,D\overline {F}(\mu )\nu ) = \left <D\overline {F}(\mu )\nu ,\nu \right > \le 0 ~ \text {for all $\mu \in \P (S)$ and all $\nu \in T\P (S)$.} \end {equation*} Hence, by \autoref {thm: delta-dissipative}, it holds that $\NE (F)$ is weakly Lyapunov stable under the EDM \eqref {eq: edm}. The fact that $\NE (F)$ is globally weakly attracting under the EDM \eqref {eq: edm} given the additional hypotheses of \autoref {ass: game_derivative} and \autoref {ass: dynamics_map} is immediate from \autoref {thm: delta-dissipative}.\end{proof}

\prAtEndRestatexxi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxi}]\phantomsection\label{proof:prAtEndxxi}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\prAtEndRestatexxii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxii}]\phantomsection\label{proof:prAtEndxxii}Since $v$ is $\delta $-dissipative with supply rate $w\colon \M (S) \times C(S) \to \R $, there exist $\sigma \colon \P (S) \times C(S) \to \Rpl $ and $\storage \colon \P (S) \times C(S) \to \Rpl $ with $\storage $ having an appropriate extension $\overline {\storage } \colon U\times C(S) \to \R $ as in \autoref {def: delta-dissipative}. Furthermore, since $u$ is $\delta $-antidissipative with supply rate $\tilde {w}\colon \M (S) \times C(S) \to \R $, there exist $\gamma \colon \P (S) \times C(S) \to \Rpl $ and $\Gamma \colon \P (S) \times C(S) \to \Rpl $ with $\Gamma $ having an appropriate extension $\overline {\Gamma } \colon \tilde {U}\times C(S) \to \R $ as in \autoref {def: delta-antidissipative}. Define $V \colon \P (S)\times K \to \Rpl $ by $V(\mu ,\rho ) = \storage (\mu ,\rho ) + \Gamma (\mu ,\rho )$. Consider $P = \{(\mu ,\rho ) \in \P (S) \times C(S) : v(\mu ,\rho ) = 0, ~ u(\mu ,\rho ) = 0\}$. If $(\mu ,\rho ) \in P$, then $u(\mu ,\rho ) = 0$, implying that $\rho = F(\mu )$ by $F$-payoff stationarity, and hence $v(\mu ,F(\mu )) = 0$, so $\mu \in \NE (F)$ by Nash stationarity. Thus, $P \subseteq \NE (F) \times F(\NE (F)) \subseteq \P (S) \times K$. By \autoref {prop: ne_closed} and \autoref {prop: weakly_continuous_payoff}, $\NE (F)$ is weakly compact, and hence $F(\NE (F))$ is compact as $F$ is weakly continuous. Since $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain, and $u$ is weak-$\infty $-continuous, it holds that $P = v^{-1}(\{0\})\cap u^{-1}(\{0\})$ is weak-$\infty $-closed, and hence must be weak-$\infty $-compact as well as $\NE (F) \times F(\NE (F))$ is. Thus, by \autoref {lem: lyapunov}, it suffices to show that $V$ is a global Lyapunov function for $P$ under $(\mu ,\rho ) \mapsto (v(\mu ,\rho ),u(\mu ,\rho ))$ (according to \autoref {def: lyapunov_function}). Let $\overline {V}\colon U\cap \tilde {U} \times C(S) \to \R $ be defined by $\overline {V}(\mu ,\rho ) = \overline {\storage }(\mu ,\rho ) + \overline {\Gamma }(\mu ,\rho )$. Note that $U\cap \tilde {U}$ is strongly open and contains $\P (S)$, and that $\overline {V}$ is weak-$\infty $-continuous and Fr\'echet differentiable since $\overline {\storage }$ and $\overline {\Gamma }$ are. Also note that $\overline {V}(\mu ,\rho ) = V(\mu ,\rho )$ for all $(\mu ,\rho ) \in \P (S) \times K$. Also, if $(\mu ,\rho ) \in P$, then $v(\mu ,\rho ) = 0$ and $u(\mu ,\rho ) = 0$, so $\overline {V}(\mu ,\rho ) = 0$ by \eqref {eq: delta-dissipative-2} and \eqref {eq: delta-antidissipative-2}. Furthermore, if $(\mu ,\rho ) \in (\P (S) \times K) \setminus P$, then again by \eqref {eq: delta-dissipative-2} and \eqref {eq: delta-antidissipative-2} we have that $\overline {V}(\mu ,\rho ) > 0$. Therefore, the first two conditions from \autoref {def: lyapunov_function} on $V$ to be a global Lyapunov function for $P$ under $(v,u)$ are satisfied. \par Next, it holds for all $(\mu ,\rho ) \in \P (S) \times K$ that \begin {equation} \begin {aligned} D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) &= \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu , \rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) u(\mu , \rho ) + \partial _1 \overline {\Gamma }(\mu ,\rho ) v(\mu , \rho ) + \partial _2 \overline {\Gamma }(\mu ,\rho ) u(\mu , \rho ) \\ &\le -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),u(\mu ,\rho )) - \gamma (\mu ,\rho ) - \tilde {w}(v(\mu ,\rho ),u(\mu ,\rho )) \\ &\le -\sigma (\mu ,F(\mu )) - \gamma (\mu ,\rho ) \\ &\le 0, \end {aligned} \label {eq: decreasing_derivative-dpedm} \end {equation} where the first inequality follows from \eqref {eq: delta-dissipative-1} and \eqref {eq: delta-antidissipative-1}, and the second inequality follows from the fact that $\tilde {w} \ge w$. Hence, $V$ is indeed a global Lyapunov function for $P$ under $(v,u)$, so $P$ is weak-$\infty $-Lyapunov stable under the DPEDM \eqref {eq: dpedm}. \par Now suppose that the $\delta $-dissipativity of $v$ and the $\delta $-antidissipativity of $u$ are both strict, and that $v$ is $\|\cdot \|_\TV $-bounded on $\P (S)\times K$. By \autoref {lem: strict_lyapunov}, it suffices to show that $V$ is a strict global Lyapunov function for $P$ under $(\mu ,\rho )\mapsto (v(\mu ,\rho ),u(\mu ,\rho ))$ (according to \autoref {def: lyapunov_function}). This amounts to proving that $(\mu ,\rho ) \mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weak-$\infty $-continuous and that $D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) < 0$ for all $(\mu ,\rho )\in (\P (S) \times K)\setminus P$. Indeed, the continuity condition holds by \autoref {lem: weakly_continuous_derivative-dpedm}, which we proof after completing the current proof. \par Next, if $(\mu ,\rho )\in (\P (S)\times K)\setminus P$, then $v(\mu ,\rho ) \ne 0$ or $u(\mu ,\rho ) \ne 0$, so $\sigma (\mu ,\rho ) > 0$ or $\gamma (\mu ,\rho ) > 0$ by \eqref {eq: delta-dissipative-3} and \eqref {eq: delta-antidissipative-3}, implying that $D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho )) < 0$ for all such $(\mu ,\rho )$ by \eqref {eq: decreasing_derivative-dpedm}. Hence, $V$ is indeed a strict global Lyapunov function for $P$ under $(v,u)$, so $P$ is globally weak-$\infty $-attracting under the DPEDM \eqref {eq: dpedm} from $K$.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexxiii}\label{thm:prAtEndxxiii}\label {lem: weakly_continuous_derivative-dpedm} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxiii}]\phantomsection\label{proof:prAtEndxxiii}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexxiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxiv}]\phantomsection\label{proof:prAtEndxxiv}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexxv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxv}]\phantomsection\label{proof:prAtEndxxv}In this proof, we denote the indicator function on a set $A \subseteq \R $ by $\chi _A \colon \R \to \R $, where \begin {equation*} \chi _A(t) = \begin {aligned} \begin {cases} 1 & \text {if $t \in A$}, \\ 0 & \text {if $t \notin A$}. \end {cases} \end {aligned} \end {equation*} \par Let $\mu ,\nu \in \P (S)$. It holds that \begin {align*} & 2 \int _S \int _S \tilde {\Theta }(s-s') d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S \tilde {\Theta }(s-s') d(\mu -\nu )(s') d(\mu -\nu )(s) + \int _S \int _S \tilde {\Theta }(s'-s) d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S \left (\tilde {\Theta }(s-s') + \tilde {\Theta }(s'-s)\right ) d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _S \int _S d(\mu -\nu )(s') d(\mu -\nu )(s) \\ & \qquad = ((\mu -\nu )(S))^2 \\ & \qquad =0, \end {align*} since $(\mu -\nu )(S) = \mu (S) - \nu (S) = 0$. Therefore, \begin {equation*} \int _S \int _S \tilde {\Theta }(s-s')d(\mu -\nu )(s')d(\mu -\nu )(s) = 0. \end {equation*} Next, we note that \begin {align*} \int _S \int _S \min \{s,s'\} d\mu (s') d\nu (s) &= \int _S \int _S \int _{[0,\min \{s,s'\}]} dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{t' \in \R : t' \le \min \{s,s'\}\}}(t) dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{t' \in \R : t'\le s\}}(t) \chi _{\{t'\in \R : t\le s'\}}(t) dt d\mu (s') d\nu (s) \\ &= \int _S \int _S \int _{[0,\infty )} \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s) \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s') dt d\mu (s') d\nu (s) \\ &= \int _{[0,\infty )} \int _S \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s') d\mu (s')\int _S \chi _{\{\tilde {s} \in S : \tilde {s} \ge t\}}(s) d\nu (s) dt \\ &= \int _{[0,\infty )} \mu (S \cap [t,\infty )) \nu (S\cap [t,\infty )) dt. \end {align*} Therefore, we find that \begin {align*} & \int _S \int _S \min \{s,s'\} d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &\qquad = \int _{[0,\infty )} \left (\mu (S\cap [t,\infty ))^2 - 2\mu (S\cap [t,\infty ))\nu (S\cap [t,\infty )) + \nu (S\cap [t,\infty ))^2\right ) dt \\ &\qquad = \int _{[0,\infty )} \left (\mu (S\cap [t,\infty )) - \nu (S\cap [t,\infty ))\right )^2 dt. \end {align*} Thus, overall, it holds that \begin {align*} \left <F(\mu ) - F(\nu ), \mu -\nu \right > &= \int _S(F_\mu (s) - F_\nu (s)) d(\mu -\nu )(s) \\ &= \int _S \int _S \tilde {f}(s,s') d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &= V\int _S \int _S \tilde {\Theta }(s-s')d(\mu -\nu )(s')d(\mu -\nu )(s) - \int _S \int _S \min \{s,s'\} d(\mu -\nu )(s') d(\mu -\nu )(s) \\ &= -\int _{[0,\infty )} \left (\mu (S\cap [t,\infty )) - \nu (S\cap [t,\infty ))\right )^2 dt \\ &\le 0. \end {align*} Hence, $F$ is monotone.\end{proof}

\prAtEndRestatexxvi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxxvi}]\phantomsection\label{proof:prAtEndxxvi}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {prop: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure0-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure1-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure10-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure11-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure12-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure13-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure2-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure3-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure4-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure5-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure6-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure7-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure8-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-long_version-figure9-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Suppose that the third condition holds, so that $F_\mu (s) \le F_\mu (s')$ for all $s\in S$ and all $s' \in \supp (\mu )$. Then, for all $s\in S$, it holds that $E_F(\delta _s,\mu ) = F_\mu (s) \le F_\mu (s')$ for all $s'\in \supp (\mu )$ and consequently that $E_F(\delta _s,\mu ) = \int _S F_\mu (s) d\mu (s') \le \int _S F_\mu (s') d\mu (s') = E_F(\mu ,\mu )$. Thus, the second condition holds. Furthermore, if $\nu \in \P (S)$, then $E_F(\nu ,\mu ) = \int _S F_\mu (s) d\nu (s) = \int _S E_F(\delta _s,\mu ) d\nu (s) \le \int _S E_F(\mu ,\mu ) d\nu (s) = E_F(\mu ,\mu )$, so the first condition holds as well. \par To complete the proof, we show that the first condition implies the third. Suppose that the first condition holds, so that $E_F(\nu ,\mu ) \le E_F(\mu ,\mu )$ for all $\nu \in \P (S)$. Notice that $\sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) \le E_F(\mu ,\mu )$, and also that \begin {align*} \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) &= \int _S \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu )\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} E_F(\delta _{s'},\mu ) d\mu (s') \\ &= \int _S F_\mu (s') d\mu (s') \\ &= E_F(\mu ,\mu ). \end {align*} Hence, $\sup _{s\in \supp (\mu )}E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $E_F(\delta _{s'},\mu ) < \sup _{s\in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$. Since $F_\mu $ is a continuous real-valued function on $S$, the preimage $U \coloneqq F_\mu ^{-1}((-\infty ,E_F(\mu ,\mu ))) = \{s\in S : F_\mu (s) < E_F(\mu ,\mu )\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= E_F(\mu ,\mu ) - E_F(\mu ,\mu ) \\ &= \int _S (E_F(\mu ,\mu ) - F_\mu (s)) d\mu (s) \\ &= \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) + \int _{S\setminus U}(E_F(\mu ,\mu ) - E_F(\delta _s,\mu ))d\mu (s) \\ &\ge \int _U (E_F(\mu ,\mu ) - F_\mu (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $E_F(\delta _{s'},\mu ) = \sup _{s \in \supp (\mu )} E_F(\delta _s,\mu ) = E_F(\mu ,\mu )$ for all $s'\in \supp (\mu )$. Therefore, $F_\mu (s') = E_F(\delta _{s'},\mu ) = E_F(\mu ,\mu ) \ge E_F(\nu ,\mu )$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $F_\mu (s') \ge E_F(\delta _s,\mu ) = F_\mu (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$, so the third condition holds.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It holds that \iftoggle {thesis}{ \begin {align*} \NE (F) &= \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} \\ &= \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}. \end {align*} }{$\NE (F) = \{\mu \in \P (S) : \text {$E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$ for all $\nu \in \P (S)$}\} = \bigcap _{\nu \in \P (S)}\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$.} For all $\nu \in \P (S)$, the set $\{\mu \in \P (S) : E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0\}$ is the preimage of the closed set $(-\infty ,0]$ under the map $\theta _\nu $. Hence, if this map is weakly continuous, then $\NE (F)$ is weakly closed. Since $\P (S)$ is weakly compact by \autoref {lem: P(S)_compact}, the weakly closed subset $\NE (F) \subseteq \P (S)$ must also be weakly compact.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Suppose that $F$ is weakly continuous and let $\nu \in \P (S)$. Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that $\theta _\nu $ is weakly sequentially continuous. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {thesis}{ \begin {align*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| &= |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| \\ &= |\left <F(\mu _n)-F(\mu ),\nu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \\ &\to 0 \end {align*} }{ \begin {equation*} |E_F(\nu ,\mu _n) - E_F(\nu ,\mu )| = |\left <F(\mu _n),\nu \right > - \left <F(\mu ),\nu \right >| = |\left <F(\mu _n)-F(\mu ),\nu \right >| \le \|F(\mu _n) - F(\mu )\|_\infty \|\nu \|_\TV \to 0 \end {equation*} } since $\|\nu \|_\TV = 1$ and $F(\mu _n) \to F(\mu )$ in $C(S)$ with the topology induced by $\|\cdot \|_\infty $ due to weak continuity of $F$. Furthermore, we have that \begin {align*} |E_F(\mu _n,\mu _n) - E_F(\mu ,\mu )| &= |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &\le |\left <F(\mu _n),\mu _n\right > - \left <F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n\right > - \left <F(\mu ),\mu \right >| \\ &= |\left <F(\mu _n) - F(\mu ),\mu _n\right >| + |\left <F(\mu ),\mu _n - \mu \right >| \\ &\le \|F(\mu _n) - F(\mu )\|_\infty \|\mu _n\|_\TV + |\left <F(\mu ),\mu _n - \mu \right >| \\ &= \|F(\mu _n) - F(\mu )\|_\infty + |\left <F(\mu ),\mu _n-\mu \right >| \\ &\to 0 \end {align*} since again $F(\mu _n) \to F(\mu )$ by weak continuity of $F$, and since $\left <F(\mu ),\mu _n - \mu \right > \to 0$ by definition of weak convergence of $\mu _n$ to $\mu $. Therefore, we conclude that \begin {equation*} \theta _\nu (\mu _n) = E_F(\nu ,\mu _n) - E_F(\mu _n,\mu _n) \to E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \theta _\nu (\mu ), \end {equation*} which proves the claim.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $v$ is Nash stationary. Let $\mu \in \P (S)$ be a rest point of the EDM \eqref {eq: edm} with dynamics map $v$. Then $v(\mu ,F(\mu )) = 0$. Since $v$ is Nash stationary, this implies that $E_F(\nu ,\mu ) - E_F(\mu ,\mu ) = \left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > \le 0$ for all $\nu \in \P (S)$. Thus, $\mu \in \NE (F)$. On the other hand, if $\mu \in \NE (F)$, then $\left <F(\mu ),\nu \right > - \left <F(\mu ),\mu \right > = E_F(\nu ,\mu ) - E_F(\mu ,\mu ) \le 0$, so $v(\mu ,F(\mu ))=0$ since $v$ is Nash stationary. Thus, $\mu $ is a rest point of the EDM \eqref {eq: edm} with dynamics map $v$.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Let $\mu \in \P (S)$ and let $\rho \in C(S)$. First consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $B\in \B (S)$. If $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then it follows immediately that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and hence $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. \iftoggle {thesis}{Suppose that $$\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0.$$}{Suppose that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0$.} Then we find that \begin {equation*} \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) = 0 \end {equation*} for all $B\in \B (S)$. Hence, $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for $\lambda $-almost every $s\in S$. Since $\lambda $ has full support by assumption and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ is continuous, this shows that $\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} = 0$ for all $s\in S$. Hence, $\left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Since $S$ is compact and $\rho $ is continuous, the optimization $\sup _{s\in S}\rho (s)$ is attained by some $s'\in S$. Therefore, for all $\nu \in \P (S)$ it holds that $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \rho (s') d\nu (s) = \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right >$. Now suppose that the other case holds, namely, that $\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) > 0$. Then it holds that \begin {equation*} \mu (B) = \int _B \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \end {equation*} for all $B\in \B (S)$. Suppose for the sake of contradiction that there exists $\tilde {s}\in S$ such that $\left <\rho ,\delta _{\tilde {s}}\right > - \left <\rho ,\mu \right > > 0$. Then, by continuity of $s'\mapsto \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >$, the preimage $\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}$ is open and contains $\tilde {s}$, and hence it must be the case that $\lambda (\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}) > 0$ by definition of $\supp (\lambda )$ and the fact that $\lambda $ has full support. Therefore, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} \left <\rho ,\mu \right > &= \int _S \rho d\mu \\ &= \int _S \rho (s') \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\delta _{s'}\right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right >- \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &> \int _{\{s'\in S : \left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right > > 0\}} \left <\rho ,\mu \right > \frac {\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\}}{\int _S \max \{0,\left <\rho ,\delta _{s}\right > - \left <\rho ,\mu \right >\} d\lambda (s)} d\lambda (s') \\ &= \left <\rho ,\mu \right >, \end {align*} which is a contradiction. Hence, it must be that $\left <\rho ,\delta _{\tilde {s}}\right > \le \left <\rho ,\mu \right >$ for all $\tilde {s}\in S$. Arguing as in the prior case, this yields that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Since this exhausts all cases to be considered, we conclude that indeed $v$ is Nash stationary. \par Now consider the pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _S \int _B \gamma (s,s',\rho )d\lambda (s') d\mu (s) - \int _S\int _B \gamma (s',s,\rho ) d\mu (s') d\lambda (s) \end {equation*} for all $B\in \B (S)$. By \autoref {lem: equivalent_nash-general}, which we prove after completing the current proof, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Thus, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then $\max \{0,\rho (s) - \rho (s')\} = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$, implying that $\sign (\max \{0,\rho (s) - \rho (s')\}) = 0$ for all $s\in S$ and all $s'\in \supp (\mu )$. Hence, since the conditional switch rate $\gamma $ satisfies sign-preservation by assumption, we find that \begin {equation*} \sign (\gamma (s',s,\rho )) = 0 \end {equation*} for all $s\in S$ and all $s'\in \supp (\mu )$. This implies that $v(\mu ,\rho )(B) = 0$ for all $B\in \B (S)$, and therefore that $v(\mu ,\rho ) = 0$. \par On the other hand, suppose that $v(\mu ,\rho ) = 0$. Define the measures $v_1(\mu ,\rho ),v_2(\mu ,\rho )\in \M (S)$ by \begin {align*} v_1(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s,s',\rho ) d\lambda (s')d\mu (s) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s'), \\ v_2(\mu ,\rho )(B) &\coloneqq \int _S \int _B \gamma (s',s,\rho ) d\mu (s')d\lambda (s) = \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {align*} so that $v(\mu ,\rho ) = v_1(\mu ,\rho ) - v_2(\mu ,\rho )$. Since $v(\mu ,\rho ) = 0$, it holds that $v_1(\mu ,\rho ) = v_2(\mu ,\rho )$, and hence $\left <\rho ,v_1(\mu ,\rho )\right > = \left <\rho ,v_2(\mu ,\rho )\right >$. Therefore, \begin {equation*} \int _S \rho (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S \rho (s') \int _S \gamma (s',s,\rho )d\lambda (s) d\mu (s'). \end {equation*} Hence, \begin {equation*} \int _S\int _S \rho (s') \gamma (s,s',\rho ) d\mu (s) d\lambda (s') = \int _S\int _S \rho (s') \gamma (s',s,\rho ) d\lambda (s) d\mu (s'), \end {equation*} implying that \begin {equation*} \int _S \int _S (\rho (s) - \rho (s')) \gamma (s',s,\rho ) d\mu (s') d\lambda (s) = 0. \end {equation*} By sign-preservation of the conditional switch rate $\gamma $, it holds that \iftoggle {thesis}{$$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$$}{$\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s) - \rho (s')\})$} for all $s,s'\in S$, and therefore, if $\rho (s) \ge \rho (s')$, we find that $\gamma (s',s,\rho ) \ge 0$ so that $(\rho (s)-\rho (s'))\gamma (s',s,\rho ) \ge 0$, and similarly if $\rho (s) \le \rho (s')$, we find that $\gamma (s',s,\rho ) = 0$ so that $(\rho (s) - \rho (s'))\gamma (s',s,\rho )=0$. Hence, $(\rho (s) - \rho (s'))\gamma (s',s,\rho ) \ge 0$ for all $s,s'\in S$, and also $\int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho )d\mu (s') \ge 0$ for all $s\in S$. Since $s\mapsto \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s')$ is continuous (which follows from compactness of $S$ and continuity of $s'\mapsto (\rho (s)-\rho (s'))\gamma (s',s,\rho )$, together with the dominated convergence theorem), the preimage $\{s\in S : \int _S(\rho (s)-\rho (s'))\gamma (s',s,\rho )d\mu (s') > 0\}$ is open and therefore must be empty, for otherwise $\int _S \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') d\lambda (s) > 0$ as $\lambda $ has full support. Hence, \begin {equation*} \int _S (\rho (s) - \rho (s'))\gamma (s',s,\rho ) d\mu (s') = 0 ~ \text {for all $s\in S$}. \end {equation*} Similarly, since $s' \mapsto (\rho (s) - \rho (s'))\gamma (s',s,\rho )$ is continuous for all $s\in S$, the preimage $\{s'\in S : (\rho (s) - \rho (s'))\gamma (s',s,\rho ) > 0\}$ is open for all $s\in S$, and hence for all $s'\in \supp (\mu )$ it must be the case that \begin {equation*} (\rho (s) - \rho (s'))\gamma (s',s,\rho ) = 0 \end {equation*} for all $s\in S$. Thus, for all $s\in S$ and all $s'\in \supp (\mu )$, either $\rho (s) = \rho (s')$, or $\gamma (s',s,\rho ) = 0$. In the latter case, we see by sign-preservation of the conditional switch rate that \iftoggle {thesis}{$$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0,$$}{$\sign (\max \{0,\rho (s)-\rho (s')\}) = \sign (\gamma (s',s,\rho )) = 0$,} and hence $\rho (s) \le \rho (s')$. Therefore, we conclude that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} By \autoref {lem: equivalent_nash-general}, this proves that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and consequently that $v$ is Nash stationary.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: equivalent_nash-general} It holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$ if and only if $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Suppose first that $\rho (s) \le \rho (s')$ for all $s\in S$ and all $s'\in \supp (\mu )$. Then, it holds that \begin {equation*} \rho (s) = \int _S \rho (s) d\mu (s') \le \int _S \rho (s') d\mu (s') = \left <\rho ,\mu \right > \end {equation*} for all $s\in S$. Therefore, for all $\nu \in \P (S)$, we conclude that \begin {equation*} \left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right > d\nu (s) = \left <\rho ,\mu \right >, \end {equation*} which proves one direction of the lemma. \par On the other hand, suppose that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Then we have that $\rho (s) = \left <\rho ,\delta _s\right > \le \left <\rho ,\mu \right >$ for all $s\in S$. Furthermore, \begin {align*} \sup _{s\in \supp (\mu )} \rho (s) &= \int _S \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &= \int _{\supp (\mu )} \left (\sup _{s\in \supp (\mu )}\rho (s)\right ) d\mu (s') \\ &\ge \int _{\supp (\mu )} \rho (s') d\mu (s') \\ &= \int _S \rho (s') d\mu (s') \\ &= \left <\rho ,\mu \right >. \end {align*} Hence, $\sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Suppose for the sake of contradiction that there exists $s'\in \supp (\mu )$ such that $\rho (s') < \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$. Since $\rho $ is a continuous real-valued function on $S$, the preimage $U\coloneqq \rho ^{-1}((-\infty ,\left <\rho ,\mu \right >)) = \{s\in S : \rho (s) < \left <\rho ,\mu \right >\}$ is open and contains $s'$, and hence it must be the case that $\mu (U) > 0$ by definition of $\supp (\mu )$. Thus, since the Lebesgue integral of a positive function over a set of positive measure is positive, we find that \begin {align*} 0 &= \left <\rho ,\mu \right > - \left <\rho ,\mu \right > \\ &= \int _S (\left <\rho ,\mu \right > - \rho (s)) d\mu (s) \\ &= \int _U(\left <\rho ,\mu \right > - \rho (s))d\mu (s) + \int _{S\setminus U}(\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &\ge \int _U (\left <\rho ,\mu \right > - \rho (s))d\mu (s) \\ &> 0, \end {align*} which is a contradiction. Hence, it must be the case that $\rho (s') = \sup _{s\in \supp (\mu )}\rho (s) = \left <\rho ,\mu \right >$ for all $s'\in \supp (\mu )$. Therefore, $\rho (s') = \left <\rho ,\mu \right > \ge \left <\rho ,\nu \right >$ for all $\nu \in \P (S)$ and all $s'\in \supp (\mu )$, and in particular, we find that $\rho (s') \ge \left <\rho ,\delta _s\right > = \rho (s)$ for all $s\in S$ and all $s'\in \supp (\mu )$. This concludes the proof.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We prove the result for the two dynamics separately. \par \paragraph {BNN dynamics\iftoggle {longform}{.}{}} Consider the BNN dynamics of \autoref {ex: bnn}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) - \mu (B) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \frac {1}{2}\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s), \\ \sigma (\mu ,\rho ) &= \left <\rho ,v(\mu ,\rho )\right > \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ and $\sigma (\mu ,\rho )$ are finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$, since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}$ and $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ are continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \M (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S)\times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) = 0. \label {eq: zero_storage_bnn} \end {equation} Since $s\mapsto \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2$ is a continuous real-valued function on $S$, the preimage $U\coloneqq \{s\in S : \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 > 0\}$ is open. Therefore, if $U$ is nonempty, it contains some $s'\in S$, and hence since $\lambda $ has full support, $s'$ must be an element of $\supp (\lambda )$, implying that $\lambda (U) > 0$. This in turn would imply that $\int _U \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 d\lambda (s) > 0$ as the Lebesgue integral of a positive function over a set of positive measure is positive. However, this would contradict \eqref {eq: zero_storage_bnn}. Thus, $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}^2 = 0 ~ \text {for all $s\in S$}, \end {equation*} which holds if and only if \begin {equation} \rho (s) \le \left <\rho ,\mu \right > ~ \text {for all $s\in S$}. \label {eq: bnn_passivity_nash} \end {equation} It is clear that, if $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, then \eqref {eq: bnn_passivity_nash} holds. Conversely, if \eqref {eq: bnn_passivity_nash} holds, then $\left <\rho ,\nu \right > = \int _S \rho (s) d\nu (s) \le \int _S \left <\rho ,\mu \right >d\nu (s) = \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and thus by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}) we conclude that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then certainly $\sigma (\mu ,\rho ) = 0$ due to linearity of $\left <\rho ,\cdot \right >$. Notice that \iftoggle {thesis}{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &\qquad - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} }{ \begin {align*} \left <\rho ,v(\mu ,\rho )\right > &= \int _S \rho (s') d(v(\mu ,\rho ))(s') \\ &= \int _S \rho (s') \max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') - \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \int _S \rho (s') d\mu (s') \\ &= \int _S \left (\rho (s') - \int _S \rho (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s') \\ &= \int _S (\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} d\lambda (s'). \end {align*} } Notice that $(\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >)\max \{0,\left <\rho ,\delta _{s'}\right > - \left <\rho ,\mu \right >\} \ge 0$ for all $s'\in S$ and hence $\left <\rho ,v(\mu ,\rho )\right > \ge 0$. Furthermore, by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $, we see that \begin {equation*} \left <\rho ,v(\mu ,\rho )\right > = 0 \end {equation*} if and only if \begin {equation*} \rho (s') = \left <\rho ,\delta _{s'}\right > \le \left <\rho ,\mu \right > ~ \text {for all $s'\in S$}, \end {equation*} which, as shown above, holds true if and only if $v(\mu ,\rho ) = 0$. Furthermore, notice that by the same arguments, \begin {equation*} \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. Thus, \begin {equation*} \sigma (\mu ,\rho ) = \left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \ge 0, \end {equation*} with equality holding if and only if $v(\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Define $\tau \colon \R \to \Rpl $ by $\tau (r) = \max \{0,r\}^2$, so that $\tau '(r) = 2\max \{0,r\}$ and $\overline {\storage }(\mu ,\rho ) = \frac {1}{2}\int _S \tau (\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >) d\lambda (s)$. Computing the first partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(-\left <\rho ,v(\mu ,\rho )\right >) d\lambda (s) \\ &= -\left <\rho ,v(\mu ,\rho )\right >\int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \\ &= -\sigma (\mu ,\rho ). \end {align*} Computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \frac {1}{2}\int _S \tau '(\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >)(\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >) d\lambda (s) \\ &= \int _S (\left <\eta ,\delta _s\right > - \left <\eta ,\mu \right >)\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \left (\eta (s) - \int _S \eta (\tilde {s}) d\mu (\tilde {s})\right )\max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\}d\lambda (s) \iftoggle {thesis}{\\ & \qquad }{} - \int _S \eta (\tilde {s})d\mu (\tilde {s}) \int _S \max \{0,\left <\rho ,\delta _s\right > - \left <\rho ,\mu \right >\} d\lambda (s) \\ &= \int _S \eta (s) d(v(\mu ,\rho ))(s) \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof for the BNN dynamics. \par \paragraph {Impartial pairwise comparison dynamics\iftoggle {longform}{.}{}} Consider the impartial pairwise comparison dynamics of \autoref {ex: pcd}. We have that \begin {equation*} v(\mu ,\rho )(B) = \int _B \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _B \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \end {equation*} for all $\mu \in \P (S)$, all $\rho \in C(S)$, and all $B\in \B (S)$. Since the pairwise comparison dynamics under consideration are impartial, it holds that for all $s'\in S$, there exists some continuous function $\phi _{s'} \colon \R \to \Rpl $ such that \begin {equation*} \gamma (s,s',\rho ) = \phi _{s'}(\rho (s') - \rho (s)) \end {equation*} for all $s\in S$ and all $\rho \in C(S)$. For all $s'\in S$, define $\tau _{s'}\colon \R \to \Rpl $ by \begin {equation*} \tau _{s'}(r) = \int _{[0,r]} \phi _{s'}(u) du, \end {equation*} where we see that $\tau _{s'}(r) = 0$ whenever $r < 0$, since we take $[0,r] = \emptyset $ in such cases. Notice that $\tau _{s'}$ is strictly increasing on $[0,\infty )$ since $\phi _{s'}(u) > 0$ for all $u>0$: let $u>0$, let $s,s'\in S$ be such that $s\ne s'$, and let $\rho \in C(S)$ be such that $\rho (s')-\rho (s) = u > 0$ (which exists by Urysohn's lemma and the fact that $S$ is a metric space and hence normal), so that, by sign-preservation, we have that $\sign (\phi _{s'}(u)) = \sign (\phi _{s'}(\rho (s')-\rho (s))) = \sign (\gamma (s,s',\rho )) = \sign (\max \{0,\rho (s')-\rho (s)\}) = 1$. Define $\overline {\storage } \colon \M (S) \times C(S) \to \R $ and $\sigma \colon \P (S) \times C(S) \to \R $ by \begin {align*} \overline {\storage }(\mu ,\rho ) &= \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s'), \\ \sigma (\mu ,\rho ) &= -\overline {\storage }(v(\mu ,\rho ),\rho ). \end {align*} Notice that $\overline {\storage }(\mu ,\rho )$ is finite for all $\mu \in \M (S)$ and all $\rho \in C(S)$ since $(s,s')\mapsto \tau _s(\rho (s)-\rho (s'))$ is continuous and $S$ is compact. Also notice that $\overline {\storage }(\mu ,\rho ) \ge 0$ for all $\mu \in \P (S)$ and all $\rho \in C(S)$. Thus, we may define $\storage \colon \P (S) \times C(S) \to \Rpl $ by the restriction of $\overline {\storage }$ to the domain $\P (S) \times C(S) \subseteq \M (S) \times C(S)$. We claim that $\sigma $ and $\storage $ are appropriate maps to prove the strict $\delta $-passivity of $v$. \par To this end, first note that $\M (S)$ is strongly open, $\overline {\storage }$ is weak-$\infty $-continuous, $\overline {\storage }$ is Fr\'echet differentiable, $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$ and $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$ are weak-$\infty $-continuous, and every partial Fr\'echet derivative $\partial _1 \overline {\storage }(\mu ,\rho )$ is weakly continuous. All that remains to prove are \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta )\mapsto \left <\eta ,\mu \right >$, \eqref {eq: delta-dissipative-2}, \eqref {eq: delta-dissipative-3}, and that $\sigma \ge 0$. \par Let $\mu \in \P (S)$ and $\rho \in C(S)$. It holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \int _S \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d\mu (s') = 0, \end {equation*} which holds if and only if \begin {equation*} \tau _s(\rho (s) - \rho (s')) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}, \end {equation*} since $\lambda $ has full support, $s\mapsto \tau _s(\rho (s) - \rho (s'))$ is nonnegative and continuous for all $s' \in S$, and $s' \mapsto \int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)$ is nonnegative and continuous (which follows from compactness of $S$ together with the dominated convergence theorem). Since, for all $s\in S$, it holds that $\tau _s$ is strictly increasing on $[0,\infty )$ and $\tau _s(0) = 0$, it must be that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Therefore, by \autoref {lem: equivalent_nash-general}, it holds that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$. Hence, by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $\storage (\mu ,\rho ) = 0$ if and only if \begin {equation*} v(\mu ,\rho ) = 0, \end {equation*} which proves \eqref {eq: delta-dissipative-2}. \par Again let $\mu \in \P (S)$ and $\rho \in C(S)$. If $v(\mu ,\rho ) = 0$, then\iftoggle {thesis}{}{ certainly} $\sigma (\mu ,\rho ) = -\overline {\storage }(v(\mu ,\rho ),\rho ) = 0$ due to linearity of $\overline {\storage }(\cdot ,\rho )$. Writing out $\sigma (\mu ,\rho )$, we find that \begin {align*} \sigma (\mu ,\rho ) &= -\int _S\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s) d(v(\mu ,\rho ))(s') \\ &= -\int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s,s',\rho ) d\mu (s)\right ) d\lambda (s') \\ &\qquad + \int _S \left (\int _S \tau _s(\rho (s) - \rho (s')) d\lambda (s)\right )\left (\int _S \gamma (s',s,\rho ) d\lambda (s)\right ) d\mu (s') \\ &= \int _S\int _S \gamma (s',s,\rho ) \int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) d\lambda (s) d\mu (s'). \end {align*} For all $s,s'\in S$ such that $\rho (s) \le \rho (s')$, it holds by sign-preservation that $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 0$, and therefore $\gamma (s',s,\rho ) = 0$ for all such $s,s'$. On the other hand, if $s,s'\in S$ are such that $\rho (s) > \rho (s')$, then $\sign (\gamma (s',s,\rho )) = \sign (\max \{0,\rho (s)-\rho (s')\}) = 1$, implying that $\gamma (s',s,\rho ) > 0$. Furthermore, in this case with $\rho (s) > \rho (s')$, we see that $\rho (\tilde {s}) - \rho (s) < \rho (\tilde {s}) - \rho (s')$ for all $\tilde {s}\in S$, and therefore $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) \ge \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s} \in S$ by the fact that every $\tau _{\tilde {s}}$ is nondecreasing. Thus, we immediately see that \begin {equation*} \sigma (\mu ,\rho ) \ge 0. \end {equation*} We furthermore see that if $\sigma (\mu ,\rho ) = 0$, then \begin {equation*} \gamma (s',s,\rho )\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0 ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$} \end {equation*} by the usual arguments based on continuity and nonnegativity of the integrand together with full support of $\lambda $. Thus, let $s\in S$ and $s'\in \supp (\mu )$. Either $\gamma (s',s,\rho ) = 0$, or $\int _S \left (\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))\right ) d\lambda (\tilde {s}) = 0$. In the former case, it must be that $\rho (s) \le \rho (s')$, for otherwise $\phi _s(\rho (s) - \rho (s')) > 0$, which would contradict the fact that $\phi _s(\rho (s) - \rho (s')) = \gamma (s',s,\rho ) = 0$. Suppose that the latter case holds. Then either $\rho (s) \le \rho (s')$ or $\rho (s) > \rho (s')$. If $\rho (s) > \rho (s')$, then, as argued above, we find that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) - \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s)) \ge 0$ for all $\tilde {s}\in S$, and hence by the usual arguments based on continuity and nonnegativity of the integrand together with the full support of $\lambda $, we conclude that $\tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s')) = \tau _{\tilde {s}}(\rho (\tilde {s}) - \rho (s))$ for all $\tilde {s}\in S$. In this case, by the fact that every $\tau _{\tilde {s}}$ is strictly increasing on $[0,\infty )$ and $\rho (s') \ne \rho (s)$, it must be the case that, for all $\tilde {s}\in S$, we have that $\rho (\tilde {s}) - \rho (s') \le 0$ and $\rho (\tilde {s}) - \rho (s) \le 0$. But these two inequalities cannot hold simultaneously, as they would imply that $\rho (s) \le \rho (s')$ and $\rho (s') \le \rho (s)$, which contradicts the fact that $\rho (s) > \rho (s')$ in the case under consideration. Hence, we conclude that, when $\sigma (\mu ,\rho ) = 0$, it must hold that \begin {equation*} \rho (s) \le \rho (s') ~ \text {for all $s\in S$ and all $s'\in \supp (\mu )$}. \end {equation*} Thus, by \autoref {lem: equivalent_nash-general}, we find that $\left <\rho ,\nu \right > \le \left <\rho ,\mu \right >$ for all $\nu \in \P (S)$, and therefore by Nash stationarity of $v$ (\autoref {prop: bnn_pcd_satisfy_ns}), it holds that $v(\mu ,\rho ) = 0$ whenever $\sigma (\mu ,\rho ) = 0$. This proves \eqref {eq: delta-dissipative-3}. \par All that remains to be proven is \eqref {eq: delta-dissipative-1} with $w\colon (\mu ,\eta ) \mapsto \left <\eta ,\mu \right >$. Let $\mu \in \P (S)$, $\rho \in C(S)$, and $\eta \in C(S)$. Since $\overline {\storage }(\cdot ,\rho )$ is linear, it is immediate that $D(\overline {\storage }(\cdot ,\rho ))(\mu ) = \overline {\storage }(\cdot ,\rho )$, which implies that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho ) v(\mu ,\rho ) = \overline {\storage }(v(\mu ,\rho ),\rho ) = -\sigma (\mu ,\rho ). \end {equation*} Furthermore, computing the second partial Fr\'echet derivative of $\overline {\storage }$ using the chain rule yields that \begin {equation*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta = \int _S \int _S \tau _s'(\rho (s)-\rho (s'))(\eta (s)-\eta (s')) d\lambda (s) d\mu (s'), \end {equation*} where the derivatives of the functions $\tau _s \colon \R \to \R _+$ are computed via the fundamental theorem of calculus: \begin {equation*} \tau _s'(r) = \frac {d}{dr} \int _{[0,r]} \phi _s(u) du = \phi _s(r). \end {equation*} By impartiality of the pairwise comparison dynamics under consideration, we find that \begin {align*} \partial _2 \overline {\storage }(\mu ,\rho ) \eta &= \int _S \int _S \gamma (s',s,\rho ) (\eta (s) - \eta (s')) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s) \int _S \gamma (s',s,\rho ) d\mu (s') d\lambda (s) - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') \int _S \gamma (s,s',\rho ) d\mu (s) d\lambda (s') - \int _S \eta (s') \int _S \gamma (s',s,\rho ) d\lambda (s) d\mu (s') \\ &= \int _S \eta (s') d(v(\mu ,\rho ))(s') \\ &= \left <\eta ,v(\mu ,\rho )\right > \\ &= w(v(\mu ,\rho ),\eta ). \end {align*} Thus, altogether we find that \begin {equation*} \partial _1 \overline {\storage }(\mu ,\rho )v(\mu ,\rho ) + \partial _2 \overline {\storage }(\mu ,\rho ) \eta = -\sigma (\mu ,\rho ) + w(v(\mu ,\rho ),\eta ), \end {equation*} which shows that \eqref {eq: delta-dissipative-1} holds and hence concludes the proof.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}Notice that weak Lyapunov stability of $\NE (F)$ follows immediately from \autoref {thm: monotone-passive} together with \autoref {prop: bnn_pcd_satisfy_ns} and \autoref {prop: bnn_pairwise_are_delta-passive}. Furthermore, global weak attraction of $\NE (F)$ under \autoref {ass: game_derivative} follows by additionally noting that, for both the BNN dynamics and the impartial pairwise comparison dynamics, $v$ satisfies the appropriate continuity conditions of \autoref {ass: dynamics_map} and $v$ is $\|\cdot \|_\TV $-bounded on weak-$\infty $ compact subsets of $\P (S)\times C(S)$ (the latter condition of which follows from the fact that $v(\mu ,\rho )(B) \le 4\|\rho \|_\infty $ for all $\mu \in \P (S)$ and all $\rho \in C(S)$ for the BNN dynamics and that the conditional switch rate $\gamma $ is assumed bounded for the pairwise comparison dynamics).\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {lem: weakly_continuous_derivative-dpedm} \iftoggle {longform}{The map }{}$(\mu ,\rho )\mapsto D\overline {V}(\mu ,\rho )(v(\mu ,\rho ),u(\mu ,\rho ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}The result follows from a nearly identical analysis as in the proof of \autoref {lem: weakly_continuous_derivative} with minor changes. In particular, it follows from the $\|\cdot \|_\TV $-boundedness of $v$ on $\P (S)\times K$, the weak-$\infty $-to-weak continuity of $v$, the weak-$\infty $ continuity of $u$, the weak continuity of every $\partial _1 \overline {\storage }(\mu ,\rho )$ and every $\partial _1 \overline {\Gamma }(\mu ,\rho )$, and the weak-$\infty $ continuity of the maps $(\mu ,\rho )\mapsto \partial _1 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _2 \overline {\storage }(\mu ,\rho )$, $(\mu ,\rho )\mapsto \partial _1 \overline {\Gamma }(\mu ,\rho )$, and $(\mu ,\rho )\mapsto \partial _2 \overline {\Gamma }(\mu ,\rho )$.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxii}]\phantomsection\label{proof:prAtEndxii}The proof follows analogously to that of \autoref {cor: recovering_monotone}.\end{proof}

\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}This is immediate from \autoref {cor: recovering_monotone} together with \autoref {thm: continuous_war-monotone} and the fact that $F$ satisfies all of the appropriate regularity conditions.\end{proof}


==> tikzext/root-tac-figure0-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac-figure1-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac-figure10-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac-figure11-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac-figure12-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac-figure2-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac-figure3-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac-figure4-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac-figure5-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac-figure6-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac-figure7-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac-figure8-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac-figure9-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} The map $\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since we also have that $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, which proves the first assumption to be proven. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac_single-column-figure0-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac_single-column-figure1-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac_single-column-figure10-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac_single-column-figure11-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac_single-column-figure12-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac_single-column-figure2-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac_single-column-figure3-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac_single-column-figure4-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac_single-column-figure5-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac_single-column-figure6-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac_single-column-figure7-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac_single-column-figure8-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}


==> tikzext/root-tac_single-column-figure9-pratenddefaultcategory.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {lem: weakly_continuous_derivative} \iftoggle {longform}{The map }{}$\mu \mapsto D\overline {V}(\mu )v(\mu ,F(\mu ))$ is weakly continuous.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Since $S$ is a metric space, the weak topology on $\P (S)$ is metrizable \citep [Theorem~11.3.3]{dudley2002real}. Therefore, the weak topology on $\P (S)$ is first-countable and hence functions with domain $\P (S)$ are weakly continuous if they are weakly sequentially continuous. Thus, to prove the claim, it suffices to show that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )) \end {equation*} whenever $\mu _n \to \mu $ weakly. To this end, let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then we have that \iftoggle {twocol}{ \begin {equation} \begin {aligned} &|D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| \\ &\quad = |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\quad \le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\quad \quad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \end {aligned} \label {eq: weak_continuity_bound} \end {equation} }{ \begin {equation} \begin {aligned} |D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) - D\overline {V}(\mu )v(\mu ,F(\mu ))| &= |D\overline {V}(\mu _n)v(\mu _n,\overline {F}(\mu _n)) - D\overline {V}(\mu )v(\mu ,\overline {F}(\mu ))| \\ &\le |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad +|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) \iftoggle {thesis}{ \\ &\qquad \qquad }{}- v(\mu ,\overline {F}(\mu )))|. \end {aligned} \label {eq: weak_continuity_bound} \end {equation} } Assume for the time being that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. Then, under this assumption, it holds that \begin {equation*} |D\overline {V}(\mu )(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \to 0, \end {equation*} since $v(\mu _n,\overline {F}(\mu _n)) \to v(\mu ,\overline {F}(\mu ))$ weakly, as $\overline {F}$ is weakly continuous and $v$ is continuous with respect to the weak-$\infty $ topology on its domain and the weak topology on its codomain. Furthermore, \iftoggle {twocol}{ \begin {align*} &|(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {align*} }{ \begin {equation*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))v(\mu ,\overline {F}(\mu ))| \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu ,\overline {F}(\mu ))\|_\TV \to 0, \end {equation*} } since $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in the dual space $\M (S)^*$ with associated operator norm $\|\cdot \|_{\M (S)^*}$ induced by the total variation norm on $\M (S)$, as $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ by our above assumption. Finally, \iftoggle {twocol}{ \begin {multline*} |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ \begin {aligned} & \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) \\ &\qquad - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \to 0, \end {aligned} \end {multline*} }{ \iftoggle {thesis}{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ & \qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ & \qquad \to 0, \end {align*} }{ \begin {align*} & |(D\overline {V}(\mu _n) - D\overline {V}(\mu ))(v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu )))| \\ &\qquad \le \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \|v(\mu _n,\overline {F}(\mu _n)) - v(\mu ,\overline {F}(\mu ))\|_\TV \\ &\qquad \le 2\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \\ &\qquad \to 0, \end {align*} } } since again $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$ by the weak continuity assumption on $D\overline {V}$, and \iftoggle {thesis}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{\iftoggle {twocol}{$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$}{$$\sup _{\nu \in \P (S)}\|v(\nu ,\overline {F}(\nu ))\|_\TV \le \sup _{(\nu ,g)\in \P (S) \times \overline {F}(\P (S))} \|v(\nu ,g)\|_\TV \le M$$}} for some finite $M\in [0,\infty )$ by the $\|\cdot \|_\TV $-boundedness of $v$ on weak-$\infty $ compact subsets of $\P (S) \times C(S)$. Therefore, under the above assumptions, it must be that \begin {equation*} D\overline {V}(\mu _n)v(\mu _n,F(\mu _n)) \to D\overline {V}(\mu )v(\mu ,F(\mu )), \end {equation*} which is what was to be proven. Thus, it remains to prove the above assumptions, namely, that every Fr\'echet derivative $D\overline {V}(\nu )$ is weakly continuous, and that $D\overline {V}$ is weakly continuous on $\P (S)$. \par Let us first prove that $D\overline {V}(\mu )\colon \M (S) \to \R $ is weakly continuous for all $\mu \in U\cap U'$. Let $\mu \in U\cap U'$. Since $\partial _2 \overline {\storage }(\mu ,\rho ) \colon C(S) \to \R $ is continuous (with respect to the topology on $C(S)$ induced by $\|\cdot \|_\infty $) for all $\rho \in C(S)$ by definition of the Fr\'echet derivative, and since $D\overline {F}(\mu )\colon \M (S) \to C(S)$ is weakly continuous under the hypotheses of the theorem, it holds that the composition $\partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \colon \M (S) \to \R $ is weakly continuous. Since $\partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \colon \M (S) \to \R $ is also weakly continuous under the hypotheses of the theorem, we conclude that \begin {equation*} D\overline {V}(\mu ) = \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) + \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \end {equation*} is weakly continuous, proving the first assumption. \par Finally, let us prove the remaining assumption, namely, that $D\overline {V} \colon U\cap U' \to \M (S)^*$ is weakly continuous on $\P (S)$ (that is, continuous with respect to the weak topology on its domain $U\cap U' \subseteq \M (S)$ and the topology on its codomain $\M (S)^*$ induced by the operator norm $\|\cdot \|_{\M (S)^*}$). Once again, since we are considering weak continuity of a function on $\P (S)$, where the weak topology is first-countable, it suffices to prove weak sequential continuity. Let $\{\mu _n \in \P (S) : n\in \N \}$ be a sequence that converges weakly to $\mu \in \P (S)$. Then \iftoggle {twocol}{ \begin {align*} &\|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} \\ &\qquad \le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\qquad + \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) \\ &\qquad \qquad - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \rVert _{\M (S)^*}. \end {align*} }{ \begin {align*} \|D\overline {V}(\mu _n) - D\overline {V}(\mu )\|_{\M (S)^*} &\le \left \lVert \partial _1 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) - \partial _1 \overline {\storage }(\mu ,\overline {F}(\mu )) \right \rVert _{\M (S)^*} \\ &\iftoggle {thesis}{\quad }{\qquad }+ \left \lVert \partial _2 \overline {\storage }(\mu _n,\overline {F}(\mu _n)) \circ D\overline {F}(\mu _n) - \partial _2 \overline {\storage }(\mu ,\overline {F}(\mu )) \circ D\overline {F}(\mu ) \right \rVert _{\M (S)^*}. \end {align*} } It is clear that the first term in the above upper bound converges to $0$ due to the weak-$\infty $ continuity of $(\nu ,\rho )\mapsto \partial _1 \overline {\storage }(\nu ,\rho )$ together with the weak continuity of $\overline {F}$. Further upper-bounding the second term in a similar manner to the bound \eqref {eq: weak_continuity_bound} and appealing to the finiteness of $\|\varphi \|_{\TV }$ and $\|\psi \|_{\M (S)^*}$ for $\varphi \in C(S)^* = \M (S)$ and $\psi \in \M (S)^*$ together with the weak continuity of $\overline {F}$ and $D\overline {F}$ as well as the weak-$\infty $ continuity of $(\nu ,\rho ) \mapsto \partial _2 \overline {\storage }(\nu ,\rho )$ yields that the second term converges to $0$ as well. Thus, $D\overline {V}(\mu _n) \to D\overline {V}(\mu )$ in $\M (S)^*$, so $D\overline {V}$ is indeed weakly continuous on $\P (S)$.\end{proof}

